A Tale of Tidal Tails in the Milky Way

Hundreds of globular clusters and dwarf galaxies encircle the Milky Way. Many of these systems have undergone partial disruption due to tidal forces, littering the halo with stellar streams. These tidal tails are sensitive to the Galactic potential, facilitating an excellent laboratory to investigate Galaxy formation and evolution, as well as local chemical signatures of differing star formation environments. To better understand the emergence of the Milky Way, this thesis examines the dynamics and chemistry of a number of known stellar streams.

==> chapter1/chapter1.tex <==
\chapter{Halo Substructures in the Vicinity of the Virgo Over-Density}
\label{chap:sgr}
% you can put a brief note at the top of your chapters using '\previouslypublished{}'. For example, to give a reference to the paper this chapter is based on, or to point out that it has been submitted to a journal.

\previouslypublished{Parts of this chapter have been previously published as \href{http://adsabs.harvard.edu/abs/2012AJ....143...88C}{`Kinematics \& Chemistry of Halo Substructures: The Vicinity of the Virgo Over-Density', {Casey}, A.~R., {Keller}, S.~C., {Da Costa}, G., 2012, AJ, 143, 88C}. The work is presented here in expanded and updated form.} \\

We present observations obtained with the AAT's 2dF wide field spectrograph AAOmega of K-type stars located within a region of the sky which contains the VOD and the leading arm of the Sgr Stream.  On the basis of the resulting velocity histogram we isolate halo substructures in these overlapping regions including Sgr and previously discovered Virgo groups. Through comparisons with \textit{N}-body models of the Galaxy-Sgr interaction, we find a tri-axial dark matter halo is favoured and we exclude a prolate shape. This result is contradictory with other observations along the Sagittarius leading arm, which typically favour prolate models.  We have also uncovered K-giant members of Sgr that are notably more metal poor ($\langle[$Fe/H$]\rangle = -1.7\,\pm\,0.3$ dex) than previous studies. This suggests a significantly wider metallicity distribution exists in the Sagittarius Stream than formerly considered. We also present data on five carbon stars which were discovered in our sample.

\section{Introduction}
%The proportion of substructure recently uncovered in the Galaxy has highlighted the crucial involvement accretion has played in the formation of the Milky Way \citep[see][and references therein]{Helmi_2008}. Properties of these stellar structures allow us to probe the formation mechanisms and history of the Galaxy. Recent studies \citep{Carollo;et-al_2007, Carollo;et-al_2010} have suggested multiple evolutionary paths are required for galaxy formation to reconcile observational evidence, although this is a subject of ongoing debate \citep{Schoenrich;et-al_2011}. Regardless, the dissipation-less merging paradigm is widely accepted and consistent with favoured Cold Dark Matter ($\Lambda$CDM) cosmology models. Through the examination of ongoing accretion events in the Milky Way and fossils from previous mergers we can trace the evolution of the outer most regions of the Galaxy \citep[e.g.,][]{Helmi;White_2001}.
	
% Accretion is at least partly \citep[e.g.,][]{Starkenburg;et-al_2009}, if not entirely responsible for the formation of the stellar halo. \citet{Bell;et-al_2008} compared Sloan Digital Sky Survey \citep[hereafter SDSS]{York;et-al_2000} data to galaxy formation simulations using different dark halos and found that observations are consistent with the stellar halo being entirely formed by hierarchical merging of accreted satellites (see also \citet{Xue;et-al_2011}).
	
The most prominent ongoing accretion event in the Milky Way is the Sgr dSph galaxy. The tidal tails of the disrupting satellite were originally discovered by \citet{ibata;et-al_1994} as a co-moving group of K- and M-type giants. Almost two decades since this discovery, stream debris is seen to circle our Galaxy. As such, the Sgr tidal tails have been extensively traced with red-clump stars \citep{Majewski;et-al_1999}, carbon stars \citep{Totten;Irwin_1998, ibata;et-al_2001}, RR Lyrae stars \citep{Ivezic;et-al_2000, Vivas;et-al_2005, keller;et-al_2008, Watkins;et-al_2009, Prior;et-al_2009b}, A-type stars \citep{Newberg;et-al_2003}, BHB stars \citep{Ruhland;et-al_2011} and K/M-giants \citep{Majewski;et-al_2003,  Yanny;et-al_2009, keller;et-al_2010}. Tracers originating from the host system can be identified with spatial and kinematical information because they remain dynamically cold, and are identifiable as kinematic substructures long after they are stripped from their progenitor \citep[e.g.,][]{Ibata;Lewis_1998, Helmi;White_1999}. 
	
Stars within these tidal tails are kinematically sensitive to the galactic potential. This has led various groups to model the Sgr interaction with different dark matter profiles. \citet{Martinez-Delgado;et-al_2004} traced the Northern leading arm and found a near spherical or oblate ($q \approx 0.85$) dark matter halo best represented the observed debris, coinciding with the findings of \citet{ibata;et-al_2001}. In contrast, \citet{Helmi_2004} found evidence in the Sgr leading debris that most favoured a prolate ($q = 1.25$) halo. \citet{Vivas;et-al_2005} found that either a prolate or spherical model of \citet{Helmi_2004} would fit their RR Lyrae observations, rather than those of an oblate model. \citet{Johnston;et-al_2005} later pointed out that no prolate model can reproduce the orbital pole precession of the Sgr debris, but an oblate potential could. \citet[hereafter LJM05]{Law;et-al_2005} performed simulations using data of the Sgr debris from the 2MASS catalogue and found that the kinematics of leading debris was best fit by prolate halos, whereas the trailing debris typically favoured oblate halos. \citet{Prior;et-al_2009a} reached a similar conclusion.
	
\citet{belokurov;et-al_2006} found an apparent bifurcation within the Sgr debris which \citet{Fellhauer;et-al_2006} argued can only result from a dark halo having a near spherical shape. \citet{Law;et-al_2009} introduced a tri-axial model with a varying flattening profile $q$, which replicates the orbital precession seen and matches kinematic observations of the Sgr debris. However \citet{Law;Majewski_2010} (hereafter LM10) concede this may be a purely numerical solution as tri-axial halos are dynamically unstable. They emphasize that more kinematic measurements in other regions of the Sgr stream are required.

After the Sgr stellar stream, the VOD is arguably the next most significant substructure within our Galaxy. The first over-density in the vicinity of the VOD was observed as a group of RR Lyrae stars by the QUEST survey \citep{Vivas;et-al_2001}. The collaboration later named this the ``$12{\mbox{$.\!\!^{\mathrm h}$}}4$ clump'' \citep{Zinn;et-al_2004}. The broad nature of the VOD was uncovered from the SDSS catalogue as a diffuse over-density of main-sequence turnoff stars centered at $r_\odot \sim18$ kpc \citep[which ][dubbed as S297+63-20.5]{Newberg;et-al_2002}. The nomenclature on the substructure names within this region is varied. In this chapter when referring to the VOD we are discussing the spatial over-density of stars within the region, separate from any detected co-moving groups.
	
It is difficult to accurately distinguish stars in the VOD, as there are multiple substructures along this line-of-sight. \citet{Duffau;et-al_2006} took observations of BHB and RR Lyrae within the ``$12{\mbox{$.\!\!^{\mathrm h}$}}4$ clump'' and found a common velocity of $V_{GSR} = 99.8$\,km s$^{-1}$ with $\sigma_{v} = 17.3$\,km s$^{-1}$. It should be noted that the dispersion in kinematics measured by \citet{Duffau;et-al_2006} is essentially their velocity precision, so the substructure may possess a much smaller kinematic dispersion. This co-moving group was coined the `Virgo Stellar Stream' (VSS) to differentiate it from the broad spatial over-density. This distinction from the VOD was strengthened with new distance measurements that placed the VOD centroid at $r_\odot = 16$\,kpc \citep{Juric;et-al_2008, keller;et-al_2010}, and the VSS 3\,kpc further away \citep{Duffau;et-al_2006}. Although, when considered in the light of systematic and observational uncertainties, this is of marginal significance. Additionally, \citet{Juric;et-al_2008} suggests the VOD may extend between $r_\odot = 6$ to 20\,kpc, which further complicates the matter of distance separation.
 
The relationship between the VSS and the S297+63-20.5 over-density is still unclear. \citet{Newberg;et-al_2007} found a kinematic signature at $V_{GSR} = 130 \pm 10$\,km s$^{-1}$ for members of the VOD/S297+63-20.5, which is extremely close to the VSS peak. The VSS and S297+63-20.5 are co-incident in space, but their velocity difference has not yet been reconciled. The distance measurements between S297+63-20.5 and the VSS are similar enough ($\sim$1\,kpc) for \citet{Newberg;et-al_2007} and \citet{Prior;et-al_2009a} to infer they are part of the same structure. \citet{Newberg;et-al_2007} estimate a distance to S297+63-20.5 of $r_\odot = 18$\,kpc from $g_0 = 20.5$ turnoff stars, but they concede the structure is likely dispersed along the line-of-sight as the Color-Magnitude Diagram (CMD) for this region does not demonstrate a tight sequence.  Certainly this region of sky, aptly coined the 'Field of Streams' by \citet{belokurov;et-al_2006}, is complex territory.
	
Photometric studies are inadequate to fully untangle this region. Kinematics are essential to identify co-moving groups that are distinct from the field. Chemical information is vital to accurately distinguish these substructures and understand their origins. However, very few studies have directly investigated metallicities for these stars. In this chapter we present spectroscopic observations of K-giants in this region.  Sgr stream kinematics are used to probe the shape of the dark matter halo in the Galaxy. We report both the velocities and metallicities of these giants in an effort to help untangle this accretion-dominated region.

Target selection methodology is outlined in the next section which is followed with details regarding the observations. Techniques used to separate K-giants from dwarfs are discussed in Section \ref{sec:ch1-dwarf-giant-separation}, and our analysis procedure for kinematics (Section \ref{sec:ch1-kinematics}) and metallicities (Section \ref{sec:ch1-metallicities}) follows. A discussion of substructures is outlined in Section \ref{sec:ch1-discussion}, and in Section \ref{sec:ch1-carbon-stars} we report the carbon stars discovered in our sample. In Section \ref{sec:ch1-conclusions} we conclude with some final remarks and critical interpretations. 

\section{Target Selection}
\label{sec:ch1-target-selection}

When the presence of a stellar substructure is uncovered, K-giants provide excellent candidates for spectroscopic follow-up. Their spectra permit precise radial velocities and chemical abundances. In order to target K-giants we have targeted candidates within the color selection box shown in Figure \ref{fig:cmd-target-selection}, taken from the SDSS DR7 catalogue. This selection box favors a metal-poor population at Sgr stream-like distances ($\sim$40 kpc) but will also contain similarly metal-poor stars at VOD/VSS distances ($\sim$20 kpc) without being significantly biased. Some field dwarfs are expected to contaminate the sample due to their similarity in colors. Although K-dwarfs are difficult to distinguish photometrically, we can spectroscopically separate these through the equivalent width (EW) of the  gravity-sensitive Mg I triplet lines at 516.7\,nm, 517.3\,nm, and 518.4\,nm (see Section \ref{sec:ch1-dwarf-giant-separation}).

\begin{figure}[h]
	\includegraphics[width=\columnwidth]{chapter1/cmd.pdf}
	\caption[Photometric target selection for the Virgo Over-Density]{CMD of our observed regions from SDSS DR7, overlaid with the color selection criterion used to target K-giants. Appropriate Dartmouth isochrones \citep{Dotter;et-al_2008} are shown for Sgr debris at a distance of $r_\odot =40$ kpc \citep{belokurov;et-al_2006}}
	\label{fig:cmd-target-selection}
\end{figure}

\section{AAT Observations with AAOmega}
\label{sec:ch1-observations}

Low-resolution spectra were obtained for targets over two runs using AAOmega on the 3.9-m Anglo-Astronomical Telescope at Siding Springs Observatory in New South Wales, Australia. AAOmega is a double-beam, multi-object (392) fibre-fed spectrograph covering a two degree field of view. The targets were observed in normal visitor mode in April 2009. Throughout all observations, sufficient sky fibres ($\sim$30) were allocated to ensure optimal sky subtraction. In total 3,453 science targets were observed across 4 fields within the VOD/Sgr region, as outlined in Table \ref{tab:ch1-observations}. Multiple configurations were observed for most fields to permit measurements of bright ($i < 16$) and faint ($i > 16$) stars, as well as repeat observations on a subset of stars.

The beam was split into red and blue arms using the 570\,nm dichroic. The 580V grating in the blue arm yields spectra between 370-580\,nm, with a resolution of $\mathcal{R} = 1300$. In the red arm we used the 1000I grating ($\mathcal{R} = 4400$) which spans the spectral range from 800-950\,nm. This coverage includes the Ca II near infrared triplet (CaT) lines, which are used for radial velocities and metallicities. Science targets on each configuration were limited to 1.5 magnitudes in range to minimise scattered-light cross talk between fibres. Globular clusters NGC 5024, 5053 and 5904 were observed as radial velocity and metallicity standards.


\begin{table}[h!]
\centering
\caption{Observed field centers and number of configurations\label{tab:ch1-observations}}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc}
\hline
\hline
Field & $\alpha$ & $\delta$ & Field \\
& (J2000) & (J2000) & Configurations \\
\hline
A & 12 00 00 & $+00$ 00 00 & 1 \\ 
B & 12 20 00 & $-01$ 00 00 & 2 \\ 
C & 12 40 00 & $-02$ 00 00 & 3 \\ 
D & 12 56 00 & $-02$ 42 00 & 6 \\ 
\hline
\end{tabular}%}
\end{table}


The data were reduced using the 2\textsc{DFDR}\footnote{http://www.aao.gov.au/AAO/2df/aaomega} pipeline. After being flat-fielded, the fibres were throughput calibrated and the sky spectrum was subtracted using the median flux of the dedicated sky fibres. Wavelength calibration was achieved from Th-Ar arc lamp exposures taken between each set of science fields. Multiple object frames were combined to assist with cosmic ray removal. 


\section{Dwarf / Giant separation}
\label{sec:ch1-dwarf-giant-separation}

When discussing our data with respect to halo substructures in this chapter, we are referring only to K-type giants.  Dwarfs that fall within our apparent magnitude limit are not sufficiently distant to probe halo substructures. Here we utilise the equivalent width (EW) of the Mg I triplet lines to identify and exclude dwarfs from our analyses. 	

A grid of synthetic spectra have been generated to quantitively establish a suitable giant/dwarf separation criterion. The grid was generated using \citet{castelli;kurucz_2004} model atmospheres with the MOOG\footnote{http://www.as.utexas.edu/$\sim$chris/moog.html} spectral synthesis code \citep{sneden_1973} and the line list of \citet{Kurucz;Bell_1995}. Spectra were also generated using stellar parameters for the Sun and Arcturus. The strength of the Mg I lines were tuned to match both the Solar and Arcturus atlases of \citet{Hinkle;et-al_2003}. \citet{girardi;et-al_2004} isochrones have been used to translate our de-reddened $g - i$ color range to effective temperature. Reddening is accounted for using the \citet{Schlafly;Finkbeiner_2011} corrected dust maps of \citet{schlegel;et-al_1998} assuming a \citet{fitzpatrick_1999} dust profile where $R_V = 3.1$. The corresponding effective temperature region ranges from 3900\,K to 5200\,K, and is stepped at 25\,K intervals. We have assumed a surface gravity of $\log{g} = 2$ for giants and $\log{g} = 4.5$ for dwarfs. Metallicities of [Fe/H] $= -0.5$, $-1.5$, and $-2.5$ were considered for both surface gravities.

All synthetic spectra were convolved with a Gaussian kernel of 3.03\,\AA{} to match the resolution of our 580V spectra, and interpolated onto the observed wavelength dispersion map. Mg I line strengths for our observations and synthetic spectra are shown against $g - i$ in Figure \ref{fig:dwarf-giant-separation}. As expected, there is an overlap of Mg I strengths between metal-rich ``giants'' ($\log{g} = 2$) and metal-poor ``dwarfs'' ($\log{g} = 4.5$). However we do not expect metal-poor dwarfs to be a principle contaminant due to their intrinsically low luminosities and comparative rarity.

\begin{figure}[h]
	\includegraphics[width=\columnwidth]{chapter1/dwarfgiant.pdf}
	\caption[Dwarf/giant discriminant for Virgo Over-Density and Sgr stars]{The sum of the Mg I triplet EWs for observations and synthetic spectra shown against the Sloan $g\,-\,i$ color. Synthetic spectra are shown for $\log{g} = 2$ ($\bigtriangledown$) and $\log{g} = 4.5$ ($\bigtriangleup$), and points are colored by metallicity. Our dwarf/giant separation line is shown (solid). }
	\label{fig:dwarf-giant-separation}
\end{figure}

We have adopted a linear separation line to distinguish dwarf and giant stars. The slope and offset of this line were varied to assess the effectiveness in differentiating giants from dwarfs. A balance must be made between the recoverability of giant stars, and the contamination of dwarf stars. Using the rule,
\begin{equation}
	EW_{Mg\,I} < 3(g-i)_o + 0.5
\end{equation}
\noindent{}we identify 185 giants in our observed fields. An analysis of our 185 giant candidates revealed three stars with high proper motions \citep[PPMXL Catalog, ][]{roser;et-al_2010}, all of which lay close to our dwarf/giant separation line. This suggests they are dwarfs, and they have been excluded. Some possible giant targets were also discarded due to insufficient $S/N$, or because the Mg I triplet fell on bad columns of the detector. All efforts were made to minimise these losses. The distilled giant sample size is 178 stars. All identified K-giant stars in our distilled sample had no proper motion detectable above measurement errors.


\section{Radial Velocities}
\label{sec:ch1-kinematics}

The Ca II triplet absorption lines at 849.8\,nm, 854.2\,nm and 866.2\,nm have been used to measure radial velocities. These lines are strong, and easily identifiable in red giant branch (RGB) stars even at low resolution.  Observed spectra have been cross-correlated with a synthetic spectrum of a metal-poor giant to measure radial velocities. Heliocentric corrections were also applied. Radial velocity measurements made of the standard stars in our globular clusters agree (within $\pm$3\,km s$^{-1}$) with the catalogue of \citet{harris_1996} (2011 edition). Furthermore, a number of our targets were observed on multiple fields, allowing us to calculate the internal measurement error. The differences between multiple measurements of the same target were calculated and they form a half-normal distribution with a {HWHM $= 3.58$\,km s$^{-1}$}. 
	
In order to compare our kinematic results in a homogenous manner, we have translated our heliocentric velocities to a galactocentric frame. We have adopted the circular velocity of the Local Standard of Rest (LSR) at the Sun as 220\,km s$^{-1}$ \citep{kerr;lynden-bell_1986} and accounted for the Sun's peculiar velocity to the LSR by using 16.5\,km s$^{-1}$ towards $l = 53^\circ, b = 25^\circ$ \citep{mihalas;binney_1981}. The corrected line-of-sight velocity is then given by,

\begin{equation}
	V_{GSR} =  V_{OBS} + 220\sin{l}\cos{b} + 16.5\times[\sin{b}\sin{25^\circ} + \cos{b}\cos{25^\circ}\cos{(l - 53^\circ)}]
\end{equation}

\noindent where $V_{OBS}$ is the heliocentric-corrected observed line-of-sight velocity. A caveat to this reference transformation is that other authors in the literature have used slightly different formulae to transpose their kinematics to a galactocentric frame. This will result in possible systematic shifts in velocities between authors of up to $\sim$11\,km s$^{-1}$. 

\section{Metallicities}
\label{sec:ch1-metallicities}

We have measured metallicities for our giants using the strength of the Ca II triplet lines. This technique was first empirically described for individual stars in globular clusters \citep{armandroff;da_costa_1991}. A spectroscopic analysis using VLT/FLAMES observations of RGB stars from composite populations led \citet{battaglia;et-al_2008} to conclude that a calibrated CaT--[Fe/H] relationship can be confidently used in composite stellar populations \citep[see also][]{Rutledge;Hesser;Stetson_1997, starkenburg;et-al_2010}. The caveat to this technique is that a luminosity (specifically $V - V_{HB}$) is required for calibration, and we have to assume a $V_{HB}$ luminosity here. Johnson $V$-band magnitudes for our giants were calculated from SDSS \textit{ugriz} photometry using \citet{Jester;et-al_2005} transformations. The weaker third Ca II triplet line is more susceptible to noise and residual sky-line contamination \citep{Tolstoy;et-al_2001,battaglia;et-al_2008}. Consequently, only the strongest two CaT lines (854.2\,nm and 866.2\,nm) have been used to form a total EW ($W'$) such that,

\begin{eqnarray}
	\textstyle\sum{W}\, &=& EW_{8542} + EW_{8662} \\
	W' &=&\textstyle\sum{W} + 0.64\left(\pm 0.02\right)\left(V-V_{HB}\right)
\end{eqnarray}
\noindent and the metallicity linearly varies with W' where,
\begin{equation}
	\mbox{[Fe/H]}_{\mbox{\small{CaT}}} = (-2.81\pm0.16) + (0.44\pm0.04) W'
	\label{eq:feh-cat}
\end{equation}

Using this calibration our globular cluster standard stars (with known $V_{HB}$ magnitudes) have metallicities that match well with the \citet{harris_1996} catalogue (2011 edition). Only K-giants within the valid calibration range ($0 > V-V_{HB} > -3$) were considered for metallicities. We assume that we have two dominant substructures present in our observations; the leading arm of Sgr and the Virgo Over-Density (see Section \ref{sec:ch1-substructure-identification}). The Sgr stream dominates our negative $V_{GSR}$ population, and our positive kinematic space primarily comprises VOD and VSS members. As such we have separated our population at $V_{GSR} = 0$\,km s$^{-1}$ into two samples with assumed $V_{HB}$ magnitudes. Although this introduces a (known) systemic effect, it is a required assumption to estimate the metallicity distribution of each population.

The horizontal branch magnitude assumed for the VSS/VOD has been ascertained from previous RR Lyrae studies. As RR Lyrae stars sit on the horizontal branch, the $V_{HB}$ is taken as the V-band median of four \citet{Prior;et-al_2009a} and three  \citet{Duffau;et-al_2006} VSS members to yield $\langle{}V\rangle{} = 17.09$. This combined value matches well with the mean horizontal branch magnitude reported by \citet{Duffau;et-al_2006}. In our K-giant sample with positive galactocentric velocities, we assume $V_{HB} = 17.09$, implying these stars are at a distance of $\sim$20 kpc.

The distance to the Sgr debris varies greatly throughout the Milky Way. Through CMD comparisons with the Sgr core \citep{Bellazzini;et-al_2006}, \citet{belokurov;et-al_2006} determined distances along the two branches of the Sgr bifurcation.  Revised distance measurements by \citet{Siegel;et-al_2007} (as tabulated in Table 1 of LM10) have been crucial in constraining dark halo models. Our observations lay on the edge of Branch A (Figure \ref{fig:sgr-field-of-streams}).

We have assumed distances to these stars by interpolating their position along a cubic spline fitted to published distances \citep{Siegel;et-al_2007}. Recent distance measurements of the stream by \citet{Ruhland;et-al_2011} match the stream distances used here within the uncertainties. The horizontal branch magnitude $V_{HB}$ is calculated using this assumed distance, and the known luminosity of RR Lyrae stars \citep[$M_V = +0.69;$][]{Tsujimoto;et-al_1998}. The typical $V_{HB}$ magnitude derived for the Sgr members is $18.7$, corresponding to a distance of $\sim{}$41 kpc. Reddening is accounted for using the \citet{schlegel;et-al_1998} maps with \citet{Schlafly;Finkbeiner_2011} corrections as described in Section \ref{sec:ch1-dwarf-giant-separation}. Uncertainties in distance are not interpolated; they are taken as the largest published uncertainty of the closest neighbouring data points, and this is propagated through to our reported metallicity uncertainties. The kinematics and metallicities derived for our giant sample are discussed in the following section.


\section{Discussion}
\label{sec:ch1-discussion}
		
	\subsection{Substructure Identification}
	\label{sec:ch1-substructure-identification}
		
A significant kinematic deviation from a canonical halo population signifies a co-moving group. There are multiple substructures along our line-of-sight. These features are identified first and discussed separately. We have represented our galactocentric velocities with a generalised histogram (Figure \ref{fig:velocity-histogram}) to quantitatively compare the observed stellar kinematics with the hypothesis that the parent distribution can be described by a canonical halo where $\mu = 0$ km s$^{-1}$, and $\sigma = 101.6$\,km s$^{-1}$ \citep{Sirko;et-al_2004}.

	\begin{figure}
		\includegraphics[width=\textwidth]{chapter1/velocity_halo.pdf}
		\caption[Generalised histogram of galactocentric velocities, illustrating the substructure present]{Generalised histogram of $V_{GSR}$ for our 178 K-type giants, highlighting the substructure present. The Gaussian distribution represents the halo contribution; it is normalised such that the integral equals the number of observed stars excluding those outside a 2.5-$\sigma$ excess. Significant ($>3\sigma$) kinematic deviations from the smooth distribution are appropriately grouped and labelled.}
		\label{fig:velocity-histogram}
	\end{figure}
	
	
The generalised histogram represents each data point with a Gaussian kernel of an equal deviation. As our internal kinematic errors between multiple measurements summate to a half-normal distribution with a FWHM of 7.16\,km s$^{-1}$, we have opted for a sigma value of 10 km s$^{-1}$ for the generalised histogram in Figure \ref{fig:velocity-histogram} to avoid under-smoothing. The most significant ($>3\sigma$) kinematic peaks have been labeled Features A, B, and C. Features A and C are our most significant structures, and the importance of Feature B becomes more evident through Monte-Carlo simulations. 


	Velocities and metallicities of our K-giants, shown in the left panel of Figure \ref{fig:monte-carlo}, were binned into grid blocks of 15\,km s$^{-1}$ and 0.3\,dex \--- roughly twice the error in each dimension. To interpret these data a population of 178 stars were randomly drawn from a simulated halo with canonical kinematics. Metallicities were randomly assigned using the observed halo metallicity distribution function (MDF) of \citet{Ryan;Norris_1991}. Each simulated population was binned identically to our observed sample. Simulation grid blocks with counts equal to or exceeding stars in the equivalent observed grid block were noted, and summed after 10,000 simulations. Results from our Monte-Carlo simulations are illustrated in Figure \ref{fig:monte-carlo} (right). The identified Features A, B, and C in our results were consistently significant when the grid was midpoint offset in both dimensions, except for the grid-block centered at $\sim185$\,km s$^{-1}$ and $\sim-1.4$\,dex, which has consequently been left unlabelled.
	
\begin{figure}
		\includegraphics[width=\textwidth]{chapter1/monte_carlo.pdf}
		\caption[Monte-Carlo simulations to quantify the level of kinematic substructure present]{The observed data for the 178 giant star sample (left panel). Monte-Carlo simulation results illustrating the number of times simulations could reproduce our observed data in the equivalent multi-dimensional bin (right panel). Significant features discussed in the text are labelled.}
		\label{fig:monte-carlo}
	\end{figure}	

	 Substructure becomes statistically significant when the observed grid blocks are rarely replicated in Monte-Carlo simulations. Specifically, the number of members in Feature A were never reproduced in some grid blocks. This feature is well in excess of the halo, and has a wide spread in kinematics. \citet{Chou;et-al_2007} mapped the Sgr debris across the sky using K/M-giants and found galactocentric velocity signatures between $-205$\,km s$^{-1}$ to $-31$\,km s$^{-1}$ in this region. As such we attribute this wide, significant kinematic peak as the leading arm of the Sgr tidal tail. Feature A is discussed in the next section. Another feature where grid blocks were never reproduced in our simulations was Feature C. This feature may also be attributed to Sgr debris and is discussed further in Section \ref{sec:ch1-feature-c}.
	 	
	 The clump of stars in the velocity bin centered on $V_{GSR} \approx 130$ km s$^{-1}$ and [Fe/H] $\approx -2$ was replicated only $\sim1$\% in 10,000 simulations. We attribute these stars to the VSS, as they are coincident in spatial position, velocity, and metallicity with previously reported values of the VSS obtained by F turnoff/BHB stars \citep{Newberg;et-al_2007} and RR Lyrae stars \citep{Prior;et-al_2009a}. Feature B is discussed in Section \ref{sec:ch1-the-vss}.

	\begin{figure}
		\includegraphics[width=\textwidth]{chapter1/adapted_belokurov_2006.pdf}
		\caption[Observed fields upon a panoramic view of the Sagittarius stream]{Observed fields are outlined upon a panoramic view of the Sgr stream, to demonstrate our field locations in context with the Sgr stream. This plot is an adaptation of Figure 2 in \citet{belokurov;et-al_2006}, which uses the 2MASS M-giant sample of \citet{Majewski;et-al_2003}.}
		\label{fig:sgr-field-of-streams}
\end{figure}
	
	\subsection{Feature A \--- Sagittarius Debris}
	\label{sec:ch1-sgr-debris}
	
	  The locations of observed fields are overlaid upon a panoramic projection of the Sgr stream and the  `Field of Streams'  \citep{belokurov;et-al_2006} in Figure \ref{fig:sgr-field-of-streams}. This is a crowded region of globular clusters, substructures and overlapping stellar streams, primarily populated by the Sgr northern leading arm. Simply from a spatial perspective, we expect the Sgr debris to dominate our data. Although the VOD is present, it is much more diffuse. 
	
	\subsubsection{Comparing Sagittarius Debris to Dark Matter Halo Models}	

	In order to investigate the spatial coverage and kinematics of our Sgr members, we have compared our data with the constant flattening spheroidal models of LJM05, and the more recent tri-axial model of LM10. The simulated data output from these models is readily available online\footnote{http://www.astro.virginia.edu/$\sim$srm4n/Sgr/}, and the released models have the best-fitting parameters for each dark halo shape (prolate, spherical, oblate and tri-axial). These were the only simulations available at the time which made use of an all-sky data set; the 2MASS M-giant sample. We have not considered particles farther than 60\,kpc to match realistic observation limitations. The $10^5$ model Sgr debris particles from their simulations are represented along the best-fit great-circle ($\Lambda_\odot$, $B_\odot$) where the longitudinal coordinate $\Lambda_\odot$ is zero in the direction of the Sgr core and increases along the trailing debris. For comprehensive details of the simulations the reader is referred to the papers of \citet{Law;et-al_2005} and \citet{Law;Majewski_2010}. 
		
\begin{figure}
	\centering
		\includegraphics[width=0.7\textwidth]{chapter1/law_spatial.pdf}
		\caption[Generalised histograms showing predicted galactocentric velocities from best-fitting dark matter halos compared with observations]{Our fields and observed bounds are shown with the simulated particles from multiple \textit{N}-body simulations by LJM05 and LM10. These particles are distance restricted (up to 60 kpc), and color-coded by their peri-centric passage (yellow; most recent passage, red; previous passage, blue; oldest observable passage).}
\label{fig:law-spatial}
\end{figure}


	The northern leading arm of Sgr is particularly sensitive both kinematically and spatially to the shape of the Milky Way dark halo (Figure \ref{fig:law-spatial}). The spherical, oblate and tri-axial models predict the Sgr stream to pass directly through our fields, whereas the prolate model predicts only the edge of the stream near this region, and no particles directly in our fields. Spatially, the prolate model predicts the Sgr stream to pass much lower in latitude ($B_\odot$) than our observed fields. When we extend a rectangle bounded by the edges of our fields (as per the zoomed insets in Figure \ref{fig:law-spatial}) a mere two model particles are found. The $10^5$ model particles are proportional to the stream density so the lack of model particles implies a negligible stream concentration in our observed region. When the number of field configurations is accounted for, our observed Sgr K-giants are uniformly distributed across the fields. If this prolate halo model is a true representation of the Sgr debris, this does not exclude the potential of finding some Sgr debris in our fields. However, it does imply that if the LJM05 prolate model is an accurate representation of the dark halo then Sgr would not be the dominant population \--- contrary to our preferred interpretation of the observations.
	
	In comparison, the tri-axial, spherical and oblate models predict varying amounts of debris from previous peri-centric passages in our fields. A kinematic comparison against our observations is necessary to evaluate model predictions. As the prolate model has only two simulated particles within our extended bounds there is no qualitative kinematic comparison to be made for this model, therefore the prolate model is excluded from further kinematic analysis.

	\begin{figure}
		\includegraphics[width=\textwidth]{chapter1/sgr_velocities.pdf}
		\caption[Generalised histogram of galactocentric velocities and heliocentric distances for simulated particles]{A generalised histogram (left) of the galactocentric rest frame velocities in our sample (dotted line) compared to the velocities (solid line) from the \textit{N}-body models of LJM05, LM10 of particles within the same spatial coverage and distance range (up to $r_\odot \sim$60 kpc) of our observed sample. Heliocentric distances for particles used to generate each velocity histogram are shown on the right. Particles are marked by their peri-centric passage. A plus ($+$) denotes debris from the current peri-centric passage by Sgr, circles ($\circ$) mark the previous passage, and squares ($\square$) represent debris from two previous passages. The prolate model from LJM05 is not considered in this plot (see text).}
		\label{fig:law-vel-compare}
	\end{figure}
	
	The number of predicted particles observable differs between models. Consequently, the kinematics for each model have been represented as a generalised histogram (Figure \ref{fig:law-vel-compare}). For consistency all simulation output and observed data has been convolved with a Gaussian kernel of 10\,km s$^{-1}$; the sigma used for the previous generalised histogram in Figure \ref{fig:velocity-histogram}. Predicted distances and peri-centric ages are shown, demonstrating that debris from multiple passages are predicted along the line-of-sight. A much tighter velocity sequence is predicted by the tri-axial model than the constant flattening models. This is because the tri-axial model predicts a peri-center almost precisely in our observable region, whereas the spherical and oblate models predict a large wrap along the line-of-sight, resulting in a wide spread of distances and velocities.
	
	Predicted distances are consistent with what we would expect from our observations. The median luminosities of our giants is $g\sim$17.5, so for the tri-axial model particles at 45\,kpc this corresponds to an absolute magnitude of $M_g\sim-0.8$; quite reasonable for a K-giant. Similarly for the spherical and oblate models, typical distances of $\sim$25\,kpc will yield luminosities of $M_g\sim+0.5$ which is also reasonable.  
	
	The spherical and oblate models also predict close-by debris with extremely negative galactocentric velocities. This signature is not represented in our data. The lowest observed velocity is $\sim{}$$-$250\,km s$^{-1}$, and we have only two observations less than $V_{GSR} < -200$\,km\,s$^{-1}$. In contrast, the spherical/oblate models predict velocities well below $V_{GSR} < -300$\,km\,s$^{-1}$. These predicted stars with highly negative velocities were also not found in Sgr RR Lyrae study of \citet{Prior;et-al_2009b}. If the dark matter potential is well-represented by either an oblate or spherical halo, then this discrepancy must be reconciled. 
	
	The oblate and spherical model also illustrate a similar signature at $r_\odot \sim$12\,kpc, with particle velocities ranging between $-100 < V_{GSR} < 0$\,km s$^{-1}$. This is the edge of a predicted crossing-point between different wraps of the stream, which occurs at $\sim$12\,kpc. These particles --and the positive kinematic signature around $\sim$20\,kpc in the oblate model -- are relatively minor signatures when compared to the northern leading arm. If these signatures are present in our observed fields, their relatively low density compared to the Northern arm would prevent them from appearing as significant. 
	
	Although the predicted velocity distribution is narrower than what we observe, the LM10 tri-axial dark halo model best fits our observations. The observed sample broadens most prominently towards more negative galactocentric velocities at $\sim-200$\,km s$^{-1}$, considerably higher than oblate/spherical model predictions. Halo contamination at highly negative velocities is likely to be small. One reconciliation for this discrepancy between our observations and the tri-axial model may lie in the workings of the tri-axial model itself. Unlike other models considered, the tri-axial model does not reproduce the observed bifurcation in the Sgr stream \citep{belokurov;et-al_2006}. Although observationally untested, it is reasonable to suggest a bifurcation may result from a significant kinematic disruption. Such an effect could result in a broader kinematic distribution \--- similar to what we have observed \--- which is most notable at the stream edges.
	
	There is further work required through observations and simulations to reconcile kinematic discrepancies. Typical examinations of the leading arm debris usually favour prolate halos and evidence along the trailing arm typically favours oblate halos \citep{Helmi_2004, Martinez-Delgado;et-al_2004, Law;et-al_2005}. Kinematic predictions of the LM10 tri-axial model reasonably match our observations, whereas the prolate model has been excluded as significant debris is not predicted in this edge of the stream. These observations along the northern leading arm are the first which are not reproducible with the current prolate model of LJM05, contrary to previous groups who have surveyed closer to the leading arm debris.

	\subsubsection{A Metal-Poor Population Uncovered in Sagittarius Debris}
	\label{sec:ch1-sgr-metal-poor}
		
	Many groups have found the population of the Sgr core to possess a mean [Fe/H] $\sim -0.5$\,dex \citep{Cacciari;et-al_2002, Bonifacio;et-al_2004, Monaco;et-al_2005}. The observed metallicity gradient along the stream suggests that as the host circles the Milky Way the older, more metal-poor stars are preferentially stripped from the progenitor \citep{Chou;et-al_2007, keller;et-al_2010}. In this region of the stream very few Sgr member metallicities have been reported. \citet{Vivas;et-al_2005} found a mean metallicity of $\langle$[Fe/H]$\rangle = -1.77$ from spectra of 16 RR Lyrae stars along a nearby region of the Sgr leading arm. Similarly, \citet{Prior;et-al_2009b} found $\langle$[Fe/H]$\rangle = -1.79 \pm 0.08$\,dex for 21 type \textit{ab} RR Lyrae stars in the region. This is somewhat expected since only the oldest, most metal-poor stars can form RR Lyraes. 
	
	Investigating the MDF of the Sgr debris requires an unbiased sample. Generally K-giants are excellent stellar candidates for such studies, as all stars go through this evolutionary phase, whereas M-giants are consistently metal-rich. If we apply the metallicity gradient found by \citet[][with M-giants]{keller;et-al_2010} to these observed K-giants, we would expect an abundance mean near $\sim{}-1.2$ dex in this observed region. The metallicity distribution for our entire negative $V_{GSR}$ sample is shown in Figure \ref{fig:sgr-metallicity-hist}, and illustrates a metal-poor population. The mean of our distribution is $\langle$[Fe/H]$\rangle = -1.7\,\pm\,0.3$\,dex. If we include only the stars attributed to Feature A (as defined by the shaded region in Figure \ref{fig:velocity-histogram}, between $-140 < V_{gsr} < -30$\,km s$^{-1}$) this value increases by only 0.04\,dex; well within observational uncertainties. As a comparison, in a sample of metal-rich biased M-giants from the 2MASS data \citet{Chou;et-al_2007} found a mean metallicity of $\langle$[Fe/H]$\rangle = -0.72$\,dex for their best subsample in the northern leading arm of Sgr. Although there may be some halo contamination in our sample, in general our more metal-poor Feature A members have higher negative velocities, which is expected for Sgr stream members in this region.
		
	\begin{figure}[h]
		\includegraphics[width=\textwidth]{chapter1/sgr_feh_hist.pdf}
		\caption[Observed metallicity histogram for giant stars with negative galactocentric velocities]{Metallicity histograms for K-giant members in our negative galactocentric velocity sample, which is largely populated by Sgr debris from the Northern leading arm.}
		\label{fig:sgr-metallicity-hist}
	\end{figure}

	It is likely that our observed K-giant sample is biased towards more metal-poor members. Given a typical distance of $r_\odot\sim 40$\,kpc for the Sgr debris in this region \citep{belokurov;et-al_2006}, a 12\,Gyr old Dartmouth \citep{Dotter;et-al_2008} isochrone with a metallicity of [Fe/H] $= -1.5$ falls directly within our target selection window. The more metal-rich isochrone with [Fe/H] $= -0.5$ does not pass through our selection range. This is consistent with our observed metallicities for Sgr. Although this does not prohibit the possibility of more metal-rich members within our sample, it implies that our distribution is biased towards the metal-poor end of the MDF. The tail of our Sgr distribution extends from [Fe/H] = $-0.71$ to $-2.35$\,dex.

	\subsection{Feature B \--- The Virgo Stellar Stream}
	\label{sec:ch1-the-vss}
	
	Another substructure which was distinguished from the VOD is the Virgo Stellar Stream \citep{Duffau;et-al_2006}. Several RR Lyrae stars have been observed with a common velocity of $V_{GSR} = 130$\,km s$^{-1}$ \citep{Newberg;et-al_2007, Prior;et-al_2009a}. \citet{Prior;et-al_2009a} also measured metallicities of stars with this kinematic signature and found a mean [Fe/H] $= -1.95\,\pm\,0.1$ for the VSS, although this is based on RR Lyrae stars, and therefore is potentially biased to the oldest, most metal-poor populations. The RR Lyrae sample from \citet{Duffau;et-al_2006} found a $\langle$[Fe/H]$\rangle = -1.86$ with a much larger abundance spread of $\sigma = 0.40$, several times larger than the relative uncertainty in individual values ($\sigma_{{\rm [Fe/H]}} = 0.08$\,dex). This led \citet{Duffau;et-al_2006} to infer the progenitor of the VSS was likely a dSph galaxy, as a large dispersion in $\mbox{[m/H]}$ indicates self-enrichment, implying the structure is a galaxy and not an isolated mono-metallic cluster. Although some globular clusters are also now known to contain multiple populations and sizeable $\mbox{[m/H]}$ dispersions, globular clusters in general have a much smaller dispersion than that observed here. Similar to \citet{Duffau;et-al_2006}, we  also observe an abundance spread within this kinematic bin, including two K-giants with mean kinematics and metallicities ($\langle{}V_{GSR}\rangle{} = 130 \pm 9$ km s$^{-1}, \langle\mbox{[Fe/H]}\rangle = -2.0 \pm 0.16$) matching those found by \citet{Prior;et-al_2009a}. Monte-Carlo simulations reproduced these targets a mere $\sim1$\% in 10,000 simulations \--- highlighting their significance.

	High resolution follow-up spectroscopy on these three targets and other VSS candidates at higher metallicities in this kinematic range will provide crucial information about the origin of the VSS.  Investigating [$\alpha$/Fe] ratios in these candidates can constrain the mass of the VSS progenitor and discern whether the host was indeed a dSph \citep{venn;et-al_2004, Casetti-Dinescu;et-al_2009}. Future observations are planned.

	\subsection{Feature C \--- Sagittarius debris?}
	\label{sec:ch1-feature-c}

	The last significant kinematic substructure we identify in our data is Feature C. There are two peaks identified at $V_{GSR} = 200$\,km s$^{-1}$ and $240$\,km s$^{-1}$. These features cannot be explained by a smooth halo distribution. \citet{Newberg;et-al_2007} identified a 4$\sigma$ peak at $V_{GSR} = 200$\,km\,s$^{-1}$ in their sample of F turnoff stars centered on $(l, b) = (288^\circ, 62^\circ)$. Our nearest field to their plate (Field B) hosts only one star associated with this peak; most of our stars are located within our most populated Field D. \citet{Prior;et-al_2009b} also noted stars in this kinematic range and compiled a list of authors who have similarly observed such peaks (see \citet{Sirko;et-al_2004, Duffau;et-al_2006, starkenburg;et-al_2009}). \citet{Prior;et-al_2009b} argue these stars may be associated with trailing debris of Sgr, as suggested by models (LJM05, LM10). Although this trailing debris would be much closer than the nearby visible leading arm, our observations support the interpretation by \citet{Prior;et-al_2009b} as the metallicities are quite similar to the nearby Sgr debris.
	
	This substructure has a range of metallicities. These metallicities were derived assuming a single distance modulus to the VOD/VSS. The abundance dispersion we observe is either representative, or these stars have a common metallicity and are dispersed along the line-of-sight. Unfortunately neither scenario can be positively excluded without further observations. If these peaks are associated with the trailing debris of Sgr debris, they are likely to be further away than the VOD. On our scale that would make these stars more metal-rich than shown in Figure \ref{fig:monte-carlo}. However, the nearest trailing debris particles predicted from any best-fitting dark halo potential that could explain this kinematic peak occur at $\sim\Lambda_\odot = 310^\circ$; our observations range in longitude between $\Lambda_\odot = 256-273^\circ$. Whether this substructure is separate from Sgr debris or not remains equivocal. Nevertheless, the apparent metallicities of the Feature C stars are not inconsistent with those of a Sgr population given our results for Feature A and those of \citet{keller;et-al_2010}.
	
\section{Carbon Stars}
\label{sec:ch1-carbon-stars}	

	Five carbon stars have been identified in this sample. The colour selection shown in Figure \ref{fig:cmd-target-selection} overlaps with the colours of carbon stars. These stars were not specifically targeted, and their surface densities are so low \citep[$\approx$ 1 per 50 deg$^2$;][]{Green;et-al_1994} that we would not expect them as a substantial contaminant.  Although our sky coverage is small ($\sim$12.5 deg$^2$), the observed carbon star spatial density is $\sim$20x higher than expected. All five carbon stars are recognisable by the presence of distinctive 473.7\,nm and 516.5\,nm Swan C$_2$ bands.


\begin{figure}
	\includegraphics[width=\textwidth]{chapter1/carbon_stars.pdf}
	\caption[Carbon stars identified in this study]{Sloan \textit{u \--- g} and \textit{g \--- r} colors for our carbon stars, and the identified carbon stars and classifications by \citet{Downes;et-al_2004}. Carbon stars identified in this work have been shaded for clarity.}
	\label{fig:carbon-sdss}
\end{figure}

	 Dwarf carbon stars exhibit a spectral signature which mimics that of a typical CH-type giant carbon star, however they have anomalous JHK colors \citep{Green;et-al_1992} and high proper motions. The existence of the 430\,nm CH G-band is representative of a CH-type carbon star, and is found in all five of our carbon stars. SDSS photometry for our stars match well with the F/G-type CH carbon stars identified by \citet{Downes;et-al_2004}, as seen in Figure \ref{fig:carbon-sdss}. However these targets were not spectroscopically observed in the SDSS follow-up survey SEGUE. Through comparisons with previous carbon-type star catalogues \citep{Totten;Irwin_1998, Downes;et-al_2004, Goswami;et-al_2010}, the stars tabulated in Table \ref{tab:carbon-stars} are previously unclassified carbon stars. This is largely because our objects are too faint to have been observed by previous spectroscopic carbon star surveys.
	
\begin{table}[h!]
\centering
\caption{Properties of carbon stars found in our sample\label{tab:carbon-stars}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccrc}
\hline
\hline
SDSS Name J+\tablenotemark{a} &
$M_g$ & 
$u - g$ & $g - r$ & $r - i$ & $i - z$ & $H-K$ & $J-H$ & $\mu_{\alpha\cos{\delta}}\tablenotemark{c}$ & $\mu_\delta\tablenotemark{c}$ & $V_{GSR}$ & Likely \\
& & & & & & & & (mas yr$^{-1}$) & (mas yr$^{-1}$) & (km s$^{-1}$) & dwarf? \\
\hline

121740.94-001839.5 & 18.66 & 1.10 & 0.54 & 0.16 & 0.05 & ...\tablenotemark{b}& ...\tablenotemark{b} & $-3.0 \pm 5.4$  & $-18.0 \pm 5.4$ & $-71 \pm 34$ & Yes\\
121853.18-004628.4 & 17.71 & 1.67 & 0.73 & 0.22 & 0.11 & 0.24 & 0.36 &  $-3.7 \pm 4.5$ & $-0.5 \pm 4.5$ & $176 \pm 9$ & - \\
122053.71-011709.5 & 17.65 & 1.79 & 0.80 & 0.26 & 0.13 & 0.16 & 0.56 &  $-7.3 \pm 4.3$ & $-3.9 \pm 4.3$ & $31 \pm 11$ & - \\
125410.80-032744.0 & 18.59 & 1.43 & 0.64 & 0.22 & 0.05 & 0.56 & 0.32 &$-21.1 \pm 5.0 $ & $-7.7 \pm 5.0$ & $-41 \pm 9$ & Yes \\ 
125416.52-031437.6 & 16.85 & 1.72 & 0.73 & 0.25 & 0.11 & -0.11 & 0.50 & $-19.8 \pm 4.2$ & $+8.7 \pm 4.2$& $15 \pm 4$ & Yes \\
\hline
\end{tabular}}
\tablenotetext{a}{To keep with convention, positional information has been truncated. Full information available through the SDSS archive.}
\tablenotetext{b}{No \textit{JHK} photometry is available for this object as it is fainter than the 2MASS survey limit.}
\tablenotetext{c}{Proper motions taken from the PPMXL Catalog \citep{roser;et-al_2010}.}
\end{table}


	There is 2MASS photometry available for four of these stars. Of those, two stars (SDSS J125410.80-032744.0 and J125416.52-031437.6) exhibit anomalous JHK colors and significant ($>3\sigma$) proper motions \citep[PPMXL;][]{roser;et-al_2010}; characteristics of a dwarf carbon star. A third star also exhibits significant proper motion (SDSS J121740.94-001839.5), however JHK photometry is unavailable. The two remaining stars in our sample have JHK photometry characteristic of the F/G type CH carbon stars found by \citet{Downes;et-al_2004} in their Faint High-Latitude Carbon (FHLC) star survey (Figure \ref{fig:carbon-sdss}), and do not exhibit significant proper motion - which strongly suggests they are not dwarfs \citep{Green;et-al_1994, Deutsch_1994}.

	
\section{Conclusions}
\label{sec:ch1-conclusions}

	We present spectroscopic observations of K-type stars in a region of the 'Field of Streams', where significant substructure is present. We utilise the gravity-sensitive Mg I triplet lines to separate giant and dwarf stars. Radial velocities and metallicities of 178 K-giants have been determined. We have recovered kinematic substructure found by other authors, which cannot be explained by a smooth halo distribution. Highly negative velocity signatures match those expected by the Sgr stream debris, and we also identify a group of K-giants with metallicities and kinematics which make them highly probable members of the VSS.

	Stars in this region of the Sgr stream are kinematically sensitive to the shape of the Galactic dark halo. As such, we have compared our velocity distribution to the Sgr-Milky Way dark matter models of \citet{Law;et-al_2005, Law;Majewski_2010}. Typically, leading arm debris favour prolate models and trailing arm debris favour oblate models. A prolate dark halo predicts relatively little debris in our observed fields. If the spheroid is prolate and LJM05 presents an accurate representation, Sgr debris would not be expected to dominate our sample even if we were $\Delta{}B_\odot\sim10^\circ$ closer to the great circle best-fit. However, Sgr debris is our most significant kinematic structure observed. No single model perfectly represents our data, although we find the more recent tri-axial model (LM10) best represents our observed kinematics. 
	
	Observed metallicities for K-giants in this region of the Sgr stream are notably lower than expected based on other Sgr samples, demonstrating the presence of a metal-poor population in the  Sgr debris. Although isochrones indicate we are biased towards metal-poor members at these distances, these stars are unequivocally Sgr in origin. Metallicity gradients reported suggest a mean of $\langle[$Fe/H$]\rangle\sim{}-1.2$, whereas our population has $\langle[$Fe/H$]\rangle = -1.7 \pm 0.3$\,dex. Previously reported abundances in this region have been ascertained from observing RR Lyrae stars (where the mean metallicity found was $\langle\mbox{[Fe/H]}\rangle\sim{}-1.7$\,dex) or from observing M-giants (where $\langle\mbox{[Fe/H]}\rangle\sim{}-0.7$\,dex was reported). In both scenarios, the measurements are reasonable with what we would expect from each particular stellar population. Thus the sample presented here is more representative of the complete MDF, and less susceptible to age or metallicity biases. These observations also demonstrate that the Sgr stream likely hosts a substantially larger abundance range than previously suggested by RR Lyrae and M-giant studies, including a previously un-detected metal-poor population of K-giants.



==> chapter1/table.tex <==
\ctable[caption=Photometric candidates within 5.5 deg of \echa,doinside=\tiny,pos=p,captionskip=3pt,width=\textwidth,label=table:photcand]{ccccccccXcccc}{}
{
\toprule[2pt]
  \multicolumn{1}{c}{2MASS ID} &
  \multicolumn{1}{c}{$J$} &
  \multicolumn{1}{c}{$H$} &
  \multicolumn{1}{c}{$K_{s}$} &
  \multicolumn{1}{c}{DENIS ID} &
  \multicolumn{1}{c}{$i$} &
  \multicolumn{1}{c}{$J$} &
  \multicolumn{1}{c}{$K$} &
  \multicolumn{1}{c}{NOMAD ID} &
  \multicolumn{1}{c}{$\mu_{\alpha}\cos\delta$} &
  \multicolumn{1}{c}{$\sigma_{\mu_{\alpha}\cos\delta}$} &
  \multicolumn{1}{c}{$\mu_{\delta}$} &
  \multicolumn{1}{c}{$\sigma_{\mu_{\delta}}$} \\
& \multicolumn{3}{c}{\rule{8mm}{0.5pt} [mag] \rule{8mm}{0.5pt}} & & \multicolumn{3}{c}{\rule{8mm}{0.5pt} [mag] \rule{8mm}{0.5pt}} & & \multicolumn{4}{c}{\rule{12mm}{0.5pt} [\masyr] \rule{12mm}{0.5pt}}  \\
\midrule
  06434426$-$8120578 & 12.54 & 11.98 & 11.75 & J064343.8$-$812058 & 14.3 & 12.66 & 11.62 & 0086$-$0022191 & $+$236.0 & 29.0 & $+$50.0 & 1.0\\
  06462710$-$8112221 & 11.39 & 10.73 & 10.48 & J064626.9$-$811222 & 12.95 & 11.36 & 10.37 & 0087$-$0021147 & $+$90.0 & 14.0 & $+$40.0 & 3.0\\
  06492625$-$7832302 & 13.97 & 13.34 & 12.97 & J064926.1$-$783230 & 16.33 & 13.91 & 13.2 & 0114$-$0022673 & 0.0 & 0.0 & 0.0 & 0.0\\
  06492684$-$7830096 & 11.81 & 11.21 & 10.95 & J064926.7$-$783009 & 13.35 & 11.88 & 10.95 & 0114$-$0022675 & $+$10.7 & 6.5 & $+$61.6 & 6.0\\
  07051818$-$8211297 & 15.34 & 14.97 & 14.45 & J070517.9$-$821130 & 18.12 & 15.67 & & \\
  07235966$-$8015179 & 11.3 & 10.82 & 10.44 & J072359.5$-$801517 & 13.42 & 11.33 & 10.34 & 0097$-$0023438 & $-$400.0 & 13.0 & $+$726.0 & 15.0\\
  07291649$-$7801257 & 11.14 & 10.54 & 10.31 & J072916.5$-$780125 & 12.7 & 11.08 & 10.18 & 0119$-$0028000 & 0.0 & 0.0 & 0.0 & 0.0\\
  07301029$-$7949465 & 11.79 & 11.2 & 10.88 & J073010.2$-$794946 & 13.38 & 11.79 & 10.83 & 0101$-$0024103 & $+$2.0 & 13.0 & $+$40.0 & 6.0\\
  07360613$-$7615306 & 11.98 & 11.35 & 11.07 & J073606.1$-$761530 & 13.78 & 11.89 & 11.1 & 0137$-$0038802 & $-$66.0 & 5.0 & $+$188.0 & 29.0\\
  07363553$-$8334516 & 11.76 & 11.26 & 10.91 & J073635.5$-$833451 & 13.47 & 11.69 & 10.84 & 0064$-$0017785 & $-$88.0 & 2.0 & $+$92.0 & 1.0\\
  07363787$-$7553548 & 15.11 & 14.53 & 14.04 & J073637.7$-$755354 & 17.71 & 15.04 & 13.73 & 0141$-$0043715 & 0.0 & 0.0 & 0.0 & 0.0\\
  07413127$-$7857463 & 12.31 & 11.73 & 11.4 & J074131.2$-$785746 & 14.22 & 12.24 & 11.41 & 0110$-$0025049 & $-$26.0 & 42.0 & $+$70.0 & 14.0\\
  07450450$-$7515483 & 13.76 & 13.34 & 13.2 & J074504.7$-$751550 & 16.33 & 13.78 &  & 0147$-$0056811 & $-$2.5 & 6.7 & $+$23.6 & 7.1\\
  07455327$-$7926217 & 12.18 & 11.54 & 11.28 & J074553.7$-$792621 & 13.82 & 12.39 & 11.29 & 0105$-$0025051 & 0.0 & 0.0 & 0.0 & 0.0\\
  07464520$-$7848403 & 15.03 & 14.41 & 13.97 & J074645.2$-$784841 & 17.84 & 15.18 &  & 0111$-$0025239 & 0.0 & 0.0 & 0.0 & 0.0\\
  07493223$-$8046366 & 12.01 & 11.43 & 11.11 & J074932.5$-$804638 & 13.73 & 12.17 & 11.05 & 0092$-$0023931 & $-$176.0 & 2.0 & $+$216.0 & 3.0\\
  07514986$-$8134348 & 10.79 & 10.15 & 9.94 & J075150.0$-$813435 & 12.35 & 10.96 & 9.94 & 0084$-$0029863 & $-$6.1 & 6.1 & $-$2.9 & 6.0\\
  07515088$-$7504221 & 11.95 & 11.4 & 11.07 & J075150.9$-$750421 & 13.59 & 12.2 & 11.22 & 0149$-$0060296 & $+$8.1 & 6.1 & $+$15.7 & 6.2\\
  07524497$-$7527172 & 9.74 & 8.98 & 8.73 & J075245.1$-$752717 & 11.28 & 9.88 & 8.76 & 0145$-$0053268 & $-$4.7 & 6.0 & $+$17.7 & 6.0\\
  07595212$-$7426018 & 11.62 & 10.97 & 10.76 & J075952.1$-$742601 & 13.39 & 11.66 & 10.81 & 0155$-$0073794 & $-$10.0 & 6.0 & $+$8.9 & 6.2\\
  08014860$-$8058052 & 11.29 & 10.6 & 10.23 & J080148.6$-$805805 & 13.17 & 11.31 & 10.23 & 0090$-$0024145 & $-$10.0 & 3.0 & $+$26.0 & 10.0\\
  08015214$-$7410216 & 11.7 & 11.13 & 10.85 & J080152.1$-$741021 & 13.22 & 11.72 & 10.76 & 0158$-$0079617 & 0.0 & 0.0 & 0.0 & 0.0\\
  08025781$-$8330076 & 10.67 & 10.04 & 9.71 & J080257.7$-$833007 & 12.52 & 10.58 & 9.65 & 0064$-$0019143 & $-$116.0 & 17.0 & $+$124.0 & 5.0\\
  08040986$-$7552265 & 15.17 & 14.42 & 14.08 & J080409.6$-$755226 & 18.06 & 15.12 &  & 0141$-$0046221 & 0.0 & 0.0 & 0.0 & 0.0\\
  08060539$-$7732313 & 12.85 & 12.29 & 11.98 & J080605.3$-$773232 & 14.73 & 12.84 & 11.9 & 0124$-$0045366 & $-$40.0 & 13.0 & $-$78.0 & 9.0\\
  08061506$-$7712441 & 11.82 & 11.23 & 10.98 & J080614.9$-$771244 & 13.32 & 12.15 & 11.25 & 0127$-$0047178 & $-$6.8 & 6.4 & $-$5.4 & 6.5\\
  08154563$-$7654027 & 11.4 & 10.89 & 10.58 & J081545.5$-$765403 & 12.96 & 11.41 & 10.62 & 0130$-$0047650 & $+$32.0 & 6.5 & $+$108.9 & 6.2\\
  08194309$-$7401232 & 10.06 & 9.43 & 9.2 & J081943.1$-$740123 & 11.67 & 10.01 & 9.23 & 0159$-$0086496 & $-$18.7 & 6.0 & $+$37.9 & 6.0\\
  08202975$-$8003259 & 11.3 & 10.73 & 10.43 & J082029.9$-$800325 & 12.96 & 11.2 & 10.32 & 0099$-$0027452 & $-$36.0 & 14.0 & $+$34.0 & 8.0\\
  08261843$-$7337418 & 12.15 & 11.52 & 11.25 & J082618.5$-$733742 & 13.8 & 12.13 & 11.22 & 0163$-$0105857 & $-$104.0 & 8.0 & $+$116.0 & 0.0\\
  08265778$-$7421593 & 11.36 & 10.71 & 10.49 & J082657.7$-$742159 & 12.9 & 11.35 & 10.59 & 0156$-$0079527 & $+$56.3 & 6.0 & $+$3.6 & 6.2\\
  08280966$-$7736574 & 14.22 & 13.58 & 13.17 & J082809.6$-$773658 & 16.8 & 14.13 & 13.15 & 0123$-$0045758 & $+$40.0 & 12.0 & $+$190.0 & 10.0\\
  08285425$-$8145094 & 13.77 & 13.2 & 12.83 & J082854.3$-$814509 & 15.96 & 13.77 & 12.63 & 0082$-$0032706 & $-$68.0 & 15.0 & $+$34.0 & 7.0\\
  08293859$-$7444155 & 14.58 & 13.98 & 13.91 & J082938.7$-$744413 & 17.73 &  &  & 0152$-$0070533 & 0.0 & 0.0 & 0.0 & 0.0\\
  08352539$-$7443428 & 12.71 & 12.15 & 11.84 & J083525.3$-$744343 & 14.54 & 12.6 & 11.85 & 0152$-$0071222 & $+$52.0 & 20.0 & $+$108.0 & 6.0\\
  08401433$-$8133555 & 13.64 & 13.14 & 12.72 & J084014.4$-$813355 & 16.13 & 13.6 & 12.84 & 0084$-$0033355 & $-$20.0 & 2.0 & $-$6.0 & 4.0\\
  08485911$-$8035017 & 10.42 & 9.79 & 9.5 & J084859.5$-$803501 & 12.06 & 10.43 & 9.51 & 0094$-$0029124 & 0.0 & 0.0 & 0.0 & 0.0\\
  08495184$-$7657072 & 11.68 & 11.12 & 10.77 & J084952.2$-$765708 & 13.32 & 11.7 & 10.84 & 0130$-$0052425 & $-$264.0 & 19.0 & $+$198.0 & 17.0\\
  08513016$-$7503119 & 11.36 & 10.76 & 10.5 & J085130.2$-$750312 & 12.93 & 11.22 & 10.41 & 0149$-$0068148 & $-$14.2 & 6.3 & $+$36.6 & 6.0\\
  08514891$-$7338397 & 12.28 & 11.7 & 11.39 & J085148.9$-$733839 & 14.06 & 12.14 & 11.32 & 0163$-$0109404 & 0.0 & 0.0 & 0.0 & 0.0\\
  08524138$-$7613377 & 11.69 & 11.11 & 10.81 & J085241.4$-$761338 & 13.27 & 11.6 & 10.68 & 0137$-$0047278 & 0.0 & 0.0 & 0.0 & 0.0\\
  08533950$-$8204523 & 11.47 & 10.83 & 10.62 & J085339.6$-$820452 & 12.98 & 11.48 & 10.51 & 0079$-$0035296 & $-$38.2 & 6.0 & $+$11.5 & 6.0\\
  08595512$-$7728298 & 11.78 & 11.22 & 10.91 & J085955.1$-$772830 & 13.45 & 11.81 & 10.82 & 0125$-$0055097 & $-$81.3 & 9.0 & $+$32.0 & 9.0\\
  09011161$-$8100433 & 13.85 & 13.26 & 12.9 & J090111.7$-$810043 & 16.03 & 13.83 & 12.74 & 0089$-$0030427 & $-$36.0 & 7.0 & $+$18.0 & 8.0\\
  09053087$-$8134572 & 12.16 & 11.6 & 11.3 & J090531.2$-$813458 & 14.16 & 12.21 & 11.21 & 0084$-$0035278 & $-$52.0 & 19.0 & $+$8.0 & 17.0\\
  09071270$-$8053594 & 12.5 & 11.88 & 11.54 & J090712.8$-$805400 & 14.28 & 12.49 & 11.6 & 0091$-$0030281 & $-$188.0 & 19.0 & $+$166.0 & 32.0\\
  09074165$-$7747024 & 11.96 & 11.35 & 11.22 & J090741.5$-$774703 & 13.8 & 11.98 & 11.23 & 0122$-$0047685 & $-$21.6 & 6.1 & $+$20.4 & 6.1\\
  09075370$-$8246148 & 15.01 & 14.5 & 14.21 & J090753.5$-$824616 & 17.63 & 14.99 &  & 0072$-$0028031 & 0.0 & 0.0 & 0.0 & 0.0\\
  09095558$-$7743129 & 14.78 & 14.04 & 13.54 & J090955.7$-$774313 & 17.68 & 14.7 & 13.17 & 0122$-$0047974 & 0.0 & 0.0 & 0.0 & 0.0\\
  09104094$-$7552528 & 13.62 & 12.98 & 12.59 & J091041.0$-$755253 & 15.82 & 13.56 & 12.48 & 0141$-$0054372 & $-$58.0 & 23.0 & $+$30.0 & 9.0\\
  09125959$-$8311515 & 11.56 & 10.98 & 10.69 & J091259.8$-$831152 & 13.4 & 11.57 & 10.55 & 0068$-$0024433 & $-$390.0 & 5.0 & $+$712.0 & 11.0\\
  09133435$-$7550099 & 11.86 & 11.32 & 11.0 & J091334.3$-$755010 & 13.82 & 11.8 & 10.89 & 0141$-$0054888 & $-$36.0 & 8.0 & $+$14.0 & 15.0\\
  09161589$-$8045205 & 14.64 & 14.04 & 13.71 & J091616.6$-$804518 & 17.44 &  &  & 0092$-$0030513 & 0.0 & 0.0 & 0.0 & 0.0\\
  09181593$-$7527342 & 11.46 & 10.86 & 10.63 & J091815.9$-$752734 & 12.98 & 11.37 & 10.52 & 0145$-$0064601 & $-$96.0 & 9.0 & $+$126.0 & 11.0\\
  09211098$-$7455270 & 11.74 & 11.46 & 11.41 & J092111.2$-$745525 & 14.08 & 11.92 & 11.5 & 0150$-$0074388 & $+$2.2 & 6.0 & $-$2.8 & 6.0\\
  09212550$-$7915133 & 12.62 & 12.1 & 11.73 & J092125.5$-$791513 & 14.7 & 12.66 & 11.68 & 0107$-$0035021 & $-$52.0 & 13.0 & $+$40.0 & 10.0\\
  09241840$-$7954161 & 15.41 & 14.71 & 14.32 & J092418.3$-$795416 & 18.12 & 15.28 &  & 0100$-$0033465 & $+$63.1 & 9.0 & $-$272.8 & 9.0\\
  09332070$-$7433127 & 10.93 & 10.37 & 10.08 & J093320.6$-$743313 & 12.55 & 10.97 & 10.21 & 0154$-$0085970 & $-$14.0 & 11.0 & $+$34.0 & 6.0\\
  09361819$-$7442386 & 12.0 & 11.44 & 11.14 & J093618.2$-$744238 & 13.57 & 11.94 & 11.18 & 0152$-$0081294 & $-$66.0 & 5.0 & $+$62.0 & 12.0\\
  09405280$-$7638233 & 12.86 & 12.22 & 11.92 & J094052.9$-$763823 & 14.92 & 12.82 & 11.95 & 0133$-$0057137 & $-$32.0 & 22.0 & $+$92.0 & 11.0\\
  09424157$-$7727130 & 12.38 & 11.79 & 11.52 & J094241.5$-$772714 & 14.11 & 12.36 & 11.56 & 0125$-$0062122 & 0.0 & 0.0 & 0.0 & 0.0\\
  09451445$-$7753150 & 13.89 & 13.23 & 12.79 & J094514.5$-$775315 & 16.84 & 13.82 & 12.83 & 0121$-$0050831 & $-$32.0 & 47.0 & $+$168.0 & 28.0\\
  09460586$-$7605479 & 12.98 & 12.4 & 12.12 & J094605.8$-$760548 & 14.89 & 12.86 & 12.08 & 0139$-$0056858 & $-$2.0 & 30.0 & $+$196.0 & 34.0\\
  09475915$-$7925481 & 14.96 & 14.36 & 13.96 & J094759.4$-$792548 & 17.8 & 14.95 & 13.88 & 0105$-$0036743 & 0.0 & 0.0 & 0.0 & 0.0\\
  09512392$-$8259057 & 12.04 & 11.5 & 11.19 & J095124.1$-$825906 & 13.86 & 12.13 & 11.32 & 0070$-$0028766 & $-$36.0 & 3.0 & $+$40.0 & 4.0\\
  09533862$-$7929598 & 11.48 & 10.94 & 10.65 & J095338.7$-$792959 & 13.08 & 11.48 & 10.52 & 0105$-$0037380 & $-$38.4 & 6.1 & $+$43.1 & 6.2\\
  09545099$-$7729327 & 11.32 & 10.74 & 10.43 & J095451.0$-$772933 & 12.92 & 11.27 & 10.41 & 0125$-$0064071 & $-$23.4 & 6.2 & $+$31.3 & 6.4\\
  09552669$-$7712005 & 10.65 & 9.88 & 9.61 & J095526.6$-$771200 & 12.2 & 10.67 & 9.68 & 0127$-$0063645 & $+$2.0 & 6.0 & $+$2.6 & 6.0\\
  09553919$-$7622119 & 11.27 & 10.63 & 10.38 & J095539.2$-$762212 & 13.12 & 11.37 & 10.42 & 0136$-$0055631 & $-$28.3 & 6.4 & $+$3.2 & 6.3\\
  10044363$-$7726032 & 10.92 & 10.16 & 9.95 & J100443.6$-$772603 & 12.51 & 10.99 & 10.04 & 0125$-$0065381 & $-$5.2 & 6.0 & $+$11.2 & 6.0\\
  10111238$-$8106419 & 10.82 & 10.24 & 9.93 & J101111.9$-$810641 & 12.43 & 10.94 & 10.0 & 0088$-$0036255 & $+$116.0 & 0.0 & $-$244.0 & 1.0\\
  10140807$-$7636327 & 9.75 & 9.16 & 8.87 & J101408.1$-$763633 & 11.32 & 9.79 & 8.86 & 0133$-$0061544 & $-$47.5 & 6.0 & $+$20.9 & 6.2\\
  10251334$-$7828257 & 13.74 & 13.16 & 12.76 & J102513.3$-$782825 & 15.91 & 13.67 & 12.73 & 0115$-$0043578 & 0.0 & 0.0 & 0.0 & 0.0\\
  10261679$-$7755442 & 11.88 & 11.44 & 11.33 & J102616.7$-$775544 & 13.47 & 12.66 & 11.95 & 0120$-$0053042 & $-$44.0 & 12.0 & $+$34.0 & 10.0\\
  10261888$-$7750251 & 12.8 & 12.18 & 12.01 & J102618.8$-$775025 & 14.66 & 13.6 & 12.57 & 0121$-$0057040 & 0.0 & 6.0 & $+$8.7 & 6.0\\
  10265445$-$7800055 & 11.56 & 10.79 & 10.56 & J102654.4$-$780005 & 13.08 & 11.61 & 10.51 & 0119$-$0051062 & $-$11.0 & 6.1 & $+$9.5 & 6.1\\
  10265556$-$7848495 & 13.12 & 12.59 & 12.32 & J102655.5$-$784849 & 15.06 & 13.12 & 12.34 & 0111$-$0042350 & 0.0 & 0.0 & 0.0 & 0.0\\
  10283359$-$8115054 & 14.21 & 13.65 & 13.21 & J102833.7$-$811505 & 17.09 & 14.22 & 13.34 & 0087$-$0038156 & $-$188.0 & 3.0 & $+$122.0 & 15.0\\
  10291761$-$7952552 & 13.41 & 12.84 & 12.48 & J102917.6$-$795255 & 15.66 & 13.38 & 12.43 & 0101$-$0041251 & $+$8.0 & 0.0 & $-$62.0 & 25.0\\
  10294163$-$8020248 & 12.54 & 12.0 & 11.72 & J102941.6$-$802024 & 14.35 & 12.65 & 11.76 & 0096$-$0039873 & $-$74.0 & 6.0 & $+$62.0 & 6.0\\
  10311806$-$8117112 & 12.24 & 11.57 & 11.34 & J103118.0$-$811711 & 14.06 & 12.79 & 11.83 & 0087$-$0038391 & $-$27.5 & 9.0 & $+$4.3 & 9.0\\
\bottomrule[2pt]}


==> chapter2/chapter2.tex <==
\chapter{Hunting the Parent of the Orphan Stream I}
\label{chap:orphan_I}
% you can put a brief note at the top of your chapters using '\previouslypublished{}'. For example, to give a reference to the paper this chapter is based on, or to point out that it has been submitted to a journal.

\previouslypublished{Parts of this chapter have been previously published as \href{http://adsabs.harvard.edu/abs/2013ApJ...764...39C}{`Hunting the Parent of the Orphan Stream: Identifying Stream Members from Low-Resolution Spectroscopy', {Casey}, A.~R., {Da Costa}, G., {Keller}, S.~C., {Maunder}, E., 2013, ApJ, 764, 39C}. The work is presented here in expanded and updated form.} \\

We present candidate K-giant members in the Orphan stream which have been identified from low-resolution data taken with the AAOmega spectrograph on the Anglo-Australian Telescope. From modest $S/N$ spectra and independent cuts in photometry, kinematics, gravity and metallicity we yield self-consistent, highly probable stream members. We find a revised stream distance of $22.5\,\pm\,2.0$\,kpc near the celestial equator, and our kinematic signature peaks at $V_{GSR} = 82.1\,\pm\,1.4$\,km s$^{-1}$. The observed velocity dispersion of our most probable members is consistent with arising from the velocity uncertainties alone. This indicates that at least along this line-of-sight, the Orphan stream is kinematically cold. Our data indicates an overall stream metallicity of [Fe/H] $= -1.63\,\pm\,0.19$\,dex which is more metal-rich than previously found and unbiased by spectral type. Furthermore, the significant metallicity dispersion displayed by our most probable members, $\sigma(\mbox{[Fe/H]}) = 0.56$\,dex, suggests that the unidentified Orphan stream parent is a dSph satellite. We highlight likely members for high-resolution spectroscopic follow-up.

\section{Introduction}
\label{sec:ch2-introduction}

%The Milky Way stellar halo has partly formed through the accretion of satellites that are disrupted by tidal forces as they fall into the Galaxy's potential. Stars which were once gravitationally bound to the satellite are distributed along the progenitor's orbit in leading and trailing streams of stars. The velocities of stars in the stream are sensitive to the shape of the dark matter halo, allowing us to constrain the Milky Way potential and reconstruct the formation history of the Galaxy. The level of accreted substructure in the Milky Way has only recently become apparent through multi-band photometric surveys like the Sloan Digital Sky Survey (SDSS). The more prominent of the detectable substructures, like Sagittarius, have been well-studied. One of the more prominent \--- yet less studied \--- substructures is that of the Orphan stream. 

% could add a sentence to the paragraph above discussing the various substructures that have been detected

The Orphan stream was independently detected by both \citet{grillmair_2006} and \citet{belokurov;et-al_2006}, and is distinct from other substructures in the halo. The stream stretches over $60^\circ$ of arc on the sky, has a low surface brightness, and a narrow stream width of only $\sim$2$^\circ$. As the name suggests, the parent object largely remains a mystery. The stream extends past the celestial equator \--- outside the SDSS footprint \--- but has not been detected in existing southern surveys \citep{newberg;et-al_2010}. Whilst the parent system remains elusive, significant effort has been placed on associating the stream with known Milky Way satellites \citep{zucker;et-al_2006, fellhaur;et-al_2007,jin;lynden-bell_2007,sales;et-al_2008}. In contrast, there has been relatively limited observational work on the Orphan stream itself other than the original discovery papers \citep{grillmair_2006, belokurov;et-al_2006, belokurov;et-al_2007} and the work of \citet{newberg;et-al_2010}. This is largely to be expected given the absence of deep multi-band photometry in the southern sky, and the low total luminosity of the stream. This makes it difficult to reliably separate Orphan stream members from halo stars. Understanding the full extent of the stream awaits the SkyMapper and Pan-STARRS photometric surveys \citep{keller;et-al_2007, hodapp;et-al_2004}.

As \citet{sales;et-al_2008} point out, there is a natural observational bias towards more massive and recent mergers like Sagittarius. Consequently, the fainter end of this substructure distribution has yet to be fully recovered, or thoroughly examined. Interestingly, there are indications that  some fainter substructures like the Orphan stream and the Palomar 5 tidal tails \citep{odenkirchen;et-al_2009} have orbits which seem to be best-fit by Milky Way models with nearly 60\% less mass \citep{newberg;et-al_2010} than generally reported by \citet{xue;et-al_2008} and \citet{koposov;et-al_2010}. Such a discrepancy in the mass of the Milky Way is troublesome. More complete photometric and kinematic maps of these low total luminosity streams may provide the best test as to whether this mass discrepancy is real, or an artefact of incomplete observations. Whilst the full spatial extent of the Orphan stream remains unknown, we can examine the detailed chemistry of its members, investigate the stream history, and make predictions about the nature of the progenitor.

In this chapter we present a detailed, self-consistent analysis to identify K-giant members of the Orphan stream. Using our selection method we have catalogued the locations of nine highly probable Orphan stream candidates, all worthy of high-resolution spectroscopic follow up. In the following section we outline our photometric target selection. In Section \ref{sec:ch2-observations} we describe the low-resolution spectroscopic observations. The data analysis, including stream identification, is discussed in Section \ref{sec:ch2-analysis} and in Section \ref{sec:ch2-conclusions} the conclusions, predictions and future work are presented.


\section{Target Selection}
\label{sec:ch2-target-selection}

We have targeted K-giant members of the Orphan stream in order to investigate their detailed chemistry. Because K-giants are difficult to unambiguously detect from photometry alone, low-resolution spectroscopy is required to estimate stellar parameters and determine radial velocities. The Orphan stream has an extremely low spatial over-density, which makes it difficult to separate stream members from halo stars. However, there is a well described distance gradient along the stream \citep{belokurov;et-al_2007, newberg;et-al_2010} which provides an indication on where we should focus our spectroscopic efforts.

The Orphan stream is closest to us in two locations on the edge of the SDSS footprint: at the celestial equator \citep{belokurov;et-al_2007}, and along outrigger SEGUE Stripe 1540 \citep{newberg;et-al_2010}. These two locations are unequivocally the best place to recover bright stream members. Two fields centered on $(\alpha, \delta) =$ (10:48:15, 00:00:00) and (10:48:15, $-$02:30:00) have been targeted, and a combination of colour cuts with the SDSS DR 7 \citep{abazajian;et-al_2009} have been employed to identify likely K-giants:
\begin{eqnarray}
0.6 <& (g-i)_0 &< 1.7 \\
-15(g-i)_0 + 27 <& g_0 &< -3.75(g-i)_0 + 22.5 \\
15  <& i_0  &< 18 
\end{eqnarray}

Given our colour selection we expect to recover giants and contaminating dwarfs. Although the 2MASS $JHK$ colours can help to separate dwarfs and giants, our target K-giants stars are too faint to be detected in the 2MASS catalogue.

\section{Observations}
\label{sec:ch2-observations}

Observations took place on the Anglo-Australian Telescope using the AAOmega spectrograph in April 2009. AAOmega is a fibre-fed, dual beam multi-object spectrograph which is capable of simultaneously observing spectra of 392 (science and sky) targets across a $2\,^\circ$ field of view. We used the 570\,nm dichroic in combination with the 1000I grating in the red arm, and the 580V grating in the blue arm. This provides a spectral coverage between $800 \leq \lambda \leq 950$\,nm in the red at $\mathcal{R} \approx 4400$, and between $370 \leq \lambda \leq 580$\,nm with a lower spectral resolution of $\mathcal{R} \approx 1300$ in the blue.

The data were reduced using the standard 2DFDR reduction pipeline\footnote{http://www.aao.gov.au/2df/aaomega/aaomega\_2dfdr.html}. After flat-fielding, throughput calibration for each fibre was achieved using the intensity of skylines in each fibre. The median flux of dedicated sky fibres was used for sky subtraction, and wavelength calibration was performed using Th-Ar arc lamp exposures taken between science frames. Three thirty minute science exposures were median-combined to assist with cosmic ray removal. The median $S/N$ obtained in the red arm for our fields is modest at 35 per pixel, although this deteriorates quickly for our fainter targets. With the presence of strong Ca\,II triplet lines in the red arm, we are able to ascertain reliable radial velocities and reasonable estimates on overall metallicity \citep[][and references therein]{starkenburg;et-al_2010}. Our spectral region also includes gravity-sensitive magnesium lines: Mg\,I at 880.7\,nm, and the Mg\,I\,b 3$p$-4$s$ triplet lines at $\sim$517.8\,nm. These lines are sufficient to discriminate dwarfs from giants even with weak signal.

The blue and red arm spectra were normalised using a third order cubic spline after multiple iterations of outlier clipping. We used defined knot spacings of 20\,nm in the red arm, and 5\,nm in the blue arm in order to accommodate often poor $S/N$, and varying strengths of molecular band-heads.

\section{Analysis \& Discussion}
\label{sec:ch2-analysis}

We have employed a combination of separate criteria to identify likely Orphan stream members: kinematics, a giant/dwarf indication from Mg\,I lines, and selecting stars with consistent metallicities derived from both isochrone fitting and the strength of the Ca\,II triplet lines. Each criteria is discussed here separately.

\subsection{Kinematics}
Radial velocities were measured by cross-correlating our normalised spectra against a synthetic spectrum of a metal-poor giant across the spectral range $845 \leq \lambda \leq 870$\,nm. Heliocentric velocities were translated to the galactic rest frame by adopting the LSR velocity as 220\,km s$^{-1}$ towards $(l, b) = (53\,^\circ, 25\,^\circ)$ \citep{kerr;lynden-bell_1986, mihalas;binney_1981}\footnote{Where $V_{GSR} = V_{HELIO} + 220\sin{l}\cos{b} + 16.5\times[\sin{b}\sin{25^\circ} + \cos{b}\cos{25^\circ}\cos{(l - 53^\circ)}]$}.

Figure \ref{fig:ch2-velocities} shows a histogram of our galactocentric velocities, compared to the predicted smooth line-of-sight velocity distribution for this region from the Besan\c{c}on model \citep{robin;et-al_2003}. We have selected particles from the Besan\c{c}on model using the same criteria outlined in Section \ref{sec:ch2-target-selection} after employing the \citet{jordi;et-al_2006} colour transformations. It is clear that our target selection has yielded mostly nearby disk dwarf stars with $V_{GSR} \approx -120$\,km\,s$^{-1}$.

\begin{figure}[h]
	\includegraphics[width=\columnwidth]{./chapter2/fig1.pdf}
	\caption[Predicted and observed galactocentric rest frame velocities]{Galactocentric rest frame velocities for stars in both our observed fields (grey), and predicted Besan\c{c}on velocities which have been scaled to match our observed sample size. The expected kinematic signature from \citet{newberg;et-al_2010} for the Orphan stream is highlighted, as is our kinematic selection window (green).}
	\label{fig:ch2-velocities}
\end{figure}
 

In a nearby ($\Delta\Lambda_{Orphan} \sim 4^\circ$) region of the stream, \citet{newberg;et-al_2010} detected the Orphan stream with a $V_{GSR} = 101.4$\,km s$^{-1}$ from BHB stars. Differences in accounting for the local standard of rest between this work and \citet{newberg;et-al_2010} means that this corresponds to approximately 95\,km s$^{-1}$ on our $V_{GSR}$ scale.  This is discussed further in Section \ref{sec:ch2-newberg}. The expected Orphan stream kinematic peak is labelled in Figure \ref{fig:ch2-velocities}. There is no obvious sharp kinematic peak representative of the Orphan stream in our sample. From kinematics alone, our targets appears largely indistinguishable from a smooth halo distribution. To isolate potential Orphan stream members we have nominated a relatively wide selection criteria between $65 \leq V_{GSR} \leq 125$\,km s$^{-1}$ (shown in Figure \ref{fig:ch2-velocities}), which yields 28 Orphan stream candidates. The typical uncertainty in our velocities is $\pm{}5.0$\,km s$^{-1}$.

\subsection{Dwarf/Giant Discrimination}
\label{sec:ch2-dwarf-giant}

We have measured the EW of the gravity-sensitive Mg\,I line at 880.7\,nm to distinguish dwarfs from giants \citep{battaglia;starkenburg_2012}. At a given temperature (or $g - r$) and metallicity, giant stars present narrower Mg\,I absorption lines than their dwarf counterparts. Given the target selection, our sample is likely to contain many more dwarfs than giants. In some cases no Mg\,I 880.7\,nm line was apparent, so an upper limit was estimated based on the $S/N$ of the spectra. In these cases the candidate was considered a ``non-dwarf" because we cannot exclusively rule out a metal-poor sub-giant with this criteria alone. For these purposes we are only looking for a simple indication as to whether a star is likely a dwarf or not. 

Figure \ref{fig:ch2-ew-mg} illustrates the trend with $EW_{\lambda880.7}$ against SDSS de-reddened\footnote{All magnitudes presented in this chapter are de-reddened using the \citet{schlegel;et-al_1998} dust maps.} $g - r$, illustrating the dominant upper dwarf branch we wish to exclude. Giant stars populate the lower, sparser branch. A separation line has been adopted to distinguish dwarfs from giants, and is shown in Figure \ref{fig:ch2-ew-mg}. If we were to place this line higher, the total number of true giant stars may increase, but the dwarf contamination rate will rise dramatically. A compromise must be made between the rate of giant recoverability and the dwarf contamination. Our dwarf/giant separation line lies just below the main dwarf population. On its own, this dwarf/giant separation line would typically result in far too many dwarf contaminants. However, we are  employing selections on multiple observables (kinematics, metallicity, proper motions) in order to refine our Orphan stream giant sample. 

\begin{figure}[h]
	\includegraphics[width=\columnwidth]{./chapter2/fig2.pdf}
	\caption[Dwarf/giant discriminant based on EW of the $\lambda$8807 Mg\,I transition]{SDSS $g - r$ against the measured EW of the Mg\,I transition at 880.7\,nm. Dwarf contaminants occupy the more populous upper branch. Our separation line between dwarfs and giants is shown in green.}
	\label{fig:ch2-ew-mg}
\end{figure}

This dwarf/giant separation method was also employed using the total EW of the Mg\,I\,b triplet lines. Both analyses were entirely consistent with each other: essentially the same candidate list was found using both techniques. However, given slightly poorer signal at the Mg\,I\,b triplet, we were forced to adopt many more upper limits than when the 880.7\,nm line was employed. Because we classify all upper limits as being ``non-dwarfs" (i.e., potential giants), we deduced a slightly larger candidate sample for the Mg\,I\,b analysis, which was primarily populated by upper limits. In conclusion, we found the Mg\,I line at 880.7\,nm appeared to be a more consistent dwarf discriminant given our weak $S/N$ \--- particularly for our fainter stars. Thus, we have used the 880.7\,nm Mg\,I selection throughout the rest of our analysis.

The adopted dwarf/giant separation line shown in Figure \ref{fig:ch2-ew-mg} yields 425 potential giants. Upon taking the intersection of our kinematic and gravity selections, we find 20 stars that appear to be likely Orphan stream giants.


\subsection{Metallicities}
\label{sec:ch2-metallicities}

We have measured the metallicities for the stars that meet our kinematic and surface gravity criteria in two ways: with the strength of their Ca\,II triplet lines, and by isochrone-fitting. After correcting for luminosity, the EW of the Ca\,II triplet lines provide a good indication of the overall metallicity of a RGB star \citep{armandroff;da_costa_1991}. We have employed the \citet{starkenburg;et-al_2010} relationship and corrected for luminosity in $g$ against the horizontal branch magnitude at $g_{HB}$ = 17.1 \citep{newberg;et-al_2010}. Strictly speaking, the Ca\,II\---[Fe/H] calibration is only valid for stars brighter than the horizontal branch, although the relationship only becomes significantly inappropriate near $g \-- g_{HB} \sim +1$ \citep{saviane;et-al_2012}. Many of our candidates are fainter than this valid luminosity range, and therefore they should not be excluded solely because of their derived metallicities, as these could be uncertain. Stars fainter than $g_{HB}$ will have slightly lower metallicities than predicted by our Ca\,II\---[Fe/H] relationship, and for these stars we will only use metallicities to assign a relative qualitative likelihood for stream membership.

Given a distance estimate to the Orphan stream, we can also deduce a star's metallicity through isochrone fitting. We have used a 10\,Gyr \citet{girardi;et-al_2004} isochrone at 21.4\,kpc \citep{newberg;et-al_2010} and found metallicities for all 20 likely stream members from their best-fitting isochrone. Derived metallicities from Ca\,II line strengths and isochrone fitting that are consistent (within $\pm0.3$\,dex) indicates these measurements are reliable, and that these stars are indeed at a distance of $\sim$21.4\,kpc. We find 10 highly likely stream members with consistently derived metallicities. They fall within the shaded region illustrated in Figure \ref{fig:ch2-feh}. 

\begin{figure}[t!]
	\includegraphics[width=\columnwidth]{./chapter2/fig3.pdf}
	\caption[Metallicities of Orphan stream candidates from isochrone fitting and Ca\,II triplet lines]{Metallicities from the Ca\,II triplet lines versus those found from fitting isochrones to the 20 stars that meet our kinematic and surface gravity criteria. Both abundance determinations imply these stars are RGB members of the Orphan stream at a distance of $\sim$21.4\,kpc \citep{newberg;et-al_2010}. Consistency between these methods indicates highly likely stream membership (shaded region). The minimum isochrone [Fe/H], and a representative uncertainty of 0.2\,dex for abundance measurements is shown.}
	\label{fig:ch2-feh}
\end{figure}

\begin{figure}[t!]
	\includegraphics[width=\columnwidth]{./chapter2/fig4.pdf}
	\caption[Color magnitude diagram of observed stars, where Orphan stream candidates are highlighted]{Color magnitude diagram showing our observed candidates (grey). Observations fulfilling kinematic and gravity cuts are colored by their metallicity, and those with upper limits for surface gravity are marked as triangles ($\triangledown$). Highly probable stream members (see text) are circled. Relevant 10\,Gyr \citet{girardi;et-al_2004} isochrones at $[\mbox{Fe/H}] = -1.5$ (dotted), $-2.0$ (dashed) at 21.4\,kpc \citep{newberg;et-al_2010} are shown, as well as our best-fitting 10\,Gyr isochrone of $[\mbox{Fe/H}] = -1.63$ at 22.5\,kpc (solid).}
	\label{fig:ch2-cmd}
\end{figure}

A final metallicity value for each star has been adopted based on the quality of our [Fe/H] measurements. These values are tabulated in Table \ref{tab:oss-members}. From our highly likely stream members we find an overall stream metallicity of $[\mbox{Fe/H}] = -1.63$ with a dispersion of $\sigma({\rm [Fe/H]}) = 0.56$\,dex. This abundance spread is larger than typically seen in globular cluster stars and is more representative of the chemical spread seen in dSph satellites.


\begin{table}[h!]
\centering
\caption{Identified Orphan stream candidates from low-resolution spectra\label{tab:oss-members}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccrcrcrrccccc}
\hline
\hline
Star & $\alpha$ & $\delta$ & $g$ & $g - r$ & \multicolumn{2}{c}{$\mu_\alpha$} & \multicolumn{2}{c}{$\mu_\delta$} & \multicolumn{2}{c}{$V_{GSR}$} & $EW_{\lambda8807}$ & [Fe/H]$_{Ca}$ & [Fe/H]$_{iso}$ & [Fe/H]\footnote{Final adopted [Fe/H] value based on quality of two metallicity measurements.} & Stream \\
Name & (J2000) & (J2000) & & & \multicolumn{2}{c}{(mas yr$^{-1}$)} & \multicolumn{2}{c}{(mas yr$^{-1}$)} & \multicolumn{2}{c}{(km s$^{-1}$)} & (m\AA{}) & (dex) & (dex) & (dex) & Prob. \\
\hline
OSS 1  & 10:46:21.9 & $+$00:43:21.8 & 17.52 & 0.50 & 4.1&$\pm$ 4.5 & $-$34.0 &$\pm$ 4.5 & 73.3 &$\pm$ \phn9.3 & 0.273 & --1.78 &$<$--2.28\phn\,& --1.78 & Low \\
OSS 2  & 10:46:29.3 & $-$00:19:38.5 & 17.77 & 0.56 & $-$1.7 &$\pm$ 4.3 & $-$2.2 &$\pm$ 4.3 & 78.4 &$\pm$ \phn5.2 & 0.126 & --1.63 & --1.68  & --1.63 & High \\
OSS 3  & 10:46:50.4 & $-$00:13:15.6 & 17.33 & 0.51 & 1.8 &$\pm$ 4.3 & $-$4.6 &$\pm$ 4.3 & 77.0 &$\pm$ \phn4.0 & 0.416 & --1.31 &$<$--2.28\phn\,& --1.31 & Low \\
OSS 4  & 10:47:06.1 & $-$01:56:03.9 & 18.74 & 0.54 & $-$6.3 &$\pm$ 4.9 & 4.6 &$\pm$ 4.9 & 74.9 &$\pm$    17.6 & 0.452 &:--1.12\footnote{Sufficiently fainter than $g_{HB}$ to qualify this measurement as uncertain.}& --1.40  & --1.40 & High \\
OSS 5  & 10:47:15.0 & $-$03:15:03.9 & 18.66 & 0.54 & $-$8.2 &$\pm$ 5.2 & 1.7 &$\pm$ 5.2 & 109.5 &$\pm$ \phn9.0 &$<$0.19&:--1.85\textsuperscript{b}& --1.43  & --1.43 & Medium \\
OSS 6  & 10:47:17.6 & $+$00:25:07.7 & 16.09 & 0.72 & $-$0.8 &$\pm$ 4.0 & $-$5.2 &$\pm$ 4.2 & 79.2 &$\pm$ \phn3.3 & 0.212 & --1.84 & --1.80  & --1.84 & High \\
OSS 7  & 10:47:29.1 & $-$02:02:22.6 & 17.86 & 0.47 & \multicolumn{2}{c}{\nodata} & \multicolumn{2}{c}{\nodata}  & 93.2 &$\pm$    29.8 &$<$0.40& --2.82 &$<$--2.28\phn\,& --2.82 & High \\
OSS 8  & 10:47:30.1 & $-$00:01:24.5 & 17.25 & 0.61 & $-$4.0 &$\pm$ 4.2 & $-$5.2 &$\pm$ 4.2 & 83.6 &$\pm$ \phn3.5 & 0.123 & --1.62 & --1.68  & --1.62 & High \\
OSS 9  & 10:48:20.9 & $+$00:26:34.4 & 17.88 & 0.55 & $-$8.1 &$\pm$ 4.3 & $-$5.4 &$\pm$ 4.3 & 118.9 &$\pm$    11.7 & 0.467 & --1.65 & --1.73  & --1.65 & High \\
OSS 10 & 10:48:27.8 & $+$00:55:24.0 & 17.72 & 0.51 & $-$14.4 &$\pm$ 4.6 & $-$5.3 &$\pm$ 4.6 & 124.5 &$\pm$ \phn6.7 & 0.182 & --1.48 &$<$--2.28\phn\,& --1.48 & Low \\
OSS 11 & 10:48:31.9 & $+$00:03:35.7 & 17.02 & 0.58 & $-$3.6 &$\pm$ 4.1 & $-$7.7 &$\pm$ 4.1  & 105.1 &$\pm$ \phn5.1 & 0.234 & --1.12 & --2.10  & --1.12 & Low \\
OSS 12 & 10:48:44.4 & $-$02:53:08.8 & 18.35 & 0.62 & $-$3.4 &$\pm$ 4.7 & $-$1.8 &$\pm$ 4.7 & 108.2 &$\pm$ \phn9.0 & 0.183 &:--1.01\textsuperscript{b}& --1.17  & --1.17 & High \\
OSS 13 & 10:48:46.9 & $-$00:32:27.8 & 17.85 & 0.46 & $-$28.4 &$\pm$ 4.8 & $-$12.3 &$\pm$ 4.8 & 109.3 &$\pm$ \phn8.1 & 0.324 & --2.37 &$<$--2.28\phn\,& --2.37 & Medium \\
OSS 14 & 10:49:08.3 & $+$00:02:00.2 & 16.27 & 0.62 & 4.9 &$\pm$ 4.0 & $-$6.0 &$\pm$ 4.0& 81.5 &$\pm$ \phn4.6 & 0.034 & --2.70 &$<$--2.28\phn\,& --2.70 & High \\
OSS 15 & 10:49:13.4 & $+$00:04:03.8 & 17.83 & 0.46 & 3.4 &$\pm$ 4.7 & $-$6.8 &$\pm$ 4.7 & 65.3 &$\pm$ \phn5.4 & 0.252 & --1.74 & $<$--2.28\phn\,& --1.74 & Medium \\
OSS 16 & 10:50:13.1 & $+$00:33:52.7 & 16.13 & 0.58 & $-$3.4 &$\pm$ 4.0 & $-$7.7 &$\pm$ 4.0 & 94.7 &$\pm$ \phn5.1 & 0.391 & --1.54 &$<$--2.28\phn\,& --1.54 & Low \\
OSS 17 & 10:50:24.2 & $-$01:49:05.4 & 17.94 & 0.54 & 3.4 &$\pm$ 4.6 & $-$2.2 &$\pm$ 4.6 & 109.9 &$\pm$    25.4 & 0.151 & --1.06 & --1.73  & --1.06 & Low \\
OSS 18 & 10:50:33.8 & $+$00:12:19.1 & 17.82 & 0.60 & $-$7.4 &$\pm$ 5.0 & $-$3.3 &$\pm$ 5.0 & 97.5 &$\pm$ \phn5.9 & 0.596 & --0.90 & --1.43  & --0.90 & Medium \\
OSS 19 & 10:51:19.7 & $+$00:05:15.5 & 17.81 & 0.65 & 4.2 &$\pm$ 4.7 & $-$11.8 &$\pm$ 4.7 & 82.7 &$\pm$ \phn5.0 & 0.198 & --1.16 & --1.20  & --1.16 & High \\
OSS 20 & 10:51:35.4 & $+$00:00:46.4 & 17.93 & 0.56 & --0.5 &$\pm$ 4.5 & $-$3.0 &$\pm$ 4.5 & 66.7 &$\pm$ \phn8.7 & 0.128 & :--1.38 & --2.10 & --2.10 & Medium \\
\hline
\end{tabular}}
\end{table}



\break
\subsection{Proper Motions \& Distances}

We have found proper motions for 19 of our candidates in the PPMXL proper motion catalogue \citep{roeser;et-al_2010}. One highly probably candidate (OSS 13 in Table \ref{tab:oss-members}) has a listed proper motion that is different from that of the other nine highly likely members at the $6\sigma$ level. Consequently, we have reduced the membership likelihood of this star from ``High" to ``Medium". Given the uncertainties in proper motions, we cannot reliably alter the membership probability for any other candidate.

Since our Orphan stream giants cover a wide evolutionary range along the giant branch (Figure \ref{fig:ch2-cmd}), we are in a good position to revise the distance estimate to the stream. Given a 10\,Gyr \citet{girardi;et-al_2004} isochrone at $[\mbox{Fe/H}] = -1.63$, we find a best-fitting distance to the stream of $22.5 \pm 2.0$\,kpc at $(l, b) = (250^\circ,\,50^\circ)$. This isochrone is shown in Figure \ref{fig:ch2-cmd}. Our derived distance is in reasonably good agreement with the measurement of $21.4 \pm 1.0$\,kpc independently deduced by \citet{grillmair_2006} and \citet{newberg;et-al_2010}.


\subsection{Comparison with \citet{newberg;et-al_2010}}
\label{sec:ch2-newberg}
\citet{newberg;et-al_2010} traced the Orphan stream using BHB stars selected from the SEGUE survey, allowing them to derive an orbit for the stream and make a strong prediction for the location of the undiscovered progenitor. Their closest stream detection to this study is at $\Lambda_{Orphan} = 18.4^\circ$, approximately $\Delta\Lambda_{Orphan} \sim 4^\circ$ away from our fields. At this location, \citet{newberg;et-al_2010} found the velocity of the stream to be $V_{GSR} = 101.4 \pm 8.9$\,km s$^{-1}$ based on 12 BHB stars. We note that this is $\sim95$\,km s$^{-1}$ on our scale, given the differences in accounting for the local standard of rest. The velocities and metallicities of our `High' and `Medium' probability candidates are illustrated in Figure \ref{fig:ch2-vgsr-feh}. Although we recover some candidates with velocities up to $V_{GSR} \sim 110$\,km s$^{-1}$, our kinematic distribution peaks near $V_{GSR} \sim 85$\,km s$^{-1}$, roughly 10\,km s$^{-1}$ lower than that of \citet{newberg;et-al_2010}.

There is a known velocity gradient along the Orphan stream which can account for this discrepancy. As $\Lambda_{Orphan}$ increases towards the edge of the SDSS boundary, galactocentric velocity quickly decreases. For the Orphan stream detection in the outrigger SEGUE Strip 1540 at $\Lambda_{Orphan} = 36^\circ$, \citet{newberg;et-al_2010} find $V_{GSR} = 38$\,km s$^{-1}$. This work presents likely Orphan stream K-giant candidates at $\Lambda_{Orphan} \sim 23^\circ$. Given the velocity gradient reported by \citet{newberg;et-al_2010}, a galactocentric velocity of $80-85$\,km s$^{-1}$ (on our scale) is perfectly reasonable. We note that since the velocities of BHB stars can have significant uncertainties, it was practical for us to assume a wide initial selection in kinematics to identify potential members. 

\begin{figure}[h!]
	\includegraphics[width=\columnwidth]{./chapter2/fig5.pdf}
	\caption[Galactocentric velocities and adopted metallicities for Orphan stream candidates]{Galactocentric velocities and adopted metallicities for the highest likely Orphan stream members (black $\bullet$), and those with probabilities assigned as ``Medium'' (grey $\circ$; see text).}
	\label{fig:ch2-vgsr-feh}
\end{figure}

\begin{figure}[h!]
	\includegraphics[width=\columnwidth]{./chapter2/fig6.pdf}
	\caption[Observed metallicity distribution for Orphan stream candidates]{Observed metallicity distribution function for the Orphan stream candidates identified here, with comparisons to the distribution found by \citet{newberg;et-al_2010} from BHB stars.}
	\label{fig:ch2-newberg-feh}
\end{figure}

The adopted metallicities of our Orphan stream candidates are generally higher than those found by \citet{newberg;et-al_2010}. Our highly likely stream members have a mean metallicity of [Fe/H] = $-1.63$, with a dispersion of $\sigma({\rm [Fe/H]}) = 0.56$\,dex. As illustrated in Figures \ref{fig:ch2-vgsr-feh} and \ref{fig:ch2-newberg-feh}, there are two very metal-poor candidates which largely drive this dispersion, but we have no reason to suspect they are non-members. The \citet{newberg;et-al_2010} sample contains 37 BHB stars identified over a 60$^\circ$ arc on the sky, and has a peak metallicity at [Fe/H] = $-2.10 \pm 0.10$. The closest detection bin in the \citet{newberg;et-al_2010} sample was the most populous, yielding 7 BHB stars. For comparison, we identify 9 giant stars across $\sim{}4^\circ$. Given BHB stars are known to trace a somewhat more metal-poor population, and we are calculating statistics with marginal sample sizes, we conclude that the accuracy of these two metallicity distributions are not mutually exclusive. It is entirely possible that we are sampling the same distribution, but a larger sample size is required.


\section{Conclusions}
\label{sec:ch2-conclusions}

We have presented a detailed analysis to isolate individual Orphan stream K-giants from low-resolution spectroscopy using a combination of photometric, kinematic, gravity, metallicity, and proper motion information. Although each individual criterion is likely to induce some level of contamination, their intersection reveals nine highly probable, self-consistent, Orphan stream K-giants.  We deduce a median stream metallicity of $[\mbox{Fe/H}] = -1.63 \pm 0.19$ and find an intrinsically wide metallicity spread of $\sigma({\rm [Fe/H]}) = 0.56$\,dex, indicative of a dSph origin. Unlike other stellar tracers, K-type giants can exist at all metallicities, hence our derived metallicity spread is likely representative of the true stream MDF. Recall that the metallicity determination was performed after kinematic and gravity cuts, and three of our most probable members lay perfectly on a 10\,Gyr isochrone of $[\mbox{Fe/H}] = -1.63$. However, it is clear that more data are required to fully characterize the stream metallicity distribution function. Our data indicate a distance to the stream of $22.5 \pm 2.0$\,kpc at $(l, b) = (250^\circ,\,50^\circ)$, in agreement with that deduced by \citet{grillmair_2006} and \citet{newberg;et-al_2010}.

Given the stream orbit derived by \citet{newberg;et-al_2010}, they excluded all possible known halo objects except for the dissolved star cluster, Segue 1. \citet{simon;et-al_2011} obtained spectroscopy for six members in Segue 1 and found an extremely wide metallicity dispersion: from [Fe/H] $<-3.4$ to $-1.63$ dex. On the basis of the extremely low metallicity in the cluster and the wide chemical dispersion, they conclude that Segue 1 is a dwarf spheroidal galaxy. Although the data presented here indicates the Orphan stream progenitor is a disrupted dwarf spheroidal galaxy, we cannot reliably associate Segue 1 as the parent without additional observational data. 

If the Orphan stream continues through SEGUE Stripe 1540 at $(l, b) = (271^\circ,\,38^\circ)$ as \citet{newberg;et-al_2010} found, then the stream is even closer there than in the region analysed here. Thus, if our observations and analyses are repeated at $(271^\circ,\,38^\circ)$, we predict K-giant stream members of brighter apparent magnitude will be recovered. 

Using a maximum-likelihood estimation we find the stream velocity at $(l, b) = (250^\circ, 50^\circ)$ from nine stars to be $V_{GSR} = 85.3 \pm 4.4$\,km s$^{-1}$ and the dispersion to be $6.5 \pm 7.0$\,km s$^{-1}$. If we exclude three stars with low $S/N$ ratios \--- and hence large ($> 10$\,km s$^{-1}$) velocity uncertainties \--- the peak occurs at $82.1 \pm 1.4$\,km s$^{-1}$ and the intrinsic dispersion is found to be {$0.2\,\pm\,3.1$\,km s$^{-1}$}. Hence, the observed stream dispersion is dominated by the velocity uncertainties, indicating that the intrinsic dispersion is small. 

The K-giants presented here can provide great insight into the chemistry and history of the Orphan stream. High-resolution spectra have been obtained for some targets, and a detailed chemical analysis is presented in Chapter \ref{chap:orphan_II}. Individual chemical abundances can help determine both the nature of the progenitor before it is discovered, and allows us to compare peculiar chemical signatures with those of the known Milky Way satellites in order to associate likely parents. However, at least for the moment, the Orphan stream remains appropriately named.



==> chapter4/equivalent_widths_table.tex <==
\setlength\tabcolsep{2pt}
\begin{landscape}
\begin{center}
\begin{longtable}{cccrcccccccccccc}
\label{tab:equivalent-widths}\\
\hline
\hline
Wavelength & Species & $\chi$ & $\log{gf}$ & HD 41667 & HD 44007 & HD 76932 & HD 122563 & HD 136316 & HD 141531 & HD 142948 & OSS 3 & OSS 6 & OSS 8 & OSS 14 & OSS 18 \\
({\AA}) & & (eV) & & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) \\
\hline
% This works.
\endfirsthead
\hline
Wavelength & Species & $\chi$ & $\log{gf}$ & HD 41667 & HD 44007 & HD 76932 & HD 122563 & HD 136316 & HD 141531 & HD 142948 & OSS 3 & OSS 6 & OSS 8 & OSS 14 & OSS 18 \\
({\AA}) & & (eV) & & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) & (m{\AA}) \\
\hline
\endhead
\hline
\multicolumn{16}{r}{Continued..}
\endfoot
\endlastfoot

 6300.300 &       O I &      0.00 &   $-$9.72 &   \nodata &     14.79 &   \nodata &      6.77 &   \nodata &     38.16 &     35.37 &   \nodata &      9.72 &   \nodata &   \nodata &   \nodata \\
 6363.780 &       O I &      0.02 &  $-$10.19 &     11.35 &   \nodata &   \nodata &   \nodata &     11.58 &     14.74 &     12.70 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5688.190 &      Na I &      2.11 &   $-$0.42 &     71.85 &     30.87 &     57.44 &   \nodata &     29.30 &     38.07 &   \nodata &     55.17 &     24.02 &     20.39 &   \nodata &     71.19 \\
 6154.230 &      Na I &      2.10 &   $-$1.53 &     10.66 &   \nodata &      7.75 &   \nodata &   \nodata &      5.23 &     28.38 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6160.750 &      Na I &      2.10 &   $-$1.23 &     16.55 &   \nodata &     13.38 &   \nodata &      4.58 &      6.98 &     43.40 &     17.39 &   \nodata &   \nodata &   \nodata &   \nodata \\
 3829.355 &      Mg I &      2.71 &   $-$0.21 &   \nodata &   \nodata &   \nodata &    190.12 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    162.57 &   \nodata \\
 3832.304 &      Mg I &      2.71 &      0.27 &   \nodata &   \nodata &   \nodata &    226.99 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    186.18 &   \nodata \\
%3838.292 &      Mg I &      2.72 &      0.49 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 3986.753 &      Mg I &      4.35 &   $-$1.03 &   \nodata &   \nodata &    132.19 &     34.70 &   \nodata &    116.98 &    181.70 &    104.81 &   \nodata &     93.49 &   \nodata &   \nodata \\
 4057.505 &      Mg I &      4.35 &   $-$0.89 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     45.65 &   \nodata \\
 4167.271 &      Mg I &      4.35 &   $-$0.71 &   \nodata &   \nodata &    157.13 &     53.07 &   \nodata &   \nodata &   \nodata &    145.01 &    108.01 &   \nodata &     55.47 &   \nodata \\
%4351.906 &      Mg I &      4.34 &   $-$0.53 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4571.096 &      Mg I &      0.00 &   $-$5.69 &    158.23 &    111.98 &     77.02 &     84.81 &    151.37 &    164.28 &    166.85 &    101.03 &    119.76 &    106.48 &     76.80 &    137.94 \\
 4702.990 &      Mg I &      4.33 &   $-$0.38 &    169.81 &    130.63 &    171.47 &     73.48 &    135.89 &    150.68 &   \nodata &    166.89 &    121.62 &    122.62 &     77.06 &    187.66 \\
 5167.321 &      Mg I &      2.71 &   $-$1.03 &   \nodata &   \nodata &   \nodata &   \nodata &    393.66 &    432.44 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5172.684 &      Mg I &      2.71 &   $-$0.45 &   \nodata &   \nodata &   \nodata &    209.21 &    359.74 &    421.31 &   \nodata &   \nodata &    285.70 &    309.40 &    219.80 &   \nodata \\
 5183.604 &      Mg I &      2.72 &   $-$0.24 &   \nodata &   \nodata &   \nodata &    239.06 &   \nodata &   \nodata &   \nodata &   \nodata &    362.50 &    368.74 &    220.89 &   \nodata \\
 5711.090 &      Mg I &      4.34 &   $-$1.72 &     94.16 &     53.77 &     64.46 &   \nodata &     58.12 &     79.05 &    114.39 &     68.72 &     38.26 &     32.39 &   \nodata &     73.16 \\
 6318.720 &      Mg I &      5.11 &   $-$1.97 &     27.26 &      9.58 &     19.64 &   \nodata &      9.99 &     11.19 &     50.77 &   \nodata &   \nodata &   \nodata &   \nodata &     35.56 \\
 6319.240 &      Mg I &      5.11 &   $-$2.22 &     19.33 &   \nodata &     13.34 &   \nodata &      7.69 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6965.410 &      Mg I &      5.75 &   $-$1.51 &     19.31 &   \nodata &      7.98 &   \nodata &   \nodata &     10.57 &     35.10 &   \nodata &   \nodata &   \nodata &   \nodata &     31.45 \\
 7387.690 &      Mg I &      5.75 &   $-$0.87 &     33.72 &     20.37 &   \nodata &   \nodata &     10.18 &     16.65 &     59.67 &     27.19 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6696.020 &      Al I &      3.14 &   $-$1.34 &     25.35 &   \nodata &      9.27 &   \nodata &   \nodata &     10.25 &     53.52 &   \nodata &      8.42 &   \nodata &   \nodata &   \nodata \\
 6698.670 &      Al I &      3.14 &   $-$1.64 &      7.93 &   \nodata &      4.38 &   \nodata &   \nodata &   \nodata &     27.54 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 7835.310 &      Al I &      4.02 &   $-$0.47 &     15.11 &   \nodata &     14.43 &   \nodata &   \nodata &   \nodata &     35.82 &     11.85 &   \nodata &   \nodata &   \nodata &   \nodata \\
 7836.130 &      Al I &      4.02 &   $-$0.31 &     19.37 &   \nodata &     19.11 &   \nodata &   \nodata &   \nodata &     48.54 &     10.56 &   \nodata &   \nodata &   \nodata &   \nodata \\
 3905.523 &      Si I &      1.91 &   $-$1.09 &   \nodata &   \nodata &   \nodata &    219.82 &   \nodata &   \nodata &   \nodata &   \nodata &    332.25 &   \nodata &    234.22 &   \nodata \\
 4102.936 &      Si I &      1.91 &   $-$3.14 &    159.40 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    123.42 &    119.00 &   \nodata &    101.44 &    125.45 \\
 5665.554 &      Si I &      4.90 &   $-$1.73 &     25.72 &   \nodata &     12.77 &   \nodata &     10.07 &     13.72 &     42.23 &     16.80 &   \nodata &   \nodata &   \nodata &     33.79 \\
 5690.430 &      Si I &      4.93 &   $-$1.75 &     33.03 &     14.58 &     20.53 &   \nodata &     15.01 &     21.30 &     54.82 &     23.80 &   \nodata &   \nodata &   \nodata &   \nodata \\
 5701.105 &      Si I &      4.93 &   $-$1.74 &   \nodata &   \nodata &     11.07 &   \nodata &   \nodata &   \nodata &     41.19 &   \nodata &   \nodata &      9.06 &   \nodata &   \nodata \\
 5708.397 &      Si I &      4.93 &   $-$1.47 &   \nodata &     33.29 &     41.04 &   \nodata &     39.59 &   \nodata &   \nodata &     38.95 &   \nodata &   \nodata &   \nodata &     78.38 \\
 5772.145 &      Si I &      5.06 &   $-$1.74 &     37.92 &     15.93 &     23.01 &   \nodata &     13.83 &     22.26 &     59.62 &     27.27 &   \nodata &   \nodata &   \nodata &     54.63 \\
 5793.070 &      Si I &      4.93 &   $-$1.84 &     28.46 &     10.81 &     17.23 &   \nodata &     11.16 &     13.61 &     46.48 &     17.02 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6125.020 &      Si I &      5.61 &   $-$1.51 &     13.50 &      5.51 &     12.37 &   \nodata &      7.98 &      8.94 &     28.23 &     10.48 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6145.010 &      Si I &      5.62 &   $-$1.36 &     20.39 &      8.50 &     13.14 &   \nodata &      7.07 &      9.69 &     37.91 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6155.130 &      Si I &      5.62 &   $-$0.79 &     45.49 &     22.58 &     37.42 &   \nodata &     18.83 &     28.65 &     71.82 &     42.56 &     13.34 &     20.80 &   \nodata &     43.74 \\
 7664.900 &       K I &      0.00 &      0.14 &    189.45 &    138.52 &    136.62 &   \nodata &    161.81 &    190.45 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 7698.960 &       K I &      0.00 &   $-$0.17 &    164.43 &    124.22 &    119.76 &     51.99 &    143.45 &    156.73 &    182.47 &    124.95 &    116.98 &    111.14 &     32.62 &    154.59 \\
 4283.010 &      Ca I &      1.89 &   $-$0.22 &   \nodata &   \nodata &    109.35 &   \nodata &   \nodata &   \nodata &   \nodata &    119.87 &    103.73 &   \nodata &     61.68 &   \nodata \\
 4318.650 &      Ca I &      1.89 &   $-$0.21 &    145.84 &   \nodata &     97.98 &     55.20 &    118.37 &    134.63 &   \nodata &    112.58 &   \nodata &   \nodata &     51.82 &   \nodata \\
 4425.440 &      Ca I &      1.88 &   $-$0.36 &    144.65 &    109.01 &    104.45 &     49.55 &   \nodata &    123.97 &    166.15 &    107.35 &     86.28 &    116.03 &     54.74 &    132.85 \\
 4435.690 &      Ca I &      1.89 &   $-$0.52 &   \nodata &   \nodata &     99.36 &     43.18 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     99.76 &     45.15 &   \nodata \\
 4454.780 &      Ca I &      1.90 &      0.26 &   \nodata &    140.19 &   \nodata &     80.27 &   \nodata &   \nodata &   \nodata &   \nodata &    138.04 &    128.98 &     78.12 &    208.55 \\
 4455.890 &      Ca I &      1.90 &   $-$0.53 &    139.51 &     95.14 &     94.80 &     40.66 &   \nodata &   \nodata &    151.57 &    116.17 &    102.23 &     89.49 &     43.65 &    128.66 \\
 5262.244 &      Ca I &      2.52 &   $-$0.47 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     29.72 &   \nodata \\
%5265.556 &      Ca I &      2.52 &   $-$0.26 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5349.465 &      Ca I &      2.71 &   $-$0.31 &     94.45 &     63.41 &     64.81 &     13.83 &     69.40 &     83.47 &    101.38 &     77.20 &     66.13 &     51.84 &   \nodata &     84.15 \\
 5581.971 &      Ca I &      2.52 &   $-$0.56 &     97.55 &     59.00 &     60.02 &     13.39 &     63.69 &     82.85 &    104.46 &     70.90 &     50.49 &     45.43 &   \nodata &    102.72 \\
 5588.760 &      Ca I &      2.52 &      0.21 &    140.55 &    102.78 &    107.67 &     50.00 &    115.34 &    130.21 &    144.74 &    117.06 &    109.15 &    104.76 &     39.14 &    141.34 \\
 5590.120 &      Ca I &      2.52 &   $-$0.57 &     96.00 &     56.06 &     58.38 &     15.87 &     63.78 &     80.32 &    103.34 &     68.21 &     45.66 &     52.98 &   \nodata &     91.73 \\
 5594.468 &      Ca I &      2.52 &      0.10 &   \nodata &   \nodata &    109.48 &     39.36 &    116.48 &   \nodata &   \nodata &   \nodata &    105.39 &     97.80 &     47.03 &   \nodata \\
 5598.487 &      Ca I &      2.52 &   $-$0.09 &   \nodata &   \nodata &   \nodata &     32.70 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     33.37 &   \nodata \\
 5601.285 &      Ca I &      2.53 &   $-$0.52 &    106.87 &     61.71 &     64.89 &     15.96 &     67.64 &     87.25 &    121.31 &     83.13 &     60.45 &     56.30 &     21.85 &    110.89 \\
 5857.450 &      Ca I &      2.93 &      0.23 &   \nodata &     83.89 &     94.26 &     26.70 &     91.80 &   \nodata &    136.73 &     87.35 &     87.52 &     78.50 &     30.36 &    113.55 \\
 6102.720 &      Ca I &      1.88 &   $-$0.79 &    140.31 &     96.95 &     90.77 &     42.88 &    115.38 &    133.09 &    141.08 &    116.51 &     98.10 &     97.07 &     42.04 &    132.26 \\
 6122.220 &      Ca I &      1.89 &   $-$0.32 &    168.67 &    124.69 &    123.31 &     74.10 &    145.57 &    158.98 &    175.56 &    139.07 &    130.75 &    123.80 &     60.95 &    186.58 \\
 6162.170 &      Ca I &      1.90 &   $-$0.09 &    186.95 &    136.58 &    141.15 &     88.99 &    161.71 &    175.05 &    197.81 &    163.47 &    140.17 &    135.91 &     74.11 &    195.81 \\
 6166.440 &      Ca I &      2.52 &   $-$1.14 &     73.04 &     30.11 &     31.62 &   \nodata &     36.05 &     51.15 &     76.39 &     45.70 &     30.36 &     22.51 &   \nodata &     73.51 \\
 6169.040 &      Ca I &      2.52 &   $-$0.80 &     89.51 &     48.47 &     51.35 &     10.36 &     54.49 &     72.50 &     96.37 &     67.20 &     46.72 &     46.99 &   \nodata &     91.73 \\
 6169.560 &      Ca I &      2.53 &   $-$0.48 &    109.49 &     66.40 &     69.73 &     18.47 &     73.02 &     93.05 &    114.55 &     90.61 &     67.38 &     62.99 &   \nodata &    117.51 \\
 6439.070 &      Ca I &      2.52 &      0.47 &    160.79 &    116.61 &    117.55 &     63.76 &    137.10 &    151.32 &    169.26 &    139.92 &    118.62 &    113.72 &     58.87 &    158.35 \\
 6449.810 &      Ca I &      2.52 &   $-$0.50 &    110.78 &     73.30 &     69.53 &   \nodata &     79.58 &     96.85 &    127.32 &     89.43 &   \nodata &     66.24 &   \nodata &    119.15 \\
 6455.600 &      Ca I &      2.52 &   $-$1.29 &     57.34 &     23.44 &     24.87 &   \nodata &     30.78 &     41.15 &     66.15 &     38.88 &     19.19 &     24.41 &   \nodata &     54.28 \\
 6499.649 &      Ca I &      2.52 &   $-$0.82 &     90.60 &     51.00 &     50.90 &   \nodata &     54.68 &     73.77 &     96.78 &     64.27 &     40.05 &     41.94 &   \nodata &     82.97 \\
 6717.685 &      Ca I &      2.71 &   $-$0.52 &   \nodata &     59.27 &     64.54 &   \nodata &     69.96 &   \nodata &   \nodata &     83.87 &     55.26 &     56.77 &   \nodata &   \nodata \\
%4995.002 &      Sc I &      2.11 &   $-$0.88 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4246.820 &     Sc II &      0.32 &      0.24 &    195.37 &   \nodata &    123.93 &    138.59 &    192.78 &    208.71 &   \nodata &    137.59 &    164.72 &    147.46 &    120.26 &    184.65 \\
 4400.389 &     Sc II &      0.61 &   $-$0.54 &   \nodata &   \nodata &     87.05 &     84.59 &    134.80 &   \nodata &   \nodata &     86.40 &   \nodata &    115.00 &     68.94 &   \nodata \\
 4415.544 &     Sc II &      0.59 &   $-$0.67 &   \nodata &   \nodata &     83.25 &     78.09 &    126.88 &    136.54 &   \nodata &   \nodata &    112.11 &    100.42 &     62.33 &    136.32 \\
 5031.010 &     Sc II &      1.36 &   $-$0.40 &    105.14 &     67.74 &     52.05 &     45.40 &     88.90 &    101.74 &    123.64 &   \nodata &     82.66 &     76.95 &     32.29 &     87.83 \\
 5239.811 &     Sc II &      1.46 &   $-$0.77 &     81.67 &     46.61 &     34.65 &     21.71 &     70.73 &     79.82 &     93.85 &     42.39 &     56.71 &     45.84 &     18.07 &     84.37 \\
 5526.785 &     Sc II &      1.77 &      0.02 &     97.62 &     69.94 &     56.32 &     43.08 &     91.33 &     99.00 &    113.74 &     57.10 &     78.47 &     72.94 &     24.24 &    100.58 \\
 5526.820 &     Sc II &      1.77 &      0.13 &     97.62 &     69.94 &     56.32 &     43.08 &     91.33 &   \nodata &    113.74 &     57.11 &     78.47 &     72.94 &     24.25 &    100.59 \\
 5641.000 &     Sc II &      1.50 &   $-$1.13 &     62.38 &     32.41 &     20.62 &   \nodata &     51.76 &     61.12 &     76.10 &     26.14 &     42.89 &     30.95 &   \nodata &   \nodata \\
 5657.880 &     Sc II &      1.51 &   $-$0.50 &     92.12 &     60.80 &     44.95 &     33.86 &     83.70 &     94.19 &    104.85 &   \nodata &     69.57 &     69.83 &     19.51 &     85.97 \\
 5657.907 &     Sc II &      1.51 &   $-$0.60 &     92.09 &     60.78 &     44.94 &     33.86 &     83.68 &     94.14 &    104.77 &   \nodata &     69.53 &     69.79 &     19.51 &     85.88 \\
 5667.150 &     Sc II &      1.50 &   $-$1.24 &     55.22 &     23.36 &     14.18 &     10.35 &     42.17 &     50.55 &     66.28 &     17.83 &     26.30 &     17.63 &   \nodata &     52.00 \\
 5669.040 &     Sc II &      1.50 &   $-$1.12 &     67.53 &     29.75 &     18.31 &     11.59 &     48.63 &     60.65 &     71.72 &     30.68 &     34.17 &     18.71 &   \nodata &   \nodata \\
 5684.214 &     Sc II &      1.51 &   $-$1.07 &     63.74 &   \nodata &     19.32 &     15.00 &     50.65 &     61.83 &     75.30 &     22.27 &     37.33 &     31.15 &   \nodata &   \nodata \\
 6245.610 &     Sc II &      1.51 &   $-$0.98 &     58.82 &     30.34 &     19.73 &     16.11 &     49.50 &   \nodata &     71.37 &     29.73 &   \nodata &     26.68 &   \nodata &     51.70 \\
 6604.578 &     Sc II &      1.36 &   $-$1.31 &     58.92 &     29.63 &     18.94 &     12.22 &     44.98 &   \nodata &     68.80 &     28.41 &     27.75 &     25.84 &   \nodata &     32.62 \\
 6604.600 &     Sc II &      1.36 &   $-$1.48 &     58.92 &     29.63 &     18.94 &     12.22 &     44.98 &     55.65 &     68.80 &   \nodata &     27.76 &     25.84 &   \nodata &   \nodata \\
 4008.928 &      Ti I &      0.02 &   $-$1.02 &   \nodata &   \nodata &   \nodata &     27.64 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     62.32 &   \nodata &   \nodata \\
 4512.730 &      Ti I &      0.84 &   $-$0.42 &     94.04 &     54.95 &     35.85 &     15.36 &     74.13 &     90.24 &     98.71 &     60.77 &     50.82 &     56.75 &   \nodata &     73.03 \\
 4518.020 &      Ti I &      0.83 &   $-$0.27 &    101.03 &     61.55 &     42.43 &   \nodata &     82.89 &     99.31 &    104.01 &     64.35 &     64.68 &     60.63 &   \nodata &     88.56 \\
 4533.249 &      Ti I &      0.85 &      0.53 &    138.90 &     91.92 &     77.67 &     55.03 &    121.65 &    140.44 &   \nodata &     92.43 &     98.71 &     91.17 &     54.83 &    119.28 \\
 4534.780 &      Ti I &      0.84 &      0.34 &    125.10 &     81.66 &     67.39 &     44.18 &    106.77 &    122.63 &    125.78 &     80.02 &     93.16 &     83.50 &     38.97 &    107.92 \\
 4544.687 &      Ti I &      0.82 &   $-$0.52 &   \nodata &   \nodata &   \nodata &     15.08 &   \nodata &   \nodata &   \nodata &   \nodata &     76.40 &   \nodata &   \nodata &   \nodata \\
 4548.760 &      Ti I &      0.83 &   $-$0.30 &    104.43 &     58.64 &     41.98 &     18.42 &     81.89 &     99.09 &    106.41 &     61.23 &     61.00 &     63.50 &     18.24 &     85.09 \\
 4555.490 &      Ti I &      0.85 &   $-$0.43 &     91.75 &     50.03 &     34.13 &     13.79 &     74.16 &     90.22 &     94.29 &     56.87 &     62.06 &     42.74 &   \nodata &     71.75 \\
 4656.470 &      Ti I &      0.00 &   $-$1.29 &    110.90 &     67.88 &     39.76 &     24.01 &     97.81 &    114.91 &    115.13 &     75.83 &     80.10 &     53.59 &   \nodata &     95.58 \\
 4681.910 &      Ti I &      0.05 &   $-$1.01 &    131.56 &     75.63 &     47.31 &     30.72 &    111.37 &    129.76 &    123.22 &     76.85 &     88.79 &     70.29 &     22.70 &   \nodata \\
 4840.870 &      Ti I &      0.90 &   $-$0.45 &     96.23 &     47.64 &     32.66 &     12.11 &     71.36 &     88.83 &     95.40 &     65.72 &     71.62 &     51.54 &   \nodata &   \nodata \\
 4981.730 &      Ti I &      0.84 &      0.56 &    140.51 &     97.09 &     79.99 &     63.31 &    131.75 &    147.48 &    148.47 &    104.77 &    110.54 &    101.34 &     74.90 &    117.16 \\
 4999.500 &      Ti I &      0.83 &      0.31 &    142.95 &     91.91 &     70.21 &     47.00 &    124.19 &    140.77 &    140.03 &     98.11 &    103.52 &     82.70 &     32.62 &    123.33 \\
 5007.206 &      Ti I &      0.82 &      0.17 &   \nodata &   \nodata &   \nodata &   \nodata &    140.81 &    157.08 &   \nodata &   \nodata &   \nodata &   \nodata &     42.32 &   \nodata \\
 5009.645 &      Ti I &      0.02 &   $-$2.20 &     63.88 &     18.40 &   \nodata &   \nodata &     41.92 &     62.32 &     63.63 &   \nodata &     17.11 &   \nodata &   \nodata &   \nodata \\
 5014.276 &      Ti I &      0.81 &      0.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     41.69 &   \nodata \\
 5016.160 &      Ti I &      0.85 &   $-$0.52 &     97.02 &     49.00 &   \nodata &     13.15 &     76.29 &     93.93 &     96.87 &     53.48 &     50.10 &     39.64 &   \nodata &    107.06 \\
 5020.024 &      Ti I &      0.84 &   $-$0.36 &    104.57 &     62.10 &     46.09 &   \nodata &     87.13 &    100.88 &    111.15 &     72.36 &     75.64 &     55.63 &     13.83 &     93.95 \\
 5020.024 &      Ti I &      0.84 &   $-$0.36 &    104.57 &   \nodata &   \nodata &     24.66 &     87.13 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5024.843 &      Ti I &      0.82 &   $-$0.55 &     98.85 &     49.93 &     32.67 &   \nodata &     77.40 &     95.44 &    103.11 &     61.20 &     66.97 &     52.10 &   \nodata &     96.96 \\
 5035.902 &      Ti I &      1.46 &      0.26 &    114.15 &   \nodata &   \nodata &   \nodata &     85.01 &    104.58 &   \nodata &   \nodata &     78.89 &     63.52 &   \nodata &    108.11 \\
 5038.396 &      Ti I &      1.43 &      0.07 &     87.41 &   \nodata &   \nodata &   \nodata &     65.41 &   \nodata &   \nodata &   \nodata &     47.10 &   \nodata &   \nodata &   \nodata \\
 5039.960 &      Ti I &      0.02 &   $-$1.13 &    109.75 &     71.50 &     44.89 &     28.32 &    108.58 &    119.76 &    118.39 &     74.00 &     72.19 &     71.06 &   \nodata &    106.79 \\
 5173.740 &      Ti I &      0.00 &   $-$1.06 &    148.61 &     85.77 &   \nodata &     32.54 &    125.37 &    144.99 &   \nodata &     83.65 &     90.98 &     67.90 &     21.94 &   \nodata \\
 5192.970 &      Ti I &      0.02 &   $-$0.95 &    154.33 &     86.08 &     54.22 &     40.89 &    138.37 &    161.26 &    139.55 &     84.88 &    111.15 &   \nodata &   \nodata &    113.03 \\
 5210.390 &      Ti I &      0.05 &   $-$0.83 &    145.32 &     88.39 &     58.40 &     43.12 &    130.99 &    152.12 &    139.97 &     94.49 &    113.95 &     78.91 &     30.86 &    110.73 \\
 6064.630 &      Ti I &      1.05 &   $-$1.89 &     21.12 &   \nodata &   \nodata &   \nodata &      8.41 &     17.09 &     26.61 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6091.170 &      Ti I &      2.27 &   $-$0.37 &     20.55 &   \nodata &   \nodata &   \nodata &      7.76 &     12.17 &     24.76 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6258.099 &      Ti I &      1.44 &   $-$0.30 &     76.67 &     29.68 &     20.74 &   \nodata &     48.22 &     68.36 &     80.31 &     41.86 &     30.54 &     21.33 &   \nodata &     64.50 \\
 6312.240 &      Ti I &      1.46 &   $-$1.50 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &      9.17 &     15.25 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6336.100 &      Ti I &      1.44 &   $-$1.69 &     14.27 &   \nodata &   \nodata &   \nodata &      4.55 &      8.38 &     14.20 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4012.396 &     Ti II &      0.57 &   $-$1.75 &   \nodata &   \nodata &   \nodata &    106.71 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    130.62 &   \nodata &   \nodata \\
 4025.120 &     Ti II &      0.61 &   $-$1.98 &    152.14 &    101.36 &     75.48 &     91.07 &    134.53 &    150.48 &    161.62 &     76.54 &    132.02 &    124.92 &     83.72 &     89.62 \\
 4028.338 &     Ti II &      1.89 &   $-$0.96 &   \nodata &   \nodata &     74.62 &     53.31 &    109.58 &   \nodata &    135.36 &     82.51 &     85.62 &     89.42 &     64.75 &   \nodata \\
 4053.829 &     Ti II &      1.89 &   $-$1.21 &   \nodata &     73.13 &     59.55 &     43.68 &     84.65 &     93.97 &     96.21 &   \nodata &     79.34 &     59.55 &     37.98 &     87.42 \\
 4161.527 &     Ti II &      1.08 &   $-$2.16 &   \nodata &     82.50 &     65.97 &     55.96 &    108.98 &    120.05 &   \nodata &     72.73 &    104.30 &     82.57 &     38.23 &    116.27 \\
 4163.634 &     Ti II &      2.59 &   $-$0.40 &   \nodata &     83.29 &     80.35 &     46.72 &     97.77 &   \nodata &    131.31 &     93.66 &     93.02 &    100.50 &     44.65 &    123.14 \\
 4184.309 &     Ti II &      1.08 &   $-$2.51 &   \nodata &     73.04 &     46.05 &     33.26 &    102.79 &   \nodata &   \nodata &     70.55 &     74.65 &     70.45 &     27.01 &   \nodata \\
 4330.723 &     Ti II &      1.18 &   $-$2.06 &   \nodata &     81.67 &     54.02 &     61.54 &    115.35 &   \nodata &   \nodata &     57.80 &     91.56 &     75.97 &   \nodata &   \nodata \\
 4337.914 &     Ti II &      1.08 &   $-$0.96 &    177.00 &    135.21 &    108.08 &    113.92 &    174.98 &    189.05 &    183.82 &    110.65 &    138.19 &    123.13 &     95.37 &    142.25 \\
 4394.059 &     Ti II &      1.22 &   $-$1.78 &   \nodata &     98.64 &     68.53 &     64.16 &    117.88 &    126.89 &   \nodata &     75.31 &     96.80 &     82.02 &     67.68 &     91.94 \\
 4395.839 &     Ti II &      1.24 &   $-$1.93 &    107.29 &     81.64 &     55.43 &     52.33 &    100.94 &    108.84 &    112.31 &     58.59 &     75.95 &     66.01 &     43.85 &     74.95 \\
 4399.765 &     Ti II &      1.24 &   $-$1.19 &    155.11 &   \nodata &    102.89 &     94.07 &    149.93 &    165.41 &   \nodata &    114.38 &    132.71 &    130.53 &    107.72 &    170.74 \\
 4417.714 &     Ti II &      1.17 &   $-$1.19 &    150.74 &    122.93 &     97.22 &     98.42 &    147.69 &    157.10 &    160.12 &     96.76 &    130.90 &    121.61 &     96.39 &    118.89 \\
 4418.331 &     Ti II &      1.24 &   $-$1.97 &    115.05 &     83.40 &     62.13 &     54.23 &    103.39 &    115.87 &    128.14 &     64.20 &     96.38 &     85.25 &   \nodata &     98.71 \\
 4441.731 &     Ti II &      1.18 &   $-$2.41 &   \nodata &     76.08 &     49.92 &     41.87 &    105.18 &   \nodata &   \nodata &     70.26 &     82.66 &     68.80 &     42.37 &   \nodata \\
 4443.801 &     Ti II &      1.08 &   $-$0.72 &    170.38 &    136.04 &    118.93 &    120.80 &    171.83 &    180.13 &    185.11 &    125.53 &    143.26 &    143.07 &    115.89 &    147.83 \\
 4444.554 &     Ti II &      1.12 &   $-$2.24 &   \nodata &     78.04 &     52.97 &     48.57 &    114.11 &    124.68 &    121.91 &     67.43 &     89.34 &     66.45 &     41.34 &   \nodata \\
 4450.482 &     Ti II &      1.08 &   $-$1.52 &   \nodata &   \nodata &     92.32 &     89.21 &    142.95 &   \nodata &   \nodata &     89.80 &    113.91 &    120.10 &     93.29 &   \nodata \\
 4464.448 &     Ti II &      1.16 &   $-$1.81 &    125.66 &     92.65 &     69.76 &     69.51 &    121.35 &    124.42 &    125.91 &     73.24 &    101.80 &     94.75 &     57.62 &   \nodata \\
 4468.517 &     Ti II &      1.13 &   $-$0.60 &    198.02 &    144.07 &    120.92 &    123.24 &    187.77 &    206.56 &    201.60 &    140.17 &    159.56 &    154.17 &    123.88 &    148.38 \\
 4470.853 &     Ti II &      1.17 &   $-$2.02 &    103.02 &     75.80 &     52.85 &     49.90 &    101.84 &    109.34 &    105.20 &     64.97 &     77.77 &     80.86 &     55.29 &     79.74 \\
 4501.270 &     Ti II &      1.12 &   $-$0.77 &    183.43 &    138.57 &    117.34 &    119.12 &    172.47 &    186.02 &    202.13 &    132.10 &    148.99 &    139.42 &    119.77 &   \nodata \\
 4529.480 &     Ti II &      1.57 &   $-$2.03 &   \nodata &   \nodata &   \nodata &     44.17 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     46.97 &   \nodata \\
 4533.960 &     Ti II &      1.24 &   $-$0.53 &   \nodata &    142.56 &    117.02 &    129.05 &    178.97 &   \nodata &   \nodata &    155.92 &   \nodata &    166.49 &    130.79 &   \nodata \\
%4545.144 &     Ti II &      1.13 &   $-$1.81 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4563.770 &     Ti II &      1.22 &   $-$0.96 &    164.47 &    128.53 &    111.35 &    113.29 &    161.62 &    172.90 &    184.16 &    117.99 &    149.94 &    127.59 &    108.88 &    151.96 \\
 4571.971 &     Ti II &      1.57 &   $-$0.32 &    169.34 &    139.56 &    123.29 &    112.11 &    176.97 &    178.13 &    192.74 &    132.65 &    164.10 &    142.28 &    113.43 &    165.54 \\
 4583.409 &     Ti II &      1.16 &   $-$2.92 &     64.82 &     41.39 &     19.86 &     16.77 &     59.02 &     68.03 &     68.18 &     34.53 &     55.95 &   \nodata &   \nodata &   \nodata \\
 4589.915 &     Ti II &      1.24 &   $-$1.79 &    112.94 &     90.40 &     71.52 &     72.45 &    116.31 &    122.85 &    123.07 &     83.61 &    104.43 &     95.43 &     64.82 &    107.54 \\
 4657.200 &     Ti II &      1.24 &   $-$2.24 &     89.20 &     60.13 &     49.51 &     39.71 &     87.17 &     90.13 &    101.93 &     58.36 &   \nodata &     64.47 &     47.71 &   \nodata \\
 4708.662 &     Ti II &      1.24 &   $-$2.34 &     81.49 &     61.76 &     40.30 &     35.69 &     83.25 &     88.40 &     89.98 &     48.57 &     75.06 &     67.12 &     30.21 &   \nodata \\
 4779.979 &     Ti II &      2.05 &   $-$1.37 &     82.88 &     67.97 &     55.40 &     35.04 &     79.13 &     88.25 &    101.04 &     67.70 &     86.64 &     82.57 &     29.89 &     80.98 \\
 4805.089 &     Ti II &      2.06 &   $-$1.10 &    111.53 &     81.50 &     66.81 &     46.20 &    105.06 &    105.11 &    133.81 &   \nodata &   \nodata &   \nodata &   \nodata &     92.05 \\
 4865.610 &     Ti II &      1.12 &   $-$2.81 &     74.98 &     48.72 &   \nodata &     25.59 &     68.25 &     73.97 &     78.32 &     35.52 &     56.29 &   \nodata &   \nodata &   \nodata \\
 5154.080 &     Ti II &      1.57 &   $-$1.92 &    115.43 &     78.91 &     56.50 &     43.33 &    102.04 &    112.97 &    105.23 &     80.73 &     99.72 &     78.34 &     57.65 &     95.13 \\
 5185.902 &     Ti II &      1.89 &   $-$1.49 &     99.78 &     69.85 &     57.20 &     42.62 &     90.94 &    100.72 &    112.69 &     56.78 &     81.28 &     75.04 &     36.51 &     84.78 \\
 5185.910 &     Ti II &      1.89 &   $-$1.35 &     99.78 &     69.85 &     57.21 &     42.62 &     90.94 &    100.72 &    112.69 &     56.78 &     81.28 &     75.04 &     36.51 &     84.78 \\
 5188.687 &     Ti II &      1.58 &   $-$1.05 &   \nodata &   \nodata &   \nodata &     90.08 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5226.538 &     Ti II &      1.57 &   $-$1.26 &    129.76 &     92.17 &     79.58 &     78.34 &    126.95 &    140.09 &    141.60 &     81.61 &   \nodata &     92.78 &   \nodata &   \nodata \\
 5336.786 &     Ti II &      1.58 &   $-$1.59 &    108.41 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     93.05 &   \nodata &   \nodata &   \nodata \\
 5336.790 &     Ti II &      1.58 &   $-$1.69 &    108.41 &     81.70 &     63.56 &     52.02 &    107.13 &    115.65 &    115.32 &     78.21 &     93.05 &     89.96 &     59.71 &    111.74 \\
 5381.021 &     Ti II &      1.57 &   $-$1.92 &    101.26 &     65.92 &     47.13 &     39.06 &     88.65 &     98.85 &    105.46 &     57.83 &     83.70 &     71.40 &   \nodata &     72.55 \\
 5381.030 &     Ti II &      1.59 &   $-$2.08 &    101.26 &     65.92 &     47.13 &     39.06 &     88.65 &     98.85 &    105.46 &     57.83 &     83.70 &     71.40 &     36.11 &     72.55 \\
 5418.768 &     Ti II &      1.58 &   $-$2.00 &     80.92 &     55.00 &     36.78 &     27.28 &     74.15 &     80.27 &     87.48 &     62.70 &     83.81 &     59.27 &   \nodata &     58.73 \\
 4379.230 &       V I &      0.30 &      0.55 &   \nodata &   \nodata &     62.78 &     29.56 &    113.78 &    133.23 &   \nodata &     77.25 &     70.80 &     70.45 &   \nodata &    108.98 \\
%4786.499 &       V I &      2.07 &      0.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
%5195.395 &       V I &      2.28 &   $-$0.12 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5727.060 &       V I &      1.08 &   $-$0.01 &     65.77 &     16.53 &     13.42 &   \nodata &     29.41 &     51.85 &     67.89 &     29.30 &   \nodata &   \nodata &   \nodata &     40.99 \\
%6008.648 &       V I &      1.18 &   $-$2.34 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6090.220 &       V I &      1.08 &   $-$0.06 &     50.77 &     14.46 &      8.68 &   \nodata &     25.97 &     41.73 &     57.11 &     18.50 &   \nodata &     18.70 &   \nodata &     38.31 \\
 6216.360 &       V I &      0.28 &   $-$1.29 &     47.57 &      8.52 &      7.00 &   \nodata &     17.79 &     34.43 &     48.98 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6251.820 &       V I &      0.29 &   $-$1.34 &     35.70 &      6.24 &   \nodata &   \nodata &     14.38 &     27.81 &     32.83 &   \nodata &      7.66 &   \nodata &   \nodata &     19.99 \\
 6274.640 &       V I &      0.27 &   $-$1.67 &   \nodata &   \nodata &   \nodata &   \nodata &      7.51 &     14.97 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
%6504.160 &       V I &      1.18 &   $-$1.23 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 3908.762 &      Cr I &      1.00 &   $-$1.00 &   \nodata &   \nodata &     55.54 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     86.03 &   \nodata &   \nodata &   \nodata \\
 4254.332 &      Cr I &      0.00 &   $-$0.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    109.68 &    215.63 \\
 4274.800 &      Cr I &      0.00 &   $-$0.22 &   \nodata &   \nodata &   \nodata &   \nodata &    223.92 &    272.20 &   \nodata &   \nodata &    190.22 &   \nodata &    104.57 &    281.69 \\
 4289.720 &      Cr I &      0.00 &   $-$0.37 &   \nodata &   \nodata &    137.50 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    184.37 &    168.62 &    112.90 &   \nodata \\
 4337.566 &      Cr I &      0.97 &   $-$1.11 &   \nodata &   \nodata &   \nodata &   \nodata &    101.48 &   \nodata &   \nodata &   \nodata &     99.70 &     77.07 &   \nodata &    116.36 \\
 4545.950 &      Cr I &      0.94 &   $-$1.37 &    102.58 &     58.49 &     42.89 &     15.72 &     83.68 &    100.67 &    104.89 &     64.34 &     79.27 &     72.24 &   \nodata &     98.26 \\
 4580.056 &      Cr I &      0.94 &   $-$1.65 &   \nodata &     53.81 &     39.63 &   \nodata &     89.53 &   \nodata &   \nodata &     69.27 &     69.98 &     57.24 &   \nodata &   \nodata \\
 4600.752 &      Cr I &      1.00 &   $-$1.26 &    105.64 &     63.25 &     47.24 &     15.69 &     98.01 &     98.90 &    106.67 &     86.68 &     85.15 &     72.62 &     22.74 &    105.98 \\
 4616.137 &      Cr I &      0.98 &   $-$1.19 &    107.09 &     65.42 &     50.24 &     19.99 &     91.12 &    104.53 &    109.57 &     77.37 &     83.72 &     62.47 &   \nodata &     85.92 \\
 4626.188 &      Cr I &      0.97 &   $-$1.32 &    101.17 &     59.08 &     42.80 &     17.18 &     83.42 &    100.44 &    103.05 &     65.03 &     75.59 &     56.78 &   \nodata &    109.95 \\
 4646.150 &      Cr I &      1.03 &   $-$0.74 &    128.09 &     83.15 &     69.00 &     37.31 &    111.83 &    128.35 &    132.23 &     87.02 &    100.03 &     86.54 &     43.44 &    118.75 \\
 4651.280 &      Cr I &      0.98 &   $-$1.46 &     97.81 &     51.98 &     36.49 &     12.73 &     77.53 &     95.55 &     99.36 &     59.72 &     70.36 &     55.98 &   \nodata &     84.75 \\
 4652.158 &      Cr I &      1.00 &   $-$1.03 &    114.03 &     68.58 &     56.00 &     23.74 &     94.77 &    111.67 &    120.22 &     83.58 &     81.37 &     71.06 &     27.62 &    104.58 \\
 4789.340 &      Cr I &      2.54 &   $-$0.33 &   \nodata &   \nodata &     19.84 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5206.040 &      Cr I &      0.94 &      0.02 &    201.39 &    127.91 &    125.14 &   \nodata &    179.68 &    189.27 &    209.49 &    156.03 &    164.93 &    142.09 &     95.71 &    188.93 \\
 5208.419 &      Cr I &      0.94 &      0.16 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    185.43 &   \nodata &   \nodata &    104.26 &    269.79 \\
 5247.564 &      Cr I &      0.96 &   $-$1.64 &   \nodata &     50.48 &     36.29 &     15.27 &     81.60 &    103.90 &   \nodata &     59.38 &     73.79 &   \nodata &   \nodata &     71.73 \\
 5296.690 &      Cr I &      0.98 &   $-$1.36 &    112.49 &     62.47 &     44.41 &   \nodata &     92.97 &    114.30 &    114.87 &     82.12 &     81.44 &     60.74 &   \nodata &     88.87 \\
 5298.280 &      Cr I &      0.98 &   $-$1.14 &   \nodata &   \nodata &   \nodata &   \nodata &    125.47 &   \nodata &   \nodata &     92.60 &    104.08 &     70.79 &   \nodata &   \nodata \\
 5300.740 &      Cr I &      0.98 &   $-$2.00 &     71.84 &     26.98 &     15.81 &   \nodata &     46.82 &     75.31 &     79.96 &     35.29 &     43.75 &     22.71 &   \nodata &     68.80 \\
 5345.800 &      Cr I &      1.00 &   $-$0.95 &    137.41 &     84.85 &     66.87 &     28.97 &    116.00 &    133.57 &   \nodata &    102.06 &     94.27 &     83.76 &     30.67 &    147.09 \\
 5348.310 &      Cr I &      1.00 &   $-$1.21 &    115.00 &     67.07 &     49.88 &     23.36 &     95.52 &    114.36 &    116.50 &     89.40 &     93.17 &     74.88 &   \nodata &    127.78 \\
 5409.770 &      Cr I &      1.03 &   $-$0.67 &   \nodata &     94.50 &     81.46 &     41.04 &    131.98 &    153.06 &   \nodata &    118.32 &    123.75 &     89.06 &     39.22 &    169.78 \\
%3408.737 &     Cr II &      2.48 &   $-$0.42 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4558.594 &     Cr II &      4.07 &   $-$0.66 &     81.95 &     56.00 &     58.15 &     21.19 &   \nodata &   \nodata &   \nodata &     60.82 &     69.52 &     62.21 &     24.11 &     89.29 \\
 4588.142 &     Cr II &      4.07 &   $-$0.83 &     62.14 &     44.61 &     49.09 &     14.42 &     46.23 &     55.77 &     78.03 &     55.53 &     56.22 &     51.15 &   \nodata &   \nodata \\
 4591.992 &     Cr II &      4.07 &   $-$1.42 &     36.44 &     21.03 &     22.37 &      4.10 &     20.81 &   \nodata &     50.83 &     16.62 &   \nodata &     28.20 &   \nodata &   \nodata \\
 4030.753 &      Mn I &      0.00 &   $-$0.48 &   \nodata &   \nodata &    166.68 &    144.08 &    232.55 &   \nodata &   \nodata &    202.53 &    213.20 &    176.54 &    124.17 &   \nodata \\
 4033.062 &      Mn I &      0.00 &   $-$0.62 &   \nodata &    167.35 &    148.38 &    130.61 &    228.29 &    259.24 &    313.20 &    197.57 &    216.18 &    177.40 &    107.47 &   \nodata \\
 4034.483 &      Mn I &      0.00 &   $-$0.81 &   \nodata &   \nodata &    137.52 &    122.72 &    199.46 &    227.79 &    230.86 &    165.95 &    189.96 &    182.87 &    115.35 &    208.73 \\
 4041.357 &      Mn I &      2.11 &      0.28 &   \nodata &   \nodata &   \nodata &     43.89 &   \nodata &   \nodata &   \nodata &    128.55 &   \nodata &   \nodata &     52.34 &   \nodata \\
 4754.048 &      Mn I &      2.28 &   $-$0.09 &    121.02 &     62.31 &     59.90 &     19.72 &     92.89 &    109.90 &    132.80 &     87.80 &     86.84 &     64.14 &   \nodata &   \nodata \\
 4783.432 &      Mn I &      2.30 &      0.04 &    127.46 &     67.53 &     63.85 &     27.56 &     99.63 &   \nodata &    143.42 &     94.64 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4823.528 &      Mn I &      2.32 &      0.14 &   \nodata &     67.61 &     70.12 &     27.56 &     98.93 &    118.59 &    140.13 &    127.66 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6013.530 &      Mn I &      3.07 &   $-$0.25 &     56.58 &     11.29 &     17.61 &   \nodata &     21.30 &     34.23 &     71.01 &     36.11 &     23.29 &   \nodata &   \nodata &     38.32 \\
 6016.670 &      Mn I &      3.08 &   $-$0.10 &     65.84 &     15.39 &     19.29 &   \nodata &     26.61 &     41.67 &     82.72 &     38.82 &     27.85 &   \nodata &   \nodata &   \nodata \\
 6021.800 &      Mn I &      3.08 &      0.03 &     71.06 &     22.10 &     24.61 &   \nodata &     36.73 &     54.54 &     86.55 &     44.24 &     39.40 &     23.08 &   \nodata &     59.40 \\
 3917.181 &      Fe I &      0.99 &   $-$2.15 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    104.41 &   \nodata \\
 3949.953 &      Fe I &      2.18 &   $-$1.25 &   \nodata &   \nodata &   \nodata &     72.79 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     70.65 &   \nodata \\
 4001.661 &      Fe I &      2.18 &   $-$1.90 &   \nodata &   \nodata &   \nodata &     37.28 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     38.87 &   \nodata \\
 4007.272 &      Fe I &      2.76 &   $-$1.28 &   \nodata &   \nodata &   \nodata &     29.49 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     37.05 &   \nodata \\
%4014.531 &      Fe I &      3.05 &   $-$0.59 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4021.866 &      Fe I &      2.76 &   $-$0.73 &   \nodata &   \nodata &   \nodata &     59.84 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4032.627 &      Fe I &      1.49 &   $-$2.38 &   \nodata &   \nodata &   \nodata &     59.82 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4044.609 &      Fe I &      2.83 &   $-$1.22 &   \nodata &   \nodata &   \nodata &     32.94 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     56.85 &   \nodata \\
 4058.217 &      Fe I &      3.21 &   $-$1.11 &   \nodata &   \nodata &   \nodata &     29.90 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4062.441 &      Fe I &      2.85 &   $-$0.86 &   \nodata &   \nodata &   \nodata &     43.78 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4067.271 &      Fe I &      2.56 &   $-$1.42 &   \nodata &   \nodata &   \nodata &     43.23 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4067.978 &      Fe I &      3.21 &   $-$0.47 &   \nodata &   \nodata &   \nodata &     45.90 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4070.769 &      Fe I &      3.24 &   $-$0.79 &   \nodata &   \nodata &   \nodata &     28.05 &     76.19 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     37.28 &   \nodata \\
 4073.763 &      Fe I &      3.27 &   $-$0.90 &   \nodata &   \nodata &   \nodata &     20.51 &   \nodata &   \nodata &   \nodata &     58.05 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4079.838 &      Fe I &      2.86 &   $-$1.36 &   \nodata &   \nodata &   \nodata &     21.76 &     76.41 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4098.176 &      Fe I &      3.24 &   $-$0.88 &   \nodata &   \nodata &   \nodata &     28.26 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4109.057 &      Fe I &      3.29 &   $-$1.56 &   \nodata &   \nodata &     33.32 &     11.48 &   \nodata &   \nodata &   \nodata &     59.14 &     62.21 &     43.58 &   \nodata &   \nodata \\
 4109.802 &      Fe I &      2.85 &   $-$0.94 &   \nodata &   \nodata &   \nodata &     44.61 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     34.89 &   \nodata \\
 4114.445 &      Fe I &      2.83 &   $-$1.30 &   \nodata &   \nodata &   \nodata &     29.41 &   \nodata &   \nodata &   \nodata &     63.67 &   \nodata &   \nodata &     37.88 &   \nodata \\
 4120.207 &      Fe I &      2.99 &   $-$1.27 &   \nodata &   \nodata &   \nodata &     23.96 &     79.21 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     58.46 &   \nodata \\
 4121.802 &      Fe I &      2.83 &   $-$1.45 &   \nodata &   \nodata &   \nodata &     27.09 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     56.65 &   \nodata \\
 4132.899 &      Fe I &      2.85 &   $-$1.01 &   \nodata &   \nodata &   \nodata &     48.41 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4134.678 &      Fe I &      2.83 &   $-$0.65 &   \nodata &   \nodata &   \nodata &     62.46 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     76.79 &   \nodata \\
 4136.998 &      Fe I &      3.42 &   $-$0.45 &   \nodata &   \nodata &   \nodata &     26.24 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4139.927 &      Fe I &      0.99 &   $-$3.63 &   \nodata &   \nodata &     36.63 &     37.32 &   \nodata &   \nodata &   \nodata &     59.28 &   \nodata &   \nodata &     22.88 &   \nodata \\
 4147.669 &      Fe I &      1.48 &   $-$2.07 &   \nodata &   \nodata &   \nodata &     80.55 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     87.30 &   \nodata \\
 4153.899 &      Fe I &      3.40 &   $-$0.32 &   \nodata &   \nodata &   \nodata &     44.85 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     48.11 &   \nodata \\
 4154.498 &      Fe I &      2.83 &   $-$0.69 &   \nodata &   \nodata &   \nodata &     55.10 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     69.59 &   \nodata \\
 4154.805 &      Fe I &      3.37 &   $-$0.40 &   \nodata &   \nodata &   \nodata &     39.35 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4157.780 &      Fe I &      3.42 &   $-$0.40 &   \nodata &   \nodata &   \nodata &     36.69 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     64.81 &   \nodata \\
 4158.793 &      Fe I &      3.43 &   $-$0.67 &   \nodata &   \nodata &   \nodata &     24.14 &     76.79 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4174.913 &      Fe I &      0.91 &   $-$2.94 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     81.37 &   \nodata \\
 4175.636 &      Fe I &      2.85 &   $-$0.83 &   \nodata &   \nodata &   \nodata &     51.95 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     61.46 &   \nodata \\
 4181.755 &      Fe I &      2.83 &   $-$0.37 &   \nodata &   \nodata &   \nodata &     77.50 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     79.73 &   \nodata \\
 4182.382 &      Fe I &      3.02 &   $-$1.18 &   \nodata &   \nodata &   \nodata &     22.90 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     23.75 &   \nodata \\
 4184.892 &      Fe I &      2.83 &   $-$0.87 &   \nodata &   \nodata &   \nodata &     46.31 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4191.430 &      Fe I &      2.47 &   $-$0.67 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    104.24 &   \nodata \\
 4195.329 &      Fe I &      3.33 &   $-$0.49 &   \nodata &   \nodata &   \nodata &     43.94 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     67.61 &   \nodata \\
 4196.208 &      Fe I &      3.40 &   $-$0.70 &   \nodata &   \nodata &   \nodata &     22.32 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4217.545 &      Fe I &      3.43 &   $-$0.48 &   \nodata &   \nodata &   \nodata &     30.67 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     50.36 &   \nodata \\
 4222.213 &      Fe I &      2.45 &   $-$0.91 &   \nodata &   \nodata &   \nodata &     76.59 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     64.79 &   \nodata \\
 4233.603 &      Fe I &      2.48 &   $-$0.58 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     77.14 &   \nodata \\
 4238.810 &      Fe I &      3.40 &   $-$0.23 &   \nodata &   \nodata &   \nodata &     44.66 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
%4282.403 &      Fe I &      2.18 &   $-$0.78 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4337.046 &      Fe I &      1.56 &   $-$1.70 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    102.03 &   \nodata \\
 4352.735 &      Fe I &      2.22 &   $-$1.29 &   \nodata &   \nodata &   \nodata &     85.66 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     83.71 &   \nodata \\
 4375.930 &      Fe I &      0.00 &   $-$3.00 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    108.29 &   \nodata \\
 4388.407 &      Fe I &      3.60 &   $-$0.68 &   \nodata &   \nodata &     53.82 &     18.68 &     63.96 &     75.75 &   \nodata &     64.97 &   \nodata &     52.62 &     18.51 &   \nodata \\
 4407.709 &      Fe I &      2.18 &   $-$1.97 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     53.24 &   \nodata \\
 4422.568 &      Fe I &      2.85 &   $-$1.11 &   \nodata &   \nodata &   \nodata &     46.62 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     66.15 &   \nodata \\
 4442.339 &      Fe I &      2.20 &   $-$1.23 &   \nodata &   \nodata &   \nodata &     83.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     78.06 &   \nodata \\
 4443.194 &      Fe I &      2.86 &   $-$1.04 &   \nodata &   \nodata &   \nodata &     40.00 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     36.64 &   \nodata \\
 4447.717 &      Fe I &      2.22 &   $-$1.34 &   \nodata &   \nodata &   \nodata &     72.28 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     69.35 &   \nodata \\
%4454.381 &      Fe I &      2.83 &   $-$1.30 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4461.653 &      Fe I &      0.09 &   $-$3.19 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    108.19 &   \nodata \\
 4466.552 &      Fe I &      2.83 &   $-$0.60 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     76.63 &   \nodata \\
 4476.019 &      Fe I &      2.85 &   $-$0.82 &   \nodata &   \nodata &   \nodata &     66.83 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     91.02 &   \nodata \\
 4484.220 &      Fe I &      3.60 &   $-$0.86 &   \nodata &   \nodata &   \nodata &     21.33 &     72.22 &   \nodata &   \nodata &     68.20 &     61.97 &   \nodata &     27.05 &   \nodata \\
 4489.739 &      Fe I &      0.12 &   $-$3.90 &   \nodata &   \nodata &   \nodata &     88.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     93.22 &   \nodata \\
 4490.083 &      Fe I &      3.02 &   $-$1.58 &   \nodata &   \nodata &     38.52 &   \nodata &   \nodata &     73.19 &   \nodata &     56.96 &     59.48 &   \nodata &   \nodata &   \nodata \\
 4494.563 &      Fe I &      2.20 &   $-$1.14 &   \nodata &   \nodata &   \nodata &     87.05 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     86.59 &   \nodata \\
 4531.148 &      Fe I &      1.48 &   $-$2.10 &   \nodata &   \nodata &   \nodata &     86.02 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     80.79 &   \nodata \\
 4592.651 &      Fe I &      1.56 &   $-$2.46 &   \nodata &   \nodata &   \nodata &     67.33 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     70.94 &   \nodata \\
 4595.359 &      Fe I &      3.29 &   $-$1.76 &   \nodata &     37.45 &     29.89 &   \nodata &     54.50 &   \nodata &   \nodata &     56.61 &     42.46 &     39.88 &   \nodata &   \nodata \\
 4602.941 &      Fe I &      1.49 &   $-$2.21 &   \nodata &   \nodata &   \nodata &     83.59 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     78.33 &   \nodata \\
 4630.120 &      Fe I &      2.28 &   $-$2.59 &   \nodata &     50.64 &     34.44 &     15.42 &     82.18 &   \nodata &   \nodata &     60.29 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4632.912 &      Fe I &      1.61 &   $-$2.91 &   \nodata &   \nodata &     53.82 &     36.00 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     45.90 &   \nodata \\
 4643.463 &      Fe I &      3.64 &   $-$1.15 &     73.22 &     33.44 &     34.44 &      5.89 &     43.90 &     63.52 &     79.61 &     57.17 &     46.32 &     46.48 &   \nodata &   \nodata \\
 4647.434 &      Fe I &      2.95 &   $-$1.35 &   \nodata &   \nodata &   \nodata &     28.46 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     31.39 &   \nodata \\
 4678.846 &      Fe I &      3.60 &   $-$0.83 &   \nodata &   \nodata &   \nodata &     20.64 &     75.58 &     92.59 &   \nodata &     72.22 &   \nodata &   \nodata &     17.17 &   \nodata \\
 4691.411 &      Fe I &      2.99 &   $-$1.52 &   \nodata &   \nodata &   \nodata &     22.30 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     38.97 &   \nodata \\
 4707.274 &      Fe I &      3.24 &   $-$1.08 &   \nodata &   \nodata &   \nodata &     30.58 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4710.283 &      Fe I &      3.02 &   $-$1.61 &   \nodata &   \nodata &     50.32 &     18.03 &   \nodata &   \nodata &   \nodata &   \nodata &     72.07 &     57.57 &   \nodata &   \nodata \\
 4733.591 &      Fe I &      1.49 &   $-$2.99 &   \nodata &   \nodata &     50.53 &     40.39 &   \nodata &   \nodata &   \nodata &     74.98 &   \nodata &   \nodata &     40.05 &   \nodata \\
 4736.772 &      Fe I &      3.21 &   $-$0.75 &   \nodata &   \nodata &   \nodata &     43.95 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     49.83 &   \nodata \\
 4859.741 &      Fe I &      2.88 &   $-$0.76 &   \nodata &   \nodata &   \nodata &     64.98 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     71.95 &   \nodata \\
 4903.310 &      Fe I &      2.88 &   $-$0.93 &   \nodata &   \nodata &   \nodata &     53.63 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4924.770 &      Fe I &      2.28 &   $-$2.11 &   \nodata &   \nodata &     51.57 &     28.66 &   \nodata &   \nodata &   \nodata &     73.61 &   \nodata &   \nodata &     23.99 &   \nodata \\
 4938.814 &      Fe I &      2.88 &   $-$1.08 &   \nodata &   \nodata &   \nodata &     43.25 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     44.99 &   \nodata \\
 4939.687 &      Fe I &      0.86 &   $-$3.25 &   \nodata &   \nodata &   \nodata &     71.75 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     63.71 &   \nodata \\
 4946.388 &      Fe I &      3.37 &   $-$1.17 &     96.29 &     57.04 &     51.65 &     16.92 &     77.37 &     90.40 &   \nodata &     78.00 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4966.089 &      Fe I &      3.33 &   $-$0.87 &   \nodata &   \nodata &   \nodata &     31.11 &     95.02 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     30.23 &   \nodata \\
 4973.102 &      Fe I &      3.96 &   $-$0.95 &   \nodata &     40.91 &     40.14 &   \nodata &     53.92 &     74.20 &   \nodata &     60.05 &     48.64 &     44.60 &   \nodata &   \nodata \\
 4994.130 &      Fe I &      0.92 &   $-$2.97 &   \nodata &   \nodata &   \nodata &     81.73 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     90.46 &   \nodata \\
 5001.870 &      Fe I &      3.88 &      0.05 &   \nodata &   \nodata &   \nodata &     33.48 &   \nodata &     97.75 &   \nodata &   \nodata &   \nodata &   \nodata &     46.69 &   \nodata \\
 5006.119 &      Fe I &      2.83 &   $-$0.61 &   \nodata &   \nodata &   \nodata &     72.78 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     71.06 &   \nodata \\
 5012.068 &      Fe I &      0.86 &   $-$2.64 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    103.90 &   \nodata \\
 5014.942 &      Fe I &      3.94 &   $-$0.30 &     98.39 &   \nodata &   \nodata &     24.91 &     76.00 &     89.61 &   \nodata &     73.27 &     74.53 &   \nodata &   \nodata &   \nodata \\
 5028.127 &      Fe I &      3.56 &   $-$1.12 &     83.55 &     41.95 &     38.90 &     11.03 &     55.32 &     72.94 &     92.80 &     66.14 &     51.90 &     31.43 &   \nodata &     76.38 \\
 5044.212 &      Fe I &      2.85 &   $-$2.02 &     78.28 &     38.24 &     26.22 &   \nodata &     64.15 &     79.45 &     85.73 &     43.73 &     54.82 &     39.31 &     31.83 &     65.69 \\
 5049.820 &      Fe I &      2.28 &   $-$1.35 &   \nodata &   \nodata &   \nodata &     74.82 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5051.634 &      Fe I &      0.92 &   $-$2.76 &   \nodata &   \nodata &   \nodata &     98.51 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5068.766 &      Fe I &      2.94 &   $-$1.04 &   \nodata &   \nodata &   \nodata &     41.45 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     44.66 &   \nodata \\
 5074.749 &      Fe I &      4.22 &   $-$0.20 &     91.98 &     59.59 &     62.08 &     18.24 &     72.61 &     86.45 &   \nodata &   \nodata &     72.15 &   \nodata &     25.99 &   \nodata \\
 5083.339 &      Fe I &      0.96 &   $-$2.84 &   \nodata &   \nodata &   \nodata &     87.55 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     78.80 &   \nodata \\
 5090.770 &      Fe I &      4.26 &   $-$0.36 &     79.33 &     41.08 &     42.94 &     12.11 &     45.98 &     64.65 &     84.77 &     56.71 &     49.71 &     38.77 &   \nodata &   \nodata \\
 5110.413 &      Fe I &      0.00 &   $-$3.76 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    105.55 &   \nodata \\
 5123.720 &      Fe I &      1.01 &   $-$3.06 &   \nodata &   \nodata &   \nodata &     78.34 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     66.38 &   \nodata \\
 5125.117 &      Fe I &      4.22 &   $-$0.14 &   \nodata &   \nodata &   \nodata &     19.00 &     85.67 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5127.360 &      Fe I &      0.92 &   $-$3.25 &   \nodata &   \nodata &     62.00 &     70.95 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     85.55 &   \nodata \\
 5131.468 &      Fe I &      2.22 &   $-$2.52 &   \nodata &     63.91 &     42.83 &     23.73 &     97.72 &   \nodata &   \nodata &     63.02 &   \nodata &   \nodata &     24.89 &   \nodata \\
 5133.689 &      Fe I &      4.18 &      0.14 &   \nodata &   \nodata &   \nodata &     29.04 &     93.77 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     35.62 &   \nodata \\
 5137.382 &      Fe I &      4.18 &   $-$0.40 &   \nodata &   \nodata &     59.25 &   \nodata &   \nodata &   \nodata &   \nodata &     76.62 &     57.63 &     47.97 &   \nodata &   \nodata \\
 5141.739 &      Fe I &      2.42 &   $-$2.24 &     99.72 &     60.44 &     42.15 &     19.82 &     84.41 &     99.47 &    100.15 &     66.45 &   \nodata &     61.26 &   \nodata &   \nodata \\
 5142.929 &      Fe I &      0.96 &   $-$3.08 &   \nodata &   \nodata &   \nodata &     82.69 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     99.26 &   \nodata \\
 5150.839 &      Fe I &      0.99 &   $-$3.04 &   \nodata &   \nodata &   \nodata &     72.64 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     66.21 &   \nodata \\
 5151.911 &      Fe I &      1.01 &   $-$3.32 &   \nodata &   \nodata &     60.22 &     62.26 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     52.00 &   \nodata \\
 5162.273 &      Fe I &      4.18 &      0.02 &   \nodata &   \nodata &   \nodata &     25.10 &     84.25 &     99.49 &   \nodata &   \nodata &   \nodata &   \nodata &     47.93 &   \nodata \\
 5166.282 &      Fe I &      0.00 &   $-$4.12 &   \nodata &   \nodata &   \nodata &     91.67 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     80.02 &   \nodata \\
 5171.596 &      Fe I &      1.49 &   $-$1.72 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    102.45 &   \nodata \\
 5191.455 &      Fe I &      3.04 &   $-$0.55 &   \nodata &   \nodata &   \nodata &     67.84 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     56.74 &   \nodata \\
 5192.344 &      Fe I &      3.00 &   $-$0.42 &   \nodata &   \nodata &   \nodata &     75.31 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     67.53 &   \nodata \\
 5194.942 &      Fe I &      1.56 &   $-$2.02 &   \nodata &   \nodata &   \nodata &     91.02 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     96.21 &   \nodata \\
 5198.711 &      Fe I &      2.22 &   $-$2.09 &   \nodata &   \nodata &     56.25 &     48.12 &   \nodata &   \nodata &   \nodata &     76.09 &   \nodata &   \nodata &     37.37 &   \nodata \\
 5202.336 &      Fe I &      2.18 &   $-$1.87 &   \nodata &   \nodata &   \nodata &     60.21 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     74.68 &   \nodata \\
 5216.274 &      Fe I &      1.61 &   $-$2.08 &   \nodata &   \nodata &   \nodata &     91.01 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     67.52 &   \nodata \\
 5217.390 &      Fe I &      3.21 &   $-$1.16 &   \nodata &   \nodata &     61.17 &     31.67 &     87.94 &    102.47 &   \nodata &   \nodata &   \nodata &   \nodata &     25.27 &   \nodata \\
 5225.526 &      Fe I &      0.11 &   $-$4.75 &   \nodata &   \nodata &     31.58 &     45.17 &   \nodata &   \nodata &   \nodata &     69.56 &   \nodata &   \nodata &     45.70 &   \nodata \\
 5242.491 &      Fe I &      3.63 &   $-$0.97 &     87.14 &     49.48 &     46.99 &     10.12 &     63.68 &     81.17 &     95.90 &     59.31 &     58.79 &     47.68 &   \nodata &   \nodata \\
 5247.050 &      Fe I &      0.09 &   $-$4.95 &   \nodata &   \nodata &     29.50 &     37.09 &   \nodata &   \nodata &   \nodata &     59.16 &   \nodata &   \nodata &     36.06 &   \nodata \\
 5250.210 &      Fe I &      0.12 &   $-$4.94 &   \nodata &     65.39 &     24.71 &     38.06 &   \nodata &   \nodata &   \nodata &     73.41 &   \nodata &     62.92 &     37.44 &   \nodata \\
 5250.646 &      Fe I &      2.20 &   $-$2.18 &   \nodata &   \nodata &     62.99 &     42.74 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     48.79 &   \nodata \\
 5263.305 &      Fe I &      3.27 &   $-$0.88 &   \nodata &   \nodata &   \nodata &     26.21 &     95.62 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     36.80 &   \nodata \\
 5266.555 &      Fe I &      3.00 &   $-$0.39 &   \nodata &   \nodata &   \nodata &     73.12 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     81.64 &   \nodata \\
 5281.790 &      Fe I &      3.04 &   $-$0.83 &   \nodata &   \nodata &   \nodata &     44.15 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     47.79 &   \nodata \\
 5283.621 &      Fe I &      3.24 &   $-$0.52 &   \nodata &   \nodata &   \nodata &     53.36 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     58.19 &   \nodata \\
 5288.527 &      Fe I &      3.68 &   $-$1.51 &     55.62 &     19.45 &     19.78 &   \nodata &     25.84 &     39.36 &     64.35 &     37.66 &     35.43 &     23.55 &   \nodata &     47.82 \\
 5302.300 &      Fe I &      3.28 &   $-$0.72 &   \nodata &   \nodata &   \nodata &     41.03 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     46.38 &   \nodata \\
 5307.361 &      Fe I &      1.61 &   $-$2.91 &   \nodata &   \nodata &     47.37 &     38.95 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     29.18 &   \nodata \\
 5321.110 &      Fe I &      4.43 &   $-$1.11 &     27.70 &      7.46 &     10.25 &   \nodata &      9.21 &     15.57 &     33.33 &     19.06 &     16.23 &   \nodata &   \nodata &     40.38 \\
 5322.040 &      Fe I &      2.28 &   $-$2.84 &     76.90 &     32.82 &     19.27 &      8.67 &     55.79 &     74.77 &     78.42 &     47.61 &     53.14 &     40.44 &   \nodata &     79.60 \\
 5324.179 &      Fe I &      3.21 &   $-$0.10 &   \nodata &   \nodata &   \nodata &     74.72 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     73.83 &   \nodata \\
 5326.140 &      Fe I &      3.57 &   $-$2.13 &     30.47 &      6.67 &      7.04 &   \nodata &     12.54 &     21.24 &     40.78 &     16.14 &   \nodata &   \nodata &   \nodata &     22.70 \\
 5328.039 &      Fe I &      0.92 &   $-$1.47 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    171.24 &   \nodata \\
 5332.900 &      Fe I &      1.55 &   $-$2.78 &   \nodata &   \nodata &     59.45 &     49.73 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     45.22 &   \nodata \\
 5339.930 &      Fe I &      3.27 &   $-$0.72 &   \nodata &   \nodata &   \nodata &     41.47 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     38.11 &   \nodata \\
 5364.871 &      Fe I &      4.45 &      0.23 &     93.56 &     59.88 &   \nodata &     24.05 &     70.28 &     87.85 &   \nodata &   \nodata &     71.67 &     66.37 &   \nodata &   \nodata \\
 5365.400 &      Fe I &      3.56 &   $-$1.02 &   \nodata &     42.04 &     38.32 &     11.13 &     52.95 &     68.30 &     85.76 &     54.20 &     53.60 &     49.44 &   \nodata &     75.99 \\
 5367.480 &      Fe I &      4.41 &      0.43 &    102.97 &     65.12 &   \nodata &     22.67 &     76.43 &     91.25 &   \nodata &   \nodata &     80.18 &   \nodata &     31.79 &   \nodata \\
 5369.962 &      Fe I &      4.37 &      0.54 &   \nodata &   \nodata &   \nodata &     27.67 &     91.69 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     31.66 &   \nodata \\
 5379.573 &      Fe I &      3.69 &   $-$1.51 &     56.79 &     23.05 &     19.73 &   \nodata &     30.32 &     45.54 &     64.21 &     44.54 &     27.95 &     14.49 &   \nodata &     45.77 \\
 5383.369 &      Fe I &      4.31 &      0.65 &   \nodata &   \nodata &   \nodata &     45.36 &     97.31 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     41.03 &   \nodata \\
 5389.479 &      Fe I &      4.42 &   $-$0.41 &     75.97 &     35.58 &     40.36 &      4.58 &     44.15 &     62.34 &     85.00 &     54.28 &     48.96 &     27.97 &   \nodata &   \nodata \\
 5393.168 &      Fe I &      3.24 &   $-$0.91 &   \nodata &   \nodata &   \nodata &     38.02 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     50.11 &   \nodata \\
 5410.910 &      Fe I &      4.47 &      0.40 &    102.94 &     64.19 &   \nodata &     21.89 &     73.98 &     90.79 &   \nodata &     72.24 &     75.95 &     64.94 &     25.01 &   \nodata \\
 5415.199 &      Fe I &      4.39 &      0.64 &   \nodata &   \nodata &   \nodata &     30.57 &     93.88 &    105.86 &   \nodata &   \nodata &   \nodata &   \nodata &     55.35 &   \nodata \\
 5424.068 &      Fe I &      4.32 &      0.52 &   \nodata &   \nodata &   \nodata &     40.12 &    105.02 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     39.45 &   \nodata \\
 5434.524 &      Fe I &      1.01 &   $-$2.13 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    135.40 &   \nodata \\
 5497.516 &      Fe I &      1.01 &   $-$2.83 &   \nodata &   \nodata &   \nodata &     92.62 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     89.53 &   \nodata \\
 5501.465 &      Fe I &      0.96 &   $-$3.05 &   \nodata &   \nodata &   \nodata &     91.59 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     94.70 &   \nodata \\
 5506.779 &      Fe I &      0.99 &   $-$2.79 &   \nodata &   \nodata &   \nodata &    101.37 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     97.95 &   \nodata \\
 5569.618 &      Fe I &      3.42 &   $-$0.54 &   \nodata &   \nodata &   \nodata &     41.66 &    103.55 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     40.10 &   \nodata \\
 5576.088 &      Fe I &      3.43 &   $-$1.00 &    109.79 &     68.09 &     64.10 &     24.41 &     88.04 &    105.02 &   \nodata &     88.16 &   \nodata &   \nodata &     36.44 &   \nodata \\
 5586.756 &      Fe I &      3.37 &   $-$0.14 &   \nodata &   \nodata &   \nodata &     62.14 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     64.16 &   \nodata \\
 5615.644 &      Fe I &      3.33 &      0.05 &   \nodata &   \nodata &   \nodata &     78.45 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     88.26 &   \nodata \\
 5618.630 &      Fe I &      4.21 &   $-$1.29 &     37.02 &     11.96 &     13.09 &   \nodata &     14.18 &     26.52 &     50.04 &     22.32 &     17.37 &     14.94 &   \nodata &     54.36 \\
 5624.542 &      Fe I &      3.42 &   $-$0.76 &   \nodata &   \nodata &     70.13 &     28.90 &     95.83 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     25.16 &   \nodata \\
 5662.516 &      Fe I &      4.18 &   $-$0.57 &     86.13 &     44.10 &     45.36 &     10.18 &     54.17 &     74.35 &     99.62 &     66.50 &     57.40 &   \nodata &   \nodata &   \nodata \\
 5686.529 &      Fe I &      4.55 &   $-$0.45 &     68.51 &     23.68 &     28.93 &   \nodata &     29.05 &     44.38 &     83.90 &     41.12 &     29.62 &     32.69 &   \nodata &   \nodata \\
 5701.550 &      Fe I &      2.56 &   $-$2.22 &    100.10 &     56.17 &     40.41 &     17.84 &     81.42 &    100.29 &    103.12 &     61.52 &     71.37 &     55.88 &   \nodata &     83.61 \\
 5705.470 &      Fe I &      4.30 &   $-$1.42 &     23.28 &      6.36 &      8.07 &   \nodata &      7.29 &     13.17 &     30.26 &     21.45 &   \nodata &      8.70 &   \nodata &     37.04 \\
 5753.122 &      Fe I &      4.26 &   $-$0.69 &     67.87 &     30.46 &     36.21 &      5.56 &     37.65 &     56.69 &     79.33 &     52.63 &     40.76 &     41.62 &   \nodata &     73.87 \\
 5775.080 &      Fe I &      4.22 &   $-$1.31 &     49.45 &     16.43 &     17.11 &   \nodata &     18.36 &     31.01 &     57.83 &     32.48 &     24.23 &     28.09 &   \nodata &     54.07 \\
 5778.450 &      Fe I &      2.59 &   $-$3.48 &     27.54 &     11.71 &   \nodata &   \nodata &     13.01 &     21.57 &     34.65 &     18.28 &   \nodata &   \nodata &   \nodata &   \nodata \\
 5816.373 &      Fe I &      4.55 &   $-$0.60 &     57.98 &     19.77 &     24.35 &   \nodata &     22.05 &     36.81 &     76.73 &     39.38 &     28.31 &     27.16 &   \nodata &     66.05 \\
 5909.970 &      Fe I &      3.21 &   $-$2.64 &     38.10 &      8.45 &     10.15 &   \nodata &     27.72 &     30.41 &     49.38 &     17.12 &   \nodata &      9.05 &   \nodata &     53.36 \\
 5916.250 &      Fe I &      2.45 &   $-$2.99 &     77.71 &   \nodata &     27.90 &   \nodata &     49.08 &     70.07 &     75.23 &     40.35 &     41.21 &     29.73 &   \nodata &     55.09 \\
 5927.800 &      Fe I &      4.65 &   $-$1.09 &     26.98 &      7.92 &     10.27 &   \nodata &      7.95 &     12.58 &     34.58 &     35.18 &   \nodata &   \nodata &   \nodata &     48.08 \\
 5956.690 &      Fe I &      0.86 &   $-$4.61 &     90.94 &     38.31 &     11.72 &     13.46 &     79.65 &    100.74 &     87.72 &     50.20 &     64.68 &     42.79 &   \nodata &   \nodata \\
 6012.210 &      Fe I &      2.22 &   $-$4.07 &     27.74 &      8.87 &   \nodata &   \nodata &     15.38 &     23.96 &     28.96 &     10.68 &   \nodata &   \nodata &   \nodata &     40.11 \\
 6027.050 &      Fe I &      4.07 &   $-$1.11 &     57.34 &     23.51 &     24.19 &   \nodata &     26.92 &     40.54 &     69.66 &     36.72 &     27.46 &     19.99 &   \nodata &     79.17 \\
 6065.481 &      Fe I &      2.61 &   $-$1.41 &   \nodata &   \nodata &     71.05 &     45.26 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     49.77 &   \nodata \\
 6136.615 &      Fe I &      2.45 &   $-$1.41 &   \nodata &   \nodata &   \nodata &     71.83 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     67.94 &   \nodata \\
 6137.691 &      Fe I &      2.59 &   $-$1.35 &   \nodata &   \nodata &   \nodata &     60.48 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     62.85 &   \nodata \\
 6151.618 &      Fe I &      2.18 &   $-$3.37 &     67.85 &     24.80 &     11.81 &   \nodata &     45.36 &     67.11 &     67.33 &     40.06 &     43.72 &     24.92 &   \nodata &     52.07 \\
 6157.730 &      Fe I &      4.08 &   $-$1.32 &     58.67 &     21.31 &     19.44 &   \nodata &     26.74 &     44.44 &     66.87 &     38.90 &     28.55 &     24.28 &   \nodata &     59.50 \\
 6159.380 &      Fe I &      4.61 &   $-$1.97 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &      8.99 &      8.98 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6165.360 &      Fe I &      4.14 &   $-$1.49 &     31.97 &      9.00 &     10.84 &   \nodata &     11.37 &     20.65 &     42.85 &     18.63 &     12.88 &   \nodata &   \nodata &     41.34 \\
 6173.340 &      Fe I &      2.22 &   $-$2.88 &     91.13 &     40.87 &     25.29 &      9.64 &     72.47 &     90.73 &     92.88 &     56.91 &     62.26 &     41.78 &   \nodata &     77.93 \\
 6180.200 &      Fe I &      2.73 &   $-$2.64 &     66.39 &     23.17 &     15.83 &   \nodata &     40.03 &     61.57 &     74.65 &     35.27 &     34.33 &     25.79 &   \nodata &     72.84 \\
 6191.558 &      Fe I &      2.43 &   $-$1.42 &   \nodata &   \nodata &   \nodata &     67.71 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     63.85 &   \nodata \\
 6200.310 &      Fe I &      2.61 &   $-$2.44 &     88.62 &     43.11 &     28.22 &     11.18 &     67.12 &     86.59 &     92.75 &     69.45 &     61.92 &     41.78 &   \nodata &     82.83 \\
 6213.429 &      Fe I &      2.22 &   $-$2.48 &    107.54 &     61.79 &     41.11 &     23.51 &     93.95 &    111.54 &    109.17 &     71.71 &     84.28 &     66.59 &     22.93 &     94.27 \\
 6219.280 &      Fe I &      2.20 &   $-$2.43 &    113.53 &     67.71 &     48.24 &     32.98 &    101.22 &    117.85 &    115.36 &     77.32 &     97.62 &     76.70 &     20.51 &   \nodata \\
 6229.230 &      Fe I &      2.84 &   $-$2.85 &     44.09 &     13.17 &      8.36 &   \nodata &     23.22 &     36.04 &     49.39 &     17.07 &     22.40 &     21.05 &   \nodata &     31.27 \\
 6230.723 &      Fe I &      2.56 &   $-$1.28 &   \nodata &   \nodata &   \nodata &     72.14 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     68.73 &   \nodata \\
 6232.640 &      Fe I &      3.65 &   $-$1.28 &     79.53 &     36.48 &     34.71 &      9.83 &     51.00 &     69.17 &     88.45 &     54.37 &     54.42 &     38.86 &   \nodata &     92.42 \\
 6240.645 &      Fe I &      2.22 &   $-$3.17 &     68.60 &     23.17 &     12.37 &   \nodata &     45.22 &     65.15 &     70.87 &     37.35 &     45.40 &     23.80 &   \nodata &     59.74 \\
 6246.320 &      Fe I &      3.60 &   $-$0.89 &    103.07 &     63.50 &     62.45 &     18.33 &     82.33 &     97.99 &    112.75 &     87.27 &     77.73 &     64.29 &     22.53 &   \nodata \\
 6252.555 &      Fe I &      2.40 &   $-$1.69 &   \nodata &   \nodata &     73.89 &     62.50 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     50.81 &   \nodata \\
 6254.257 &      Fe I &      2.28 &   $-$2.44 &    123.51 &     73.81 &     61.72 &     26.43 &    102.35 &    119.97 &   \nodata &     84.85 &     94.58 &     76.08 &     27.65 &   \nodata \\
 6265.130 &      Fe I &      2.17 &   $-$2.55 &    109.59 &     67.71 &     43.60 &     33.58 &     97.18 &    114.32 &    114.91 &     79.37 &     91.61 &     73.90 &   \nodata &   \nodata \\
 6270.220 &      Fe I &      2.86 &   $-$2.50 &   \nodata &     20.19 &     14.27 &   \nodata &     38.87 &     53.86 &     68.21 &     39.73 &     34.69 &   \nodata &   \nodata &     78.20 \\
 6271.280 &      Fe I &      3.33 &   $-$2.73 &   \nodata &      4.13 &      3.85 &   \nodata &     10.67 &     16.14 &     27.05 &      8.63 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6301.499 &      Fe I &      3.65 &   $-$0.72 &    104.47 &     62.41 &     61.66 &     18.08 &     80.26 &     96.74 &    115.51 &     83.90 &   \nodata &     78.58 &   \nodata &   \nodata \\
 6322.684 &      Fe I &      2.59 &   $-$2.47 &     89.66 &     44.99 &     29.64 &     11.28 &     71.50 &     88.94 &     92.87 &     60.37 &     59.24 &     44.58 &   \nodata &     71.50 \\
 6335.330 &      Fe I &      2.20 &   $-$2.18 &    120.99 &   \nodata &     58.09 &     42.84 &    114.70 &   \nodata &    124.11 &     88.62 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6336.835 &      Fe I &      3.69 &   $-$1.05 &     95.25 &     56.56 &     53.31 &     11.80 &     70.52 &     89.37 &    105.82 &     71.14 &     72.51 &     59.81 &   \nodata &     96.94 \\
 6344.148 &      Fe I &      2.43 &   $-$2.88 &     83.53 &     30.86 &     21.83 &   \nodata &     56.26 &     74.06 &     85.29 &     44.74 &     48.14 &     38.63 &   \nodata &     77.23 \\
 6355.030 &      Fe I &      2.84 &   $-$2.40 &     84.23 &     33.96 &     25.11 &   \nodata &     54.51 &     73.78 &     93.42 &     54.40 &     53.32 &     40.66 &   \nodata &     89.31 \\
 6393.601 &      Fe I &      2.43 &   $-$1.58 &   \nodata &   \nodata &   \nodata &     66.06 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     56.44 &   \nodata \\
 6400.000 &      Fe I &      3.60 &   $-$0.29 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     62.01 &   \nodata \\
 6411.649 &      Fe I &      3.65 &   $-$0.59 &    110.66 &     72.25 &     69.20 &     22.65 &     89.26 &    106.20 &    121.17 &     97.62 &     89.13 &     71.02 &     23.93 &   \nodata \\
 6421.350 &      Fe I &      2.28 &   $-$2.01 &   \nodata &   \nodata &     66.87 &     48.91 &    123.94 &   \nodata &   \nodata &     99.68 &   \nodata &   \nodata &     42.74 &   \nodata \\
 6430.846 &      Fe I &      2.18 &   $-$1.95 &   \nodata &   \nodata &     70.33 &     59.23 &   \nodata &   \nodata &   \nodata &    101.70 &   \nodata &   \nodata &     58.93 &   \nodata \\
 6469.190 &      Fe I &      4.84 &   $-$0.77 &   \nodata &     15.55 &     11.99 &   \nodata &   \nodata &     22.85 &     53.45 &     29.67 &   \nodata &     13.34 &   \nodata &     45.68 \\
 6494.980 &      Fe I &      2.40 &   $-$1.24 &   \nodata &   \nodata &   \nodata &     85.84 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     84.87 &   \nodata \\
 6498.940 &      Fe I &      0.96 &   $-$4.70 &     85.46 &     30.43 &     11.10 &      8.77 &     75.92 &     88.68 &     80.85 &     41.80 &     52.32 &     30.76 &   \nodata &     71.47 \\
 6574.230 &      Fe I &      0.99 &   $-$5.00 &     64.55 &     14.26 &   \nodata &   \nodata &     46.55 &     66.16 &     56.43 &     19.62 &     36.38 &     18.49 &   \nodata &     56.45 \\
 6575.020 &      Fe I &      2.59 &   $-$2.73 &     78.96 &     28.43 &     14.95 &   \nodata &     52.78 &     89.96 &     95.51 &     47.88 &     51.99 &     26.31 &   \nodata &     76.35 \\
 6592.912 &      Fe I &      2.73 &   $-$1.47 &    130.15 &   \nodata &     66.41 &     42.39 &    115.64 &    129.47 &   \nodata &    100.01 &   \nodata &   \nodata &     39.38 &   \nodata \\
 6593.868 &      Fe I &      2.44 &   $-$2.37 &    104.75 &     57.89 &     40.63 &     15.43 &     89.08 &    104.53 &    110.78 &     66.85 &     79.04 &     60.90 &     15.02 &     86.51 \\
 6609.109 &      Fe I &      2.56 &   $-$2.66 &     81.80 &     33.93 &     21.79 &      6.88 &     58.11 &     77.61 &     86.68 &     48.38 &     51.96 &     36.93 &      9.84 &     78.42 \\
 6663.440 &      Fe I &      2.42 &   $-$2.48 &    113.58 &     59.69 &     43.19 &     20.21 &     91.42 &    112.15 &    130.08 &     82.50 &     85.64 &     65.07 &     15.48 &   \nodata \\
 6677.986 &      Fe I &      2.69 &   $-$1.42 &   \nodata &   \nodata &     75.81 &     51.38 &    127.92 &   \nodata &   \nodata &    101.66 &   \nodata &   \nodata &     52.39 &   \nodata \\
 6739.520 &      Fe I &      1.56 &   $-$4.82 &     24.81 &   \nodata &   \nodata &   \nodata &     12.72 &     22.25 &     19.75 &     12.29 &   \nodata &   \nodata &   \nodata &     17.53 \\
 6750.152 &      Fe I &      2.42 &   $-$2.58 &     92.85 &     48.20 &     31.09 &     14.16 &     78.78 &     96.18 &     95.72 &     66.68 &     73.12 &     54.00 &     21.47 &     88.12 \\
 6810.260 &      Fe I &      4.60 &   $-$1.00 &     30.52 &      9.20 &     14.04 &   \nodata &     10.35 &     19.22 &     42.42 &     32.95 &   \nodata &   \nodata &   \nodata &     41.82 \\
 6971.930 &      Fe I &      3.02 &   $-$3.39 &     15.07 &   \nodata &   \nodata &   \nodata &     11.07 &     12.96 &     17.55 &     13.77 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6978.850 &      Fe I &      2.48 &   $-$2.45 &   \nodata &     51.48 &     35.51 &     18.08 &     97.86 &    103.34 &    112.75 &     66.31 &     76.67 &     54.45 &     22.62 &    108.45 \\
 7112.170 &      Fe I &      2.99 &   $-$3.04 &     35.31 &   \nodata &   \nodata &   \nodata &     15.97 &     26.88 &     35.96 &     20.28 &   \nodata &   \nodata &   \nodata &   \nodata \\
 7223.660 &      Fe I &      3.01 &   $-$2.27 &     74.07 &     34.57 &     20.70 &   \nodata &     44.63 &   \nodata &   \nodata &     36.06 &     39.60 &     23.02 &   \nodata &     64.11 \\
 7401.690 &      Fe I &      4.18 &   $-$1.66 &     30.99 &      9.46 &      9.17 &   \nodata &   \nodata &     18.71 &     40.32 &     23.88 &      7.80 &   \nodata &   \nodata &     31.85 \\
 7710.360 &      Fe I &      4.22 &   $-$1.13 &     53.54 &     18.77 &     24.83 &   \nodata &     27.04 &     47.40 &     70.61 &     44.45 &     33.75 &   \nodata &   \nodata &   \nodata \\
 7723.200 &      Fe I &      2.28 &   $-$3.62 &     54.35 &     18.97 &     12.20 &   \nodata &     39.17 &     55.14 &     58.92 &     37.81 &     40.57 &   \nodata &   \nodata &     59.76 \\
 7941.090 &      Fe I &      3.27 &   $-$2.33 &     39.56 &   \nodata &     10.55 &   \nodata &     23.43 &     33.26 &     48.87 &     22.36 &     21.79 &   \nodata &   \nodata &     43.78 \\
 4128.748 &     Fe II &      2.58 &   $-$3.47 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     34.81 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4178.860 &     Fe II &      2.58 &   $-$2.51 &   \nodata &   \nodata &   \nodata &     55.18 &   \nodata &   \nodata &   \nodata &     58.28 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4233.170 &     Fe II &      2.58 &   $-$1.97 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     90.71 &   \nodata \\
 4416.817 &     Fe II &      2.78 &   $-$2.60 &   \nodata &   \nodata &   \nodata &     45.12 &   \nodata &   \nodata &   \nodata &     64.95 &   \nodata &   \nodata &     49.37 &   \nodata \\
 4489.185 &     Fe II &      2.83 &   $-$2.97 &   \nodata &   \nodata &     55.65 &     25.98 &   \nodata &   \nodata &   \nodata &     70.52 &   \nodata &   \nodata &   \nodata &   \nodata \\
 4491.410 &     Fe II &      2.86 &   $-$2.71 &     77.05 &   \nodata &     50.28 &     32.30 &     69.65 &     76.52 &   \nodata &     56.37 &   \nodata &   \nodata &     35.71 &     69.88 \\
 4508.283 &     Fe II &      2.86 &   $-$2.58 &   \nodata &   \nodata &   \nodata &     53.13 &   \nodata &   \nodata &   \nodata &     64.73 &   \nodata &   \nodata &     62.51 &   \nodata \\
 4515.340 &     Fe II &      2.84 &   $-$2.60 &   \nodata &   \nodata &   \nodata &     45.69 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     54.03 &   \nodata \\
 4520.224 &     Fe II &      2.81 &   $-$2.60 &   \nodata &   \nodata &   \nodata &     42.73 &   \nodata &   \nodata &   \nodata &     67.39 &   \nodata &   \nodata &     45.60 &   \nodata \\
 4541.523 &     Fe II &      2.86 &   $-$3.05 &   \nodata &     54.68 &     45.28 &     24.44 &   \nodata &   \nodata &   \nodata &     51.25 &   \nodata &   \nodata &     29.11 &   \nodata \\
 4555.890 &     Fe II &      2.83 &   $-$2.40 &   \nodata &   \nodata &   \nodata &     57.29 &   \nodata &   \nodata &   \nodata &     71.15 &   \nodata &   \nodata &     59.12 &   \nodata \\
 4576.340 &     Fe II &      2.84 &   $-$2.95 &     72.79 &     48.59 &     41.76 &     22.70 &     63.02 &     71.26 &     81.44 &     55.56 &     60.37 &     57.25 &     27.27 &     68.79 \\
 4583.840 &     Fe II &      2.81 &   $-$1.93 &   \nodata &   \nodata &   \nodata &     81.24 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     97.86 &   \nodata \\
 4620.520 &     Fe II &      2.83 &   $-$3.21 &     55.66 &     33.09 &     27.47 &     13.37 &     42.37 &     52.08 &     66.94 &     30.43 &     52.18 &     40.91 &   \nodata &   \nodata \\
 4731.439 &     Fe II &      2.89 &   $-$3.36 &   \nodata &     46.94 &     41.00 &     16.13 &   \nodata &   \nodata &   \nodata &     57.96 &     59.44 &   \nodata &   \nodata &   \nodata \\
 4923.930 &     Fe II &      2.89 &   $-$1.32 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    107.38 &   \nodata \\
 4993.360 &     Fe II &      2.80 &   $-$3.48 &   \nodata &   \nodata &     16.23 &   \nodata &   \nodata &   \nodata &     45.57 &     22.37 &     41.42 &     31.95 &   \nodata &     50.43 \\
 5197.580 &     Fe II &      3.23 &   $-$2.22 &     90.24 &     65.33 &     60.61 &     50.89 &     78.68 &     91.06 &    103.68 &     57.20 &   \nodata &     64.84 &     36.89 &   \nodata \\
 5234.630 &     Fe II &      3.22 &   $-$2.18 &     88.56 &   \nodata &     63.66 &     39.69 &     79.21 &     89.53 &    101.29 &     69.41 &   \nodata &   \nodata &     43.80 &   \nodata \\
 5276.000 &     Fe II &      3.20 &   $-$2.01 &   \nodata &   \nodata &   \nodata &     59.65 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     62.58 &   \nodata \\
 5284.080 &     Fe II &      2.89 &   $-$3.19 &     63.70 &     41.12 &     35.48 &     16.23 &   \nodata &     57.34 &   \nodata &     39.05 &     57.54 &     36.48 &     19.80 &     72.08 \\
 5325.550 &     Fe II &      3.22 &   $-$3.22 &     40.90 &     20.88 &     22.65 &      8.71 &     29.16 &     38.13 &     57.34 &     24.65 &     44.31 &   \nodata &   \nodata &     73.82 \\
 5425.260 &     Fe II &      3.20 &   $-$3.37 &     36.80 &     21.69 &     18.65 &   \nodata &     28.41 &     33.63 &     50.20 &     25.00 &     33.55 &     28.26 &   \nodata &     45.26 \\
 5534.834 &     Fe II &      3.25 &   $-$2.93 &     62.38 &     41.72 &     38.90 &     20.13 &     50.89 &     61.92 &     80.26 &     48.01 &     63.06 &   \nodata &   \nodata &     59.35 \\
 5991.380 &     Fe II &      3.15 &   $-$3.56 &     30.02 &     14.28 &     12.68 &   \nodata &     17.10 &     29.77 &     39.25 &     20.79 &     22.64 &     16.98 &   \nodata &   \nodata \\
 6084.110 &     Fe II &      3.20 &   $-$3.81 &     18.37 &     10.85 &      7.74 &   \nodata &     12.08 &     16.73 &     28.21 &     13.71 &     13.10 &   \nodata &   \nodata &   \nodata \\
 6149.260 &     Fe II &      3.89 &   $-$2.72 &     27.30 &     15.62 &     16.15 &   \nodata &     18.59 &     25.04 &     41.11 &     23.41 &     25.02 &     27.61 &   \nodata &     47.66 \\
 6369.460 &     Fe II &      2.89 &   $-$4.25 &     17.80 &     10.40 &   \nodata &   \nodata &     13.01 &     16.38 &     24.55 &     10.12 &   \nodata &   \nodata &   \nodata &     22.66 \\
 6416.920 &     Fe II &      3.89 &   $-$2.74 &     29.90 &     13.55 &     17.24 &   \nodata &     16.93 &     23.89 &     41.08 &     24.00 &     21.39 &     18.36 &   \nodata &   \nodata \\
 6432.680 &     Fe II &      2.89 &   $-$3.71 &     42.05 &     23.45 &     18.75 &      7.28 &     31.11 &     39.29 &     54.87 &     22.28 &     33.13 &     37.16 &     15.80 &     47.21 \\
 6456.380 &     Fe II &      3.90 &   $-$2.08 &     57.22 &     40.03 &     43.25 &     11.45 &     47.50 &     51.87 &     71.98 &     42.26 &     50.77 &     46.87 &   \nodata &     53.32 \\
 7711.720 &     Fe II &      3.90 &   $-$2.54 &     33.56 &     25.78 &     25.61 &      7.41 &     32.79 &     35.06 &     51.35 &     32.79 &     38.50 &     30.30 &   \nodata &     37.53 \\
 3995.306 &      Co I &      0.92 &   $-$0.22 &    166.58 &    108.31 &     93.05 &     86.47 &    146.52 &    153.01 &    168.31 &    108.10 &    111.51 &    117.56 &     65.60 &    134.30 \\
 4020.898 &      Co I &      0.43 &   $-$2.07 &   \nodata &     69.19 &     31.68 &     40.23 &    107.41 &    116.40 &   \nodata &     71.54 &   \nodata &     58.76 &   \nodata &    111.37 \\
 4110.532 &      Co I &      1.05 &   $-$1.08 &   \nodata &   \nodata &     41.45 &     39.29 &   \nodata &   \nodata &   \nodata &     89.23 &    105.49 &     71.30 &     33.70 &    133.17 \\
 4118.767 &      Co I &      1.05 &   $-$0.49 &   \nodata &   \nodata &   \nodata &     83.37 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4121.318 &      Co I &      0.92 &   $-$0.32 &    153.18 &    106.33 &     88.96 &     92.98 &    143.69 &    152.85 &    158.42 &    103.11 &    118.46 &    122.59 &    116.06 &   \nodata \\
 6189.000 &      Co I &      1.71 &   $-$2.45 &     22.97 &   \nodata &   \nodata &   \nodata &     11.95 &     20.80 &     27.65 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6455.030 &      Co I &      3.63 &   $-$0.25 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &      7.47 &     20.01 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6632.450 &      Co I &      2.28 &   $-$2.00 &     12.87 &   \nodata &   \nodata &   \nodata &   \nodata &     11.33 &     20.12 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 3807.140 &      Ni I &      0.42 &   $-$1.22 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    165.99 &    208.38 &    146.24 &    123.46 &   \nodata \\
 3858.301 &      Ni I &      0.42 &   $-$0.95 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    191.30 &   \nodata &   \nodata &    143.33 &   \nodata \\
 4605.000 &      Ni I &      3.48 &   $-$0.29 &     80.98 &     38.78 &     39.69 &     12.11 &     47.97 &     63.77 &     97.72 &     46.59 &     38.40 &     31.21 &   \nodata &   \nodata \\
 4648.659 &      Ni I &      3.42 &   $-$0.16 &     82.81 &     46.99 &     50.79 &     20.02 &     60.53 &     74.42 &     93.05 &     57.12 &     54.78 &   \nodata &   \nodata &   \nodata \\
 4686.220 &      Ni I &      3.60 &   $-$0.64 &     48.56 &     17.78 &     21.81 &      4.63 &     22.04 &     32.23 &     67.44 &     30.32 &     19.90 &   \nodata &   \nodata &     53.63 \\
 4714.421 &      Ni I &      3.38 &      0.23 &   \nodata &     75.28 &     75.90 &     31.20 &     89.06 &    104.04 &   \nodata &     91.62 &     85.24 &     85.11 &     36.26 &    129.33 \\
 4904.410 &      Ni I &      3.54 &   $-$0.17 &     79.06 &     41.76 &     45.28 &     16.83 &     55.61 &     68.37 &     94.10 &     63.35 &     59.11 &     37.49 &   \nodata &     98.41 \\
 4980.161 &      Ni I &      3.61 &   $-$0.11 &     91.46 &     51.90 &     54.02 &     17.80 &     61.80 &     76.06 &   \nodata &     81.01 &     60.78 &     51.44 &   \nodata &     86.99 \\
 5017.591 &      Ni I &      3.54 &   $-$0.08 &     77.85 &     46.31 &     46.92 &     17.50 &     53.69 &     67.70 &     95.90 &     60.80 &     48.07 &     43.54 &   \nodata &    102.71 \\
 5035.374 &      Ni I &      3.63 &      0.29 &   \nodata &     54.50 &     57.54 &     23.90 &     62.32 &     69.82 &     96.38 &     68.75 &     67.31 &     56.64 &     24.00 &     87.51 \\
 5080.523 &      Ni I &      3.65 &      0.13 &   \nodata &     59.70 &     64.98 &     24.91 &     76.25 &     92.37 &   \nodata &     89.71 &     71.92 &     59.28 &   \nodata &   \nodata \\
 5081.110 &      Ni I &      3.85 &      0.30 &     88.55 &     45.90 &     52.22 &     19.64 &     59.06 &     76.39 &    101.76 &     65.93 &     58.59 &     49.88 &   \nodata &     91.21 \\
 5084.080 &      Ni I &      3.68 &      0.03 &     69.10 &     41.10 &     46.97 &     13.73 &     50.27 &     61.10 &     84.33 &     58.63 &     51.88 &     52.55 &   \nodata &     61.94 \\
 5115.400 &      Ni I &      3.83 &   $-$0.11 &     57.72 &     28.22 &     36.35 &   \nodata &     32.32 &     46.36 &     76.99 &     38.17 &     36.01 &     29.65 &   \nodata &     59.22 \\
 5137.075 &      Ni I &      1.68 &   $-$1.99 &   \nodata &   \nodata &     49.79 &     38.53 &   \nodata &   \nodata &   \nodata &     74.64 &     96.75 &     72.91 &   \nodata &     84.59 \\
 5155.760 &      Ni I &      3.90 &   $-$0.09 &     63.91 &     30.16 &     34.97 &      9.51 &     32.51 &     43.02 &     78.36 &     57.26 &     38.75 &   \nodata &   \nodata &     44.12 \\
 5476.900 &      Ni I &      1.83 &   $-$0.89 &   \nodata &   \nodata &    101.17 &     92.06 &    151.42 &    165.98 &    182.80 &    132.55 &    139.50 &    118.25 &     81.75 &   \nodata \\
 5578.734 &      Ni I &      1.68 &   $-$2.64 &     74.58 &     29.02 &     16.36 &     10.24 &     53.40 &     70.61 &     84.74 &     39.21 &     43.76 &     32.37 &   \nodata &     49.79 \\
 5754.675 &      Ni I &      1.94 &   $-$2.33 &   \nodata &     44.04 &     28.95 &     13.20 &     73.17 &     92.30 &   \nodata &     55.45 &     56.52 &     41.77 &   \nodata &     65.05 \\
 5846.990 &      Ni I &      1.68 &   $-$3.21 &     33.46 &      8.29 &      6.18 &   \nodata &     19.96 &     27.46 &     40.85 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6086.280 &      Ni I &      4.26 &   $-$0.52 &     20.40 &      8.97 &     10.79 &   \nodata &      9.72 &     15.26 &     39.53 &     21.32 &   \nodata &   \nodata &   \nodata &   \nodata \\
 6108.121 &      Ni I &      1.68 &   $-$2.45 &     85.23 &     38.40 &     21.98 &     13.06 &     68.42 &     85.54 &     95.68 &     45.19 &     56.28 &     39.38 &   \nodata &     79.37 \\
 6175.370 &      Ni I &      4.09 &   $-$0.54 &     32.73 &      9.13 &     13.85 &   \nodata &     11.35 &     19.43 &     47.60 &     22.51 &   \nodata &     11.93 &   \nodata &     29.50 \\
 6177.240 &      Ni I &      1.83 &   $-$3.51 &     18.05 &      5.80 &   \nodata &   \nodata &      9.46 &     15.53 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6204.600 &      Ni I &      4.09 &   $-$1.14 &     11.00 &   \nodata &      5.25 &   \nodata &   \nodata &   \nodata &     23.93 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6635.120 &      Ni I &      4.42 &   $-$0.83 &     11.85 &   \nodata &   \nodata &   \nodata &   \nodata &      5.13 &     21.45 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6643.640 &      Ni I &      1.68 &   $-$2.30 &   \nodata &     65.21 &     41.54 &     32.41 &    105.08 &    117.76 &    127.52 &     79.15 &     87.95 &     65.36 &   \nodata &    107.25 \\
 6767.770 &      Ni I &      1.83 &   $-$2.17 &     98.51 &     55.96 &     38.24 &     22.99 &     92.42 &    103.23 &    109.09 &     60.31 &     74.11 &     50.15 &   \nodata &     83.51 \\
 6772.320 &      Ni I &      3.66 &   $-$0.99 &     39.67 &     10.96 &     14.29 &   \nodata &     17.38 &     26.44 &     56.30 &     27.41 &     18.15 &      9.18 &   \nodata &   \nodata \\
 5105.540 &      Cu I &      1.39 &   $-$1.52 &     96.29 &     32.36 &     24.72 &   \nodata &     60.71 &     84.14 &    120.53 &     53.85 &     29.56 &     20.38 &     15.20 &     73.77 \\
 4722.150 &      Zn I &      4.03 &   $-$0.39 &     63.35 &     43.59 &     41.89 &     17.07 &     48.01 &     48.71 &     84.48 &     50.23 &     39.48 &     40.86 &   \nodata &     67.35 \\
 4810.528 &      Zn I &      4.08 &   $-$0.14 &     68.76 &     45.32 &     49.43 &     19.22 &     47.31 &     54.13 &     92.42 &     46.89 &     35.76 &   \nodata &   \nodata &   \nodata \\
%7800.290 &      Rb I &      0.00 &      0.13 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
%4077.714 &     Sr II &      0.00 &      0.15 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4215.524 &     Sr II &      0.00 &   $-$0.18 &    344.50 &    228.55 &    196.85 &    155.19 &    284.60 &    325.80 &    393.31 &    234.56 &    215.45 &    171.82 &    156.61 &    319.51 \\
 5123.220 &      Y II &      0.99 &   $-$0.83 &   \nodata &     25.78 &     14.63 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     64.09 \\
 5200.420 &      Y II &      0.99 &   $-$0.57 &     66.75 &     35.34 &     20.28 &     22.81 &     56.38 &     58.90 &     65.51 &     21.71 &   \nodata &   \nodata &   \nodata &   \nodata \\
 5509.910 &      Y II &      0.99 &   $-$1.01 &     60.03 &     23.41 &   \nodata &   \nodata &     33.96 &     44.58 &     74.50 &     31.48 &   \nodata &   \nodata &   \nodata &   \nodata \\
 5544.610 &      Y II &      1.74 &   $-$1.08 &     10.39 &   \nodata &   \nodata &   \nodata &      6.99 &      8.75 &     14.24 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6127.440 &      Zr I &      0.15 &   $-$1.06 &      6.26 &   \nodata &   \nodata &   \nodata &   \nodata &      4.50 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6134.550 &      Zr I &      0.00 &   $-$1.28 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &      5.17 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6143.200 &      Zr I &      0.07 &   $-$1.10 &      7.20 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5112.270 &     Zr II &      1.67 &   $-$0.59 &     25.91 &      7.96 &      5.27 &   \nodata &     17.55 &     23.64 &     19.13 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4554.033 &     Ba II &      0.00 &      0.16 &    215.02 &    162.60 &    134.68 &     99.19 &    217.03 &    227.68 &    198.34 &    159.86 &    174.56 &    143.84 &     90.65 &    221.48 \\
 4934.086 &     Ba II &      0.00 &   $-$0.16 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &    100.03 &   \nodata \\
 5853.640 &     Ba II &      0.60 &   $-$1.01 &     99.15 &     68.79 &     44.06 &      9.17 &    102.42 &    111.30 &     96.01 &     66.40 &     67.25 &     43.54 &   \nodata &    103.04 \\
 5805.770 &     La II &      0.13 &   $-$1.56 &     20.21 &      7.01 &      3.10 &   \nodata &     16.22 &     20.08 &     16.58 &   \nodata &   \nodata &   \nodata &   \nodata &     29.27 \\
 6390.480 &     La II &      0.32 &   $-$1.41 &     16.32 &      6.29 &   \nodata &   \nodata &     13.19 &     13.82 &     10.32 &   \nodata &   \nodata &     10.47 &   \nodata &   \nodata \\
%4943.450 &     Ce II &      1.20 &   $-$0.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5274.240 &     Ce II &      1.04 &   $-$0.32 &   \nodata &   \nodata &   \nodata &   \nodata &     12.69 &     18.65 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5472.300 &     Ce II &      1.24 &   $-$0.18 &   \nodata &   \nodata &   \nodata &   \nodata &      4.05 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
%5512.060 &     Ce II &      1.00 &      0.29 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 4959.120 &     Nd II &      0.06 &   $-$0.80 &     54.95 &     17.69 &      8.14 &   \nodata &     47.54 &     55.87 &     45.02 &     37.96 &     15.95 &     26.67 &   \nodata &   \nodata \\
 5092.790 &     Nd II &      0.38 &   $-$0.61 &   \nodata &     12.36 &   \nodata &   \nodata &     30.89 &     33.09 &   \nodata &   \nodata &     14.63 &   \nodata &   \nodata &   \nodata \\
 5212.360 &     Nd II &      0.20 &   $-$0.96 &     37.84 &      6.49 &   \nodata &   \nodata &     25.65 &     32.72 &     25.07 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5234.190 &     Nd II &      0.55 &   $-$0.51 &     31.86 &      8.46 &   \nodata &   \nodata &     26.13 &     32.60 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &     51.74 \\
 5249.580 &     Nd II &      0.98 &      0.20 &     45.08 &     17.66 &   \nodata &   \nodata &     32.29 &     39.87 &     40.70 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5255.510 &     Nd II &      0.20 &   $-$0.67 &   \nodata &     19.04 &   \nodata &   \nodata &     45.79 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 5293.160 &     Nd II &      0.82 &      0.10 &     49.19 &   \nodata &      7.51 &   \nodata &     37.22 &     45.26 &     37.58 &   \nodata &   \nodata &   \nodata &   \nodata &     65.78 \\
 5319.810 &     Nd II &      0.55 &   $-$0.14 &     61.00 &     17.03 &      6.79 &   \nodata &     42.39 &     45.11 &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata &   \nodata \\
 6645.110 &     Eu II &      1.38 &      0.20 &     26.67 &      4.62 &   \nodata &   \nodata &     16.10 &     18.73 &     22.18 &   \nodata &   \nodata &   \nodata &   \nodata &     33.31 \\
\hline
\end{longtable}
\end{center}
\end{landscape}

==> dedication.tex <==
\begin{figure}
\centering
{\large\usefont{OT1}{qzc}{m}{n}\selectfont 
%To my cat, Mr Smigglesworth\dots
\\[4cm]\phantom{1}}
\end{figure}


==> introduction/introduction.tex <==
\chapter{Introduction}\label{sec:introduction}

\epigraph{Given enough time, hydrogen starts to wonder where it came from, and where it is going.}{-- Edward R. Harrison}

The creation of the Universe gave birth to space-time and the laws of nature. A rapid exponential expansion transpired a mere picosecond after the big bang, smoothing out all previous structure in the Universe with the exception of quantum-scale fluctuations \citep[e.g.,][]{guth_1997}. Over time, these fluctuations resulted in cold dark matter (CDM) density perturbations, causing minuscule gravitational potential wells. This process furnished the Universe with the seeds required to build cosmological structure \citep{liddle;lyth_2000,springel;et-al_2005}. Baryonic matter followed the influence of the gravitational field  \citep[$z \sim 200$;][]{rees_1986}, and subsequently began to condense into primordial gas clouds of Hydrogen, Helium, as well as trace elements of Deuterium and Lithium \citep{2004PhLB..592....1P}.

A prolonged, quiescent period followed. The first stars didn't start to form until after $\sim$200 Myr \citep{bromm;et-al_1999,abel;et-al_2002,barkana;loeb_2007}, when primordial gas had sufficiently cooled. The first (so-called Population III) stars had limited cooling capability, and were subsequently were massive \citep[$\sim$10$-100 M_\odot$;][]{bromm;yoshida_2011} and  short-lived \citep{yoshida;et-al_2004,gao;theuns_2007}. They were metal-free\footnote{Following the inexplicable tradition of astronomers, the term `metals' describes elements heavier than He.}, and extremely turbulent \citep{bromm;yoshida_2011}. Given their size, it is unlikely any such objects have survived to the present day \citep{loeb_2010}, and no such object has been found. These objects filled the interstellar medium with the first nucleosynthetic products through their spectacular deaths. The chemically-enriched gas ultimately condensed to initiate the next cycle of star formation \citep[for a review, see][]{bromm;yoshida_2011}. Unlike most stars observable today, which are the product of many hundreds of supernovae, these stars formed from the nucleosynthetic products of a single star. Since the explosive deaths of the Population III stars, successive cycles of star formation have continued to enrich the interstellar medium until the present day. Initially, this chemical enrichment occurred largely independently in each initial potential wells. As time passed, baryonic matter within seed formation sites conglomerated together to form larger stellar systems, and cosmological structure has continued to build hierarchically in a bottom-up fashion.

While Population III stars are no longer expected to exist, a fraction of their progeny are considered to have stellar masses low enough ($\sim$0.8$M_\odot$) to survive to the present epoch. These stars are particularly rare, and provide us a view of the early Universe. With the exception of C, N, O, and Li, the observed stellar abundances (i.e., those in the upper photosphere) remain largely unchanged during a star's lifetime. Regardless of their age, stars are fossilised records containing the chemical composition of their natal gas cloud. While the dynamical information of stars dissipates over time, chemical signatures remain. This permits the use of chemical and dynamical information in stellar groups to be effectively used for the study of galaxy formation and evolution. This was first demonstrated by \citet{eggen;et-al_1962}, which has grown to become the most influential paper of galactic archaeology\footnote{The study of galaxy formation and evolution from observations of fossilised records (e.g., stars).}.

Understanding galaxy formation remains a key goal of astrophysics. This thesis seeks to further our understanding of galaxy formation through the observed motions and chemistry of nearby stars. Most of the stars studied in this thesis have been enriched in different star formation environments before later being accreted onto the Galaxy through hierarchical merging. Thus, these stars posses important information about the merger history of the Milky Way. Throughout this thesis we\footnote{For stylistic reasons I use the plural form throughout this thesis to refer to work led by myself, but naturally performed in collaboration with my supervisors and colleagues. The text however is solely my own.} seek to identify signatures of galaxy formation from these stars, and to chronicle these events in the context of the Milky Way's history. An introduction to hierarchical structure within a context of galaxy formation is provided, and the distinguishable structural components of our Galaxy are discussed in detail. Observational evidence for signatures of galaxy formation is presented, and the accreted stellar groups examined in each chapter are outlined.

\section{History of Hierarchical Structure}

Hierarchical structure formation has grown to become the dominant paradigm since the work of \citet{de_vaucouleurs_1970a}. The preferred $\Lambda$CDM paradigm  proposes structure formation is driven by the effect of the large-scale distribution of CDM. The $\Lambda$CDM paradigm provides simple models of galaxy formation and produces hierarchical structure across cosmic scales as a natural consequence \citep{peebles_1974,white;rees_1978,blumenthal;et-al_1984}. From an observational perspective, the efficiency of multiplexing has enabled redshift surveys to explore the properties of galaxies across cosmic time in great detail \citep[for a review, see][]{mo;et-al_2010}. Within the $\Lambda$CDM paradigm, N-body and semi-analytic models simulating cosmic growth since the early universe have been quite successful at replicating these surveys. Simulations include star formation, gas pressure, radiative cooling and heating, as well as metal production. However an accurate prescription for how baryonic matter produces realistic galaxies within a hierarchy of dark matter is required to fully comprehend galaxy formation.

Observations of Milky Way stars have further aided our understanding of galaxy formation and cosmological structure. \citet{eggen;et-al_1962} was instrumental in demonstrating this link. \citet{eggen;et-al_1962} observed the motions of high velocity stars and found while orbital energies and eccentricities increased, the metal abundance and orbital angular momenta decreased. This implied a metallicity gradient with galactocentric radii. From these data they inferred metal-poor halo stars were created from the rapid collapse of a mostly uniform protogalactic cloud. 

This framework was challenged by \citet{searle;zinn_1978}. Following their observations of globular clusters at a range of galactic radii, \citet{searle;zinn_1978} concluded that globular clusters were found at all metallicities, regardless of their distance to the Galactic center. They suggested the halo could emerge over a long period of time from coalescing gas fragments, each with their own level of independent chemical evolution. Smaller systems would fall into the gravitational potential of larger ones, and become tidally disrupted during this process. This Searle \& Zinn view of galaxy formation was certainly influential, but not entirely new. \citet{searle;zinn_1978} made a noteworthy link with theoretical studies of cosmology and galaxy formation ongoing at the time, where hierarchical aggregation was becoming the preferred interpretation of the time \citep{peebles_1971,press;schechter_1974}. This paradigm has become the accepted dominant formation mechanism for the stellar halo (see Section \ref{sec:stellar-halo}).
 
Observationally, evidence of hierarchical formation remains observable today through the accretion of satellite systems onto the Milky Way. Hundreds of globular clusters and dwarf galaxies orbit our Galaxy \citep{harris_1996}, and many are observed to undergo tidal disruption (c.f. Table \ref{tab:tidal-tails}). This has provided the strongest evidence for the \citet{searle;zinn_1978} paradigm in the stellar halo. Disrupted systems serve as tracers of the Milky Way's merger history, allowing us to reconstruct the chemical and dynamical evolution of the Galaxy, probe the Galactic potential, and explore galaxy formation more generally.


\section{Components of The Milky Way}
Humans are unable to observe the Milky Way with the same context or perspective that we are afforded for other galaxies, making it difficult to distinguish the overall breadth and structure of our Galaxy. This is a natural consequence of our location, yet astronomers remain undeterred. \citet{de_vaucouleurs_1970b} classified the Milky Way as a SAB(rs)bc galaxy: a spiral weakly barred and ringed galaxy. However there is ongoing \citep{urquhart;et-al_2014} debate about whether our Galaxy has 2 or 4 spiral arms, and whether these arms are symmetric. The existence of a central bar has been debated, as well as the interacting effect it would have on the disk. The existence of a thick disk has been brought into question \citep{bovy_2011}, and the warp/flare of the disk has been discussed at length \citep[e.g., see][]{momany_2006}. Generally accepted structural components of the Milky Way include a central bulge/bar, a thin disk, thick disk, a dark matter halo, and a stellar halo. While this thesis focusses on accreted substructure in the Milky Way halo, there is interplay between the structural components of our Galaxy, making it important to introduce these pieces.

\subsection{Bulge}
A concentrated region of stars exists at the very heart of our Galaxy. The Milky Way bulge has a somewhat boxy shape, which are generally seen to have an exponential surface brightness distribution in other galaxies. Bulges in spiral galaxies -- including the Milky Way -- are usually assumed to be old. Color-magnitude diagrams for populations in the Milky Way bulge suggest it is old. The presence of RR Lyrae and metal-poor RGB stars also indicate that at least some fraction of the Milky Way bulge is old. Although a large metallicity range is observed, most stars in the bulge are also predominantly metal-rich. This is seemingly counterintuitive with the expectation that metal-poor stars are fossil remnants of an older stellar population. The old, metal-rich population in the bulge is explainable by rapid metal enrichment at early times, facilitated by extremely short dynamical timescales. Following this intense star formation, mean metallicities around [Fe/H] $\sim -1$ at $z \sim 1$ are not unreasonable.

Cold dark matter simulations suggest the bulge formed via mergers, whereas the boxy/peanut shape of the bulge suggests it has arisen from disk instabilities. A combination of the two mechanisms is also possible. The formation mechanisms that led to the present-day bulge are represented in the dynamics and chemistry of stellar populations still present in the bulge. Recent large-scale spectroscopic surveys targeting the bulge (e.g., the ARGOS survey) have drastically improved our understanding of these formation processes \citep{argosI,argosII,argosIII}. \citet{ness;et-al_2012} find distinct stellar components in the galactic bulge, identifiable by their velocities and metallicities: stars with [Fe/H] $> -0.5$ are claimed to be part of the boxy/peanut bar/bulge, and stars with [Fe/H] $< -0.5$ are associated with the thick disk. Distinct sub-components are also present, and their population gradients across the bulge suggest an instability-driven bar/bulge formation originating from the thin disk. Thus, there is clear interplay between the structural components in the Milky Way since the earliest times of formation, whose signatures remain observable today.

\subsection{The Thin Disk}
The defining component for disk galaxies is the existence of an exponential thin disk. The thin disk is considered as the final product of quiescent dissipation of baryons within a virialized dark matter halo, and contains most of the baryonic angular momenta in the Galaxy \citep{read;et-al_2008}. In the Milky Way, the vertical scale height of the thin disk is $\sim$300\,pc \citep{gilmore;reid_1983}, and the oldest disk stars are observed to be between 10 to 12 gigayears old \citep{oswalt_1996, phelps;et-al_1994}. This is consistent with the disk being almost entirely formed by $z \sim 1$. 

The metallicity of stars in the thin disk varies between [Fe/H] $\sim -0.5$ to $+0.3$ \citep{bensby;et-al_2003}. While the bulge underwent rapid star formation at early times, chromospheric ages of thin disk stars indicate star formation in the thin disk near the Sun has been roughly uniform over the last 10 gigayears, although episodic variations by a factor of 2 are evident \citep{rocha-pinto;et-al_2000}. Five independent surveys aiming to measure the age of the thin disk population find an average of 8.7 $\pm$ 0.4 Gyr \citep{lineweaver_1999}. The presence of an old thin disk suggests that the Galaxy has experienced most of its accretion in early times. The accretion of satellite systems at later times would dynamically heat the thin disk. In fact, the presence of the thick disk (Section \ref{sec:thick-disk}) is perhaps an example of such a thin disk-subhalo  (baryonic or dark) interaction that occurred at early times, dynamically heating the thin disk before it had fully settled. 


\subsection{The Thick Disk}
\label{sec:thick-disk}
In addition to the thin disk, the Milky Way has a second fainter disk component, referred to as the thick disk \citep{gilmore;reid_1983}. The thick disk is much more diffuse than the thin disk. It has a scale height of $\sim$1-1.5\,kpc \citep{reynolds;et-al_1989} -- approximately three times that of the thin disk -- and a surface brightness only 10\% of the thin disk \citep[e.g.,][]{fuhrmann;et-al_2011}. Metallicities for thick disk stars range from [Fe/H] = $-2.2$ to $-0.5$ \citep{reddy;et-al_2006}, considerably more metal-poor than the thin disk.

A thick disk is not an essential element for the formation of disk galaxies. Given the diffusivity of the thick disk compared to the thin disk, detailed chemical abundances are usually necessary to discern the two populations. Stars in the thick disk are typically more metal-poor than stars in the thin disk.

% alpha/Fe in thick/thin discs


\subsection{Stellar Halo}
\label{sec:stellar-halo}
The stellar halo is the largest baryonic component of the Milky Way, extending out to at least 100\,kpc. Although the extent of the stellar halo is large, it is extremely diffuse. The mass of the stellar halo is $\sim$1\% of the total mass, and as such it is not readily observed in other galaxies, as the surface brightness is too low to detect from diffuse light. Most objects in the halo were probably some of the first objects to form, and they remain relics of galaxy formation in the present day.

Many groups have examined the stellar density distribution of the Milky Way, finding that it roughly follows a power law density distribution $\rho \propto r^{-3.5}$ \citep[e.g.,][]{Juric;et-al_2008}. There are substantial offsets in the magnitude of this exponent, which appear to depend on the stellar population chosen as a tracer. Even between groups using the same stellar tracer, the results are varied \citep{sluis;arnold_1998,de_propris;et-al_2010}. This is because the contamination, recoverability and fractional volume of the halo observed at a given galactocentric radii can be non-trivial to accurately quantify. Nevertheless the stellar halo diminishes quickly with increasing galactocentric radii, where the presence of accreted substructure becomes evermore apparent.

In recent decades it has become clear that at least part of the stellar halo has been formed through the accretion of small metal-poor satellite systems \citep{ibata;et-al_1994,belokurov;et-al_2006,grillmair_2006,bell;et-al_2008}. Stars from a disrupted parent system have coherent velocities that persist over long timescales. This allows us to identify individual stars that were once disrupted, and chronicle the merger tree of the halo from events that occurred long ago. Groups of stars can be identified by their position, kinematics and chemistry, and associated to a progenitor satellite that matches the phase space signature. It's possible that the entire stellar halo has formed through accretion \citep{bell;et-al_2008}, implying that every halo star is be a remnant from a fossil object accreted by the proto-Milky Way, each with completely independent -- and perhaps, distinguishable -- star formation histories.

\subsection{Dark Halo}
Kinematic galaxy studies as far back as \citet{freeman_1970} and \citet{rubin;et-al_1970} have repeatedly found galaxies to rotate faster than expected \citep[see also][]{rubin;et-al_1980}. This has led to a flurry of research, with the general acceptance that the dynamics are driven by non-luminous (dark) matter. The actual nature of dark matter remains elusive, but its effects are observable through the gravitational field. Exploring the properties of dark matter has shifted away from astrophysics towards particle physics. However, the quantity and distribution of dark matter remains quantifiable on astrophysical scales, providing important constraints for direct dark matter detection techniques.

The Milky Way is dark matter-dominated, with dark matter contributing $>$90\% of the total galactic mass \citep[$1-1.5 \times 10^{12} M_\odot$;][]{smith;et-al_2007,nichols;et-al_2012,kafle;et-al_2012}. The dark halo follows a $\rho \sim r^{-2}$ distribution out to at least 100\,kpc \citep[e.g.,][]{kochanek_1996,battaglia;et-al_2005}, enveloping most of the baryonic matter in the Milky Way. The distribution of dark matter is believed to be spheroidal rather than disk-like \citep{creze;et-al_1998,ibata;et-al_2001}. Although non-luminous, the gravitational forces of the dark halo significantly contribute to the structure of the luminous Galactic components. The misalignment of angular momentum between the dark and baryonic components can result in warps in the thin/thick disk. This implies that a triaxial dark halo distribution has strong repercussions for the tidal disruption of luminous systems in the stellar halo. Interestingly, from their models of the Milky Way--Sagittarius interaction, \citet{Law;et-al_2009} finds a tri-axial dark matter halo to best represent the observed positions and kinematics of stars in the Sagittarius (Sgr) stream (c.f. Chapter \ref{chap:sgr}).

Cosmological simulations \citep{moore;et-al_1999} of cold dark matter suggests that the dark halo is strongly substructured (i.e., clumpy). This has important consequences for the formation of the Milky Way, and the dissipation of the disk. While significant work has been placed on quantifying the complete mass distribution of dark matter sub-halos \citep[e.g., ][]{madau;et-al_2008}, some groups have attempted to identify individual clumps of dark matter via measurable dips in the surface brightness along a stream \citep{diemand;et-al_2008,carlberg;et-al_2012,carlberg;et-al_2013}. However it is not clear whether these observations can be used to identify individual dark matter sub-halos, or they are simply observing the presence of epicyclic stripping. 

\section{Substructure in the Milky Way}

The term substructure is used to describe a group of stars that demonstrate coherent and distinguishable signature in phase space. This coherence may be in any number of observables, including their position, kinematics, or possibly through individual elemental abundances. In the last two decades astronomers have discovered that the Milky Way is rich with substructure, particularly in the outer halo. This has been observed in the presence of globular clusters, open clusters, diffuse over-densities, and the tidal tails of disrupted systems -- also referred to as stellar streams. 

The presence of substructure in the Milky Way is evident by numerous photometric and spectroscopic studies \citep[for a review, see][]{helmi_2008}. Both diffuse and coherent over-densities (e.g. tidal tails) are observable in the Sloan Digital Sky Survey \citep[hereafter SDSS;][]{York;et-al_2000} with extremely simple colour cuts (e.g., see Figure \ref{fig:field-of-streams}). Radial velocities obtained by follow-up spectroscopy of individual stars in tidal tails reveals a composite velocity distribution: an expected Galactic velocity dispersion, and a significant peak of stars with similar, or indistinguishable, velocities. This signature is usually evidence of a co-moving group of stars which cannot be explained by a smooth halo distribution, radial mixing, or disk heating. Table \ref{tab:tidal-tails} outlines a number of known tidal tails in the Milky Way\footnote{Table \ref{tab:tidal-tails} is an updated and extended version of the database compiled by \href{http://homepages.rpi.edu/~newbeh/mwstructure/MilkyWaySpheroidSubstructure.html}{Heidi Newberg}.}. Diffuse photometric over-densities often have more elaborate explanations as the velocity distribution may be nearly homologous with the expected Galactic contribution. In these cases -- if the over-density is the result of a disrupted satellite -- it suggests considerable mixing has occurred since accretion, and at least some of the dynamical information has already been lost. Nevertheless, any stellar over-density in a focussed direction of the halo is a signature of a significant Galactic formation event. While dynamical information may be lost, distinguishing between accreted and in-situ scenarios may be discernible from detailed chemical abundances (see \ref{sec:intro-chemical-tagging}). Through successive generations of star formation, the detailed chemical abundances represent the integrated star formation history of the local environment. Thus, accreted and in-situ stars will exhibit distinguishable chemical signatures that are representative of their formation environment. With increasing observational data astronomers may be able to identify all substructure in the Milky Way, even those that have undergone nearly complete disruption. This will allow us to identify the inflexion point from in situ-dominated and accretion-dominated formation, build up the Galactic merger history, and would drastically increase the level of known accretion in the Milky Way.

\begin{figure}[h]
	\includegraphics[width=\columnwidth,height=0.5\columnwidth]{fos_dr6_marked.pdf}
	\caption[A mercator projection of the ``Field of Streams'']{A mercator projection of the ``Field of Streams'' \citet{belokurov;et-al_2006} assembled from SDSS images of the northern sky. Color indicates the approximate distance to the stars. Structures visible in this region of the sky are marked, including the prominent Sgr stream, the Orphan stream, the `Monoceros Ring', as well as a number of diffuse overdensities and globular clusters.\\Credit: Vasily Belokurov (Institute of Astronomy, Cambridge) and the Sloan Digital Sky Survey collaboration.}
	\label{fig:field-of-streams}
\end{figure}


\newcommand{\vat}[1]{\begin{tabular}{@{}l@{}}#1\end{tabular}}
\newcommand{\vatc}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}


\begin{table}
\caption{Tidal tails in the Milky Way\label{tab:tidal-tails}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccl}
\hline
\vat{\\Name\\} & \vatc{Right\\Ascension} & \vatc{Declination\\} & \vatc{Position\\Angle} & \vatc{Tail\\Length} & \vat{\\Literature\\ } \\
& (J2000) & (J2000) & ($^\circ$) & (kpc) & \\
\hline
\\

\multicolumn{6}{c}{\textbf{Disrupting Dwarf Galaxies}} \\
\hline
\object[NAME FORNAX dSPH]{Fornax} 			& 02:39:59.30	& $-$34:26:57.0	& --42		& 2.5	& \citet{coleman_fornax} \\
\vat{\object[NAME LMC]{LMC}\\\\ }	& \vat{05:23:33.61\\\\ }&\vat{$-$69:45:36.2\\\\ } & \vat{\nodata\\\\ }	& \vat{22\\\\ }& \begin{tabular}{@{}l@{}}\citet{putman_1998};\\\citet{munoz_2006}\end{tabular} \\
\vat{\object[CARINA dSPH]{Carina}\\\\ } & \vat{06:41:36.70\\\\ } & \vat{$-$50:57:58.0\\\\ } & \vat{65\\\\ } & \vat{\nodata\\\\ } & \begin{tabular}{@{}l@{}}\citet{irwin_1995};\\\citet{munoz_2006}\end{tabular} \\
\object[LEO I]{Leo I}	& 10:08:28.12 & $+$12:18:23.4 & 84 & $\sim$0.4 & \citet{sohn;et-al_2007} \\
\object[URSA MAJOR dSPH]{Ursa Major} & 10:34:52.80 & $+$51:55:12.0 & 78 & $\sim$29 & \citet{okamoto;et-al_2008} \\
\vat{\object[URSA MINOR dSPH]{Ursa Minor}\\\\ } & \vat{15:09:11.34\\\\ } & \vat{$+$67:12:51.7\\\\ } & \vat{53\\\\ } & \vat{3\\\\ } & \vat{\citet{irwin_1995};\\\citet{palma;et-al_2003}} \\
\vat{\object[NAME HER DWARF GALAXY]{Hercules}\\\\ } & \vat{16:31:02.40\\\\ } & \vat{$+$12:47:30.0\\\\ } & \vat{$-$73\\\\ } & \vat{$\sim$21\\\\ } & \vat{\citet{belokurov;et-al_2007_quintet};\\
\citet{coleman;et-al_2007}} \\ % D = 132 \pm 12 kpc from same article
\object[NAME SDG]{Sagittarius} & 18:55:03.10 & $-$30:28:42.0 & 100 & $>$500 &
\citet{pakzad;et-al_2004}
\\
\object[NGC 6822]{NGC 6822} & 19:44:56.20 & $-$14:47:51.3 & $\sim$170 & $\sim$1.4 & \citet{de_block;et-al_2000} \\
\hline

\\
\multicolumn{6}{c}{\textbf{Disrupting Globular Clusters}} \\
\hline

\object[NGC 362]{NGC 362} & 01:03:14.26	& $-$70:50:55.6	& $\sim$135 & $\sim$2.5 & \citet{grillmair;et-al_1995} \\
\object[NGC 1261]{NGC 1261} & 03:12:16.21 & $-$55:12:58.4	& $\sim$135 & $\sim$2.8 & \citet{leon;et-al_2000} \\
\object[NGC 1851]{NGC 1851} & 05:14:06.76 & $-$40:02:47.6  & $\sim$140 & $\sim$2 & \citet{leon;et-al_2000} \\
\vat{\object[NGC 1904]{NGC 1904} (M 79)\\\\ }& \vat{05:24:10.59\\\\ } & \vat{$-$24:31:27.3\\\\ } & \vat{$\sim$40\\\\ } & \vat{$\sim$2.4\\\\ } & \vat{\citet{grillmair;et-al_1995}\\\citet{leon;et-al_2000}} \\
\object[NGC 2298]{NGC 2298} & 06:48:59.41 & $-$36:00:19.1 & $\sim$150 & $\sim$1.5 & \citet{leon;et-al_2000} \\
\object[NGC 2808]{NGC 2808} & 09:12:03.10 & $-$64:51:48.6 & $\sim$160 & $\sim$3 & \citet{grillmair;et-al_1995} \\
\object[NGC 3201]{NGC 3201} & 10:17:36.82 & $-$46:24:44.9 & $\sim$140 & $\sim$4.4 & \citet{grillmair;et-al_1995} \\
\object[NGC 4372]{NGC 4372} & 12:25:45.43 & $-$72:39:32.7 & \nodata & \nodata & \citet{leon;et-al_2000} \\
\object[NGC 4590]{NGC 4590} (M 68) & 12:39:27.98 & $-$26:44:38.6 & $\sim$90 & $\sim$3.7 & \citet{grillmair;et-al_1995} \\
\vat{\object[NGC 5139]{NGC 5139} ($\omega$Cen)\\\\ } & \vat{13:26:47.28\\\\ } & \vat{$-$47:28:46.1\\\\ } & \vat{$\sim$165\\\\ } & \vat{$\gtrsim$5.3\\\\ } & \vat{\citet{leon;et-al_2000}; \\ \citet{majewski;et-al_2012}\\} \\

\object[NGC 5272]{NGC 5272} (M 3) & 13:42:11.62 & $+$28:22:38.2 & $\sim$85 & $\sim$3.5 & \citet{leon;et-al_2000} \\
\vat{\object[NAME NGC 5466]{NGC 5466}\\\\ } & \vat{14:05:27.29\\\\ } & \vat{$+$28:32:04.0\\\\ } & \vat{130\\\\ } & \vat{45\\\\ } & 
\vat{\citet{belokurov;et-al_2006_5466};\\\citet{grillmair_johnson_2006}} \\
\object[NGC 5694]{NGC 5694} & 14:39:36.52 & $-$26:32:18.0 & $\sim$135 & $\sim$1.3 & \citet{leon;et-al_2000} \\
\object[NGC 5824]{NGC 5824} & 15:03:58.61 & $-$33:04:06.7 & $\sim$175 & $\sim$3.8 & \citet{leon;et-al_2000} \\
\object[PAL 5]{Palomar 5} & 15:16:05.30 & $-$00:06:41.0 & 45 & 22.5 & \citet{grillmair_dionatos_2006a} \\

\object[NGC 5904]{NGC 5904} (M 5) & 15:18:33.22 & $+$02:04:51.7 & $\sim$140 & $\sim$1.3 & \citet{leon;et-al_2000} \\
\object[NGC 6205]{NGC 6205} (M 13) & 16:41:41.63 & $+$36:27:40.8 & $\sim$150 & $\sim$1 & \citet{leon;et-al_2000} \\
\object[NGC 6254]{NGC 6254} (M 10) & 16:57:09.05 & $-$04:06:01.1 & $\sim$5 & $\sim$4 & \citet{leon;et-al_2000} \\
\object[NGC 6397]{NGC 6397}  & 17:40:42.09 & $-$53:40:27.6 & $\sim$100 & $\sim$3.5 & \citet{leon;et-al_2000} \\
\object[NGC 6535]{NGC 6535}  & 18:03:50.51 & $-$00:17:51.5 & $\sim$160 & $\sim$0.8 & \citet{leon;et-al_2000} \\
\object[NGC 6712]{NGC 6712}  & 18:53:04.32 & $-$08:42:21.5 & \nodata & \nodata & \citet{de_marchi;et-al_1999} \\
\object[NGC 6864]{NGC 6864} (M 75) & 20:06:04.84 & $-$21:55:20.1 & $\sim$125 & $\sim$3 & \citet{grillmair;et-al_1995} \\
\object[NGC 6934]{NGC 6934} & 20:34:11.37 & $+$07:24:16.1 & $\sim$135 & $\sim$3 & \citet{grillmair;et-al_1995} \\
\object[NGC 6981]{NGC 6981} (M 72) & 20:53:27.70 & $-$12:32:14.3 & $\sim$100 & $\sim$2.8 & \citet{grillmair;et-al_1995} \\
\object[NGC 7078]{NGC 7078} (M 15) & 21:29:58.33 & $+$12:10:01.2 & $\sim$160 & $\sim$3.6 & \citet{grillmair;et-al_1995} \\
\object[NGC 7089]{NGC 7089} (M 2) & 21:32:35.27 & $-$44:04:02.9 & $\sim$55 & $\sim$3.3 & \citet{grillmair;et-al_1995} \\
\object[PAL 12]{Palomar 12} & 21:46:38.84 & $-$21:15:09.4 & $\sim$0 & $\sim$2.3 & \citet{leon;et-al_2000} \\
\object[NGC 7492]{NGC 7492} & 23:08:26.68 & $-$15:36:41.3 & $\sim$70 & $\sim$0.6 & \citet{leon;et-al_2000} \\
\hline
\end{tabular}}
\end{table}


Not all Galactic accretion has occurred long ago. The discovery that the Sgr dwarf spheroidal (dSph) galaxy was experiencing ongoing accretion is a prominent example for recent and substantial accretion onto the Milky Way. \citet{ibata;et-al_1994} detected the Sgr stream by a clear peak in their velocity distribution of stars in the direction of the bulge: a significant fraction of stars in their field all had nearly the same velocity, and that signature was distinct from the background Galactic contribution. Stars from the disrupting dwarf remained kinematically cold, and a coherent velocity histogram is observable for long timescales. Since its discovery, the tidal arms of the Sgr dwarf have been seen to encircle around the Milky Way with overlapping tidal tails, littering debris throughout the Galaxy. The Sgr stream remains the most prominent evidence of ongoing accretion in the Milky Way, inspiring extensive observational and theoretical work in the last two decades. 

Sgr is by far not the only example of recent accretion in the Milky Way. The epoch of large scale digital imaging surveys has facilitated significant leaps forward in galaxy formation and substructure identification. The SDSS and 2-Micron All Sky Survey \citep[hereafter 2MASS;][]{skrutskie;et-al_2006} have been particularly useful in this regard. Using these data, a wealth of structure has been identified across a broad range of cosmological scales. In fact, perhaps the most iconic example of substructure in the Local Group has  resulted from the SDSS catalogue. The aptly named `Field of Streams' \citep[Figure \ref{fig:field-of-streams};][]{belokurov;et-al_2006} contains a wealth of substructure in a single image. Multiple disrupting tidal tails are present including two arms of Sgr, as well as numerous globular clusters and diffuse over-densities. The coming decade will be equally exciting for substructure discovery, as the SkyMapper \citep{keller;et-al_2007} and Pan-STARRS \citep{hodapp;et-al_2004} telescopes begin their deep imaging surveys of the southern sky.

There is a wide distribution of masses and structure sizes that have been accreted onto the stellar halo across all cosmic times. Around $\sim$10 dwarf galaxies are known to be have undergone tidal disruption, and $\sim{}$30 of the 150 Galactic globular clusters present evidence of tidal tails. In addition to these systems, at least another dozen or so stellar streams have been identified \emph{without} the presence of any disrupting host (see Table \ref{tab:tidal-tails} for a referenced overview). A detailed account of the discovery and properties of these substructures is beyond the scope of this thesis\footnote{A full examination of known substructures in the Milky Way would serve as the subject of a (presumably) excellent review article in the future, years after a thorough deep photometric survey of the southern sky has concluded.}. A table highlighting some of the disrupting systems in the Milky Way without known parent systems is shown in Table \ref{tab:milky-way-substructure}.


Some tension exists between observations and theory of substructure in the Milky Way. Cold dark matter simulations suggest the level of substructure observed in the Milky Way is at least an order of magnitude less than what ought to be present. Simulations indicated there should be approximately $\sim{}$10-100 times more globular clusters and dwarf galaxies surrounding the Galaxy \citep{klypin;et-al_1999}. Although recent work \citep{kravtsov;et-al_2004,simon;et-al_2007,brooks;et-al_2012} has found the discrepancy between observations and theory is not as substantial as first proposed \citep[$\sim$4 too many;][]{simon;et-al_2007}, this disparity is commonly referred to as the `Missing Satellites Problem'. Additional Galactic satellites may be found through deep multi-band imaging of the Southern Sky, which would further alleviate or resolve this issue.


\subsection{Quantifying the Level of Substructure}

Many studies have tried to quantify the level of substructure in the halo, and the results are varied. Some groups have placed lower limits \citep{starkenburg;et-al_2009}, whereas others claim the entire halo ($D>20$\,kpc) to have been formed through accretion \citep{bell;et-al_2008}. There are many difficulties in measuring the substructure contribution, including the stellar tracer used \citep{preston;et-al_1991,green;morrison_1993,vivas;zinn_2006}, the definition employed to identify substructure, as well as recoverability and contamination, to name a few. The stellar tracer must also be intrinsically bright -- such that they can probe far distances in the halo -- and be relatively free of contamination.

When quantifying the level of substructure in the halo, one must be particularly careful when specifying what qualifies as a substructure. In the simplest scenario, a substructure may be definable as a cohort of stars with a common observable that is statistically significant above the smooth halo background. Unfortunately, even this abstract description is plagued. Defining statistical significance usually requires some comparison to a smooth model of the Galaxy. Even a statistical measure that is non-parameterized will require a comparison with a model of the smooth Galactic background. Thus, some model of the Galaxy has historically been employed to quantitatively measure substructure in the Milky Way. If the model employed is oversimplified, then the warp of the disk may be qualitatively recognised as statistically significant accreted substructure. In reality our over-simplification of the Galaxy is resulting in an over-estimation of the substructure present. These considerations become important in Chapter \ref{chap:aquarius}, where we examine the existence of the recently discovered Aquarius stream \citep{williams;et-al_2011}.


\subsection{Weighing the Milky Way}

In addition to probing the merger history of the Galaxy, there are key measurements that can be made with stellar streams. One of particular interest is measuring the mass of the Milky Way. Since the positions and velocities of stars in stellar streams are sensitive to the gravitational potential, tidal tails serve as powerful probes to measure the galactic potential \citep[e.g.,][]{adrn_2013}. Through this process, one can also infer the shape, extent and distribution of dark matter \citep[e.g., ][]{Law;et-al_2009}. These are critical measurements for cosmological simulations. 

Several groups have used the prominent Sgr stream for inferring the Milky Way potential \citep{edelsohn_1997,Law;et-al_2005,Law;et-al_2009}. The more diffuse, less luminous streams have also been used \citep{newberg;et-al_2010}, but this is reliant on a wealth of accurate positional and kinematic data \citep{adrn_2013}. As more exquisite distances are obtained from the Gaia satellite mission \citep{perryman}, more representative models of the Milky Way can be devised.


\begin{table}[h!]
\caption{Stellar streams in the Milky Way without associated systems\label{tab:milky-way-substructure}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccl}
\hline
\vat{\\Name\\} & \vatc{Right\\Ascension} & \vatc{Declination\\} & \vatc{Position\\Angle} & \vatc{Tail\\Length} & \vat{\\Literature\\ } \\
& (J2000) & (J2000) & ($^\circ$) & (kpc) & \\
\hline
\object[Cetus Polar Stream]{Cetus Polar Stream} & 01:33:24 & $+$03:13:48 & \nodata & \nodata & \citet{newberg;et-al_2009} \\
\object[Triangulum Stream]{Triangulum Stream} & 01:35:54 & $+$23:12:04 & $\sim$160 & 5.5 & \citet{bonaca;et-al_2012} \\
\vat{\object[Orphan Stream]{Orphan Stream}\\\\ } & \vat{10:40:00\\\\ } & \vat{$+$05:00:00\\\\ } & \vat{159\\\\} & \vat{60\\\\ } & \vat{\citet{grillmair_2006};\\\citet{belokurov;et-al_2006}} \\
%GD2006 & 10:44:00 & +43:00:00 & $\sim$45 & 63 & \citet{grillmair_dionatos_2006b} \\
\object[Styx Stream]{Styx Stream} & 13:56:24 & $+$26:48:00 & $\sim$45 & 65 & \citet{grillmair_2009} \\
\object[Acheron Stream]{Acheron Stream} & 15:50:24 & $+$09:48:36 & $\sim$70 & 37 & \citet{grillmair_2009} \\
\object[Lethe Stream]{Lethe Stream} & 16:15:45 & $+$29:57:00 & $\sim$30 & 87 & \citet{grillmair_2009} \\
\object[Cocytos Stream]{Cocytos Stream} & 16:29:22 & $+$26:40:12 & $\sim$40 & 80 & \citet{grillmair_2009} \\
\hline
\end{tabular}}
\end{table}


\section{Chemical Evolution of the Milky Way}

Astrophysics is limited by observations; we cannot easily replicate the conditions of stellar interiors in any laboratory. Additionally, we cannot directly observe the interiors of stars. The interior must be inferred with models employing observables as boundary constraints. Only the outer layers of the photosphere are accessible for the inference of stellar structure and elemental abundances. Modulo surface abundance variations due to internal mixing, atomic diffusion and mass transfer from a binary companion, the abundances in the photosphere of a star retain the chemical signature of the proto-stellar gas cloud from which they formed. Thus by measuring the elemental abundances of a given star, we are effectively observing the gas cloud composition where that star was born. 

This facilitates extraordinarily research. Since each star forms from gas chemically enriched by its predecessors, the observed chemical abundances for any star are the cumulative sum of elements produced throughout its star formation history. Through measuring the elemental abundances in stellar photospheres we can effectively trace the changing gas composition throughout the Milky Way history, as well as the yields and frequency of supernovae throughout throughout the Galaxy. Even as dynamical signatures dissipate over time, the chemical signature remains largely fossilised in the photospheres of stars.

High-resolution spectra are required to accurately capture the full extent of chemical abundances for a given system. While overall metallicities can be reliably obtained from low-resolution spectra ($\mathcal{R} < 2000$), the evolution of abundance groups (e.g., $\alpha$-elements, Fe-peak elements, and neutron-capture elements) is critically important to infer the environment where those stars have formed, and can only be accurately ascertained with high-resolution spectra ($\mathcal{R} \sim 20,000+$). With high-resolution spectra from enough stars, the chemical enrichment of a system can be fully characterised. Following this idea, large samples of high-resolution spectra allow us to identify stars that have formed from the same gas composition, but are now dispersed in Milky Way \citep[e.g., `chemical tagging';][]{freeman;bland-hawthorn_2002}.

For tidal tails in the Milky Way that do not have a known parent system, this allows us to infer properties of the undiscovered host before it is discovered. With high-resolution spectra of disrupted members, one can reveal the chemical enrichment of the stream system, and compare its chemical signatures to known satellites in the Galaxy. This approach becomes relevant in Chapter \ref{chap:orphan_II}, where we undertake the first high-resolution spectroscopic study on the Orphan stream.

\subsection{Chemically Tagging the Galaxy}
\label{sec:intro-chemical-tagging}

In the coming years a number of high-resolution spectroscopic surveys will be completed. The APOGEE \citep{apogee} and the Gaia-ESO \citep{gilmore} surveys are already underway, and the GALAH survey \citep{hermes} is commencing in 2014A. These surveys complement each other in their scientific objectives, target selection, and spectral coverage. Together, they will obtain high-resolution spectra for over a million stars -- an unprecedented volume of spectral data in astronomy.

With these data, the chemical evolution of the Galaxy can be unravelled. Moreover it may be possible to chemically tag individual stars as remnants of individual proto-galaxy fragments. The merger history of the Milky Way can be exposed with unprecedented detail, allowing for the exploration of stellar interiors, nucleosynthesis, and galactic structure formation. However the crux of these interpretations will rely on the homogeneity of their spectral analyses. As we will outline in Chapters \ref{chap:smh} and \ref{chap:aquarius}, non-negligible offsets in results are found between spectroscopists, even with high-resolution spectra. To infer minute chemical differences throughout the Galaxy, a homogenous analysis is essential. For the high-resolution spectra presented in Chapters \ref{chap:orphan_II} and \ref{chap:aquarius}, we have strived for an easily reproducible, homogenous analysis through the use of the analysis software outlined in Chapter \ref{chap:smh}.

% can't observe stellar interiors where elements are forged
% can only observe outer abundances
% outer abundances serve as a relic of the protostellar gas cloud
% thus by measuring the elemental abundances in stars we can trace the changing protostellar gas clouds throughout the history of the galaxy
% allowing us to trace supernovae yields throughout the galaxy
% the stellar abundances in a star are the cumulative star formation history
% 

% Chemical evolution of the Milky Way
% - traces supernovae yields of the Galaxy
% - from hydrogen until now
% - separate the thick/thin disc
% - chemical tagging
% - Unravelling the Milky Way
% - is the milky way normal?

\section{Thesis Outline}
Although the formation history of the Milky Way is tangled and chaotic, it serves as an excellent -- and more importantly, accessible -- laboratory to investigate the evolution of the Universe since the earliest times. To understand the formation history of the Milky Way, this thesis investigates known substructures in our Galaxy. Specifically, we focus on the Virgo Over-Density (VOD), and three previously discovered tidal tails; the Sgr stream, and the Orphan and Aquarius streams. We aim to place these systems in context with the rest of the Galaxy, and to further chronicle the Milky Way's evolution. Thus far we have presented an introduction to cosmological structure and galaxy formation and the components of the Milky Way have been outlined, providing context for the following chapters.

In Chapter \ref{chap:sgr} we present an analysis of low-resolution spectra taken in the vicinity of the VOD and the Sgr stream. Although debris from the Sgr stream is littered throughout the Galaxy, it is distinctive from the galactic background and coherent in position and velocity. In contrast the VOD is a diffuse cloud of stars, showing an excess of stellar material from its polar opposite. Both of these substructures -- and others -- reside in a complex, accretion-dominated region of the sky. We explore the metallicity distribution function of each system, and use phase-space information on the Sgr debris to constrain the shape and extent of dark matter in the Milky Way.

The structure of Chapter \ref{chap:smh} is distinguishable from the rest of this thesis. Chapter \ref{chap:smh} outlines a software package that was written during the course of this doctoral candidature. This software, named `Spectroscopy Made Hard', has been written with the intent to streamline the analysis of high-resolution stellar spectra. The motivation for this software is outlined, and the steps involved in a classical curve-of-growth analysis are discussed in the context of presenting the software. This software has been used for a number of projects by expert spectroscopists, and has been used for the analysis of spectra in Chapters \ref{chap:orphan_II} and \ref{chap:aquarius}.

Chapter \ref{chap:orphan_I} presents the first of two chapters where we investigate the Orphan stream. The Orphan stream was independently discovered by \citet{grillmair_2006} and \citet{belokurov;et-al_2006} in the SDSS catalogue, stretching over 60$^\circ$ of arc. In Chapter \ref{chap:orphan_I} we present our method to identify sparse red giant branch stars in the stream from low-resolution spectra.

High-resolution spectra were obtained for a number of targets presented in Chapter \ref{chap:orphan_I}. Strong conclusions about the undiscovered host system can be drawn from the detailed chemical abundances of the disrupted stream stars. We present our analysis of these spectra in Chapter \ref{chap:orphan_II}, and discuss our chemical abundances in context of  known systems that have been suggested as the parent to the Orphan stream.

A detailed examination of the Aquarius stream is chronicled in Chapter \ref{chap:aquarius}. The Aquarius stream was discovered by \citet{williams;et-al_2011} from the Radial Velocity Experiment \citep[hereafter RAVE;][]{steinmetz;et-al_2006} survey catalogue. A follow-up spectroscopic analysis by \citet{wylie-de-boer;et-al_2012} proposed the Aquarius stream to have resulted from a disrupted globular cluster. We have obtained high-resolution, high signal-to-noise ($S/N$) ratio spectra for a third of the known members in the stream. Detailed chemical abundances suggests the stream is actually Galactic in origin, ruling out any accretion origin.

Concluding remarks are summarised in Chapter \ref{chap:conclusions}, which includes a discussion of future work planned for the analysis software presented in Chapter \ref{chap:smh}.


% I think ctable gives the best LaTeX tables, once you get to know its syntax. All of the objects in this table are resolvable in SIMBAD using the \object{} command defined in macros.tex


